Optimizing LLM Queries in Relational Data Analytics Workloads

Batch data analytics is a growing application for Large Language Models (LLMs). LLMs enable users to perform a wide range of natural language tasks, such as classification, entity extraction, and translation, over large datasets. However, LLM inference is highly costly and slow: for example, an NVIDIA L4 GPU running Llama3-8B can only process 6 KB of text per second, taking about a day to handle 15 GB of data; processing a similar amount of data costs around $10K on OpenAI's GPT-4o. In this paper, we propose novel techniques that can significantly reduce the cost of LLM calls for relational data analytics workloads. Our key contribution is developing efficient algorithms for reordering the rows and the fields within each row of an input table to maximize key-value (KV) cache reuse when performing LLM serving. As such, our approach can be easily applied to existing analytics systems and serving platforms. Our evaluation shows that our solution can yield up to 3.4x improvement in job completion time on a benchmark of diverse LLM-based queries using Llama 3 models. Our solution also achieves a 32% cost savings under OpenAI and Anthropic pricing models.

==> evaluation/queries.tex <==
\begin{itemize}
    \item \textit{Q1/Q5: LLM Projection}
    \vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Recommend movies for the user based on {movie information} and {user review}', m.info, r.review)
FROM reviews r JOIN movies m ON r.link = m.link
\end{minted}
\end{mdframed} 
\vspace{4pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Given the following fields, answer in ONE word, 'Yes' or 'No', whether the movie would be suitable for kids.', 
    mr.*)
FROM ( SELECT r.*, m.* FROM reviews r JOIN movies m ON r.link = m.link ) AS mr
\end{minted}
\end{mdframed} 

    \vspace{8pt}
    \item \textit{Q2: LLM Filter}
    \vspace{8pt}
    
    \begin{mdframed}[linecolor=black, linewidth=.5pt]
    \begin{minted}[fontsize=\small]{sql}
SELECT m.movie_title
FROM Movies m JOIN Reviews r ON r.link = m.link
WHERE LLM('Analyze whether this movie would be suitable for kids based on {movie information} and {user review}', m.info, r.review) = 'Yes'  
AND r.rtype == 'Fresh'
    \end{minted}
    \end{mdframed} 
    \vspace{8pt}

    
    \item \textit{Q3: Multi-LLM invocation}
    \vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Recommend movies for the user based on {movie information} and {user review}', m.info, r.review) AS recommendations
FROM Movies m JOIN Reviews r ON r.link = m.link
WHERE LLM('Analyze whether this movie would be suitable for kids based on {movie information} and {user review}', m.info, r.review) = 'Yes'  
AND r.rtype = 'Fresh'
\end{minted}
\end{mdframed} 
    \vspace{8pt}
    
\item \textit{Q4: LLM Average}
\vspace{10pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT AVG(LLM('Rate a satisfaction score between 0 (bad) and 5 (good) based on {review} and {info}: ', r.review, m.info)) as AverageScore
FROM reviews r JOIN movies m ON r.link = m.link
GROUP BY m.movie_title
\end{minted}
\end{mdframed} 
    \vspace{8pt}
%     \item \textit{Q5: LLM Projection (Entire Table)}
% \vspace{10pt}
% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
% SELECT LLM('Given the following fields, answer in ONE word, 'Yes' or 'No', whether the movie would be suitable for kids.', 
%     mr.*)
% FROM ( SELECT r.*, m.* FROM reviews r JOIN movies m ON r.link = m.link ) AS mr
% \end{minted}
% \end{mdframed} 
%     \vspace{8pt}
    \item \textit{Q6: RAG}
    \vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Given the following {context}, answer this {question}', VectorDB.similarity_search(s.question), s.question)
FROM squad s WHERE s.is_impossible = False
\end{minted}
\end{mdframed}
% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
% SELECT
%     LLM("You are given 3 pieces of evidence as {evidence_1}, {evidence_2}, and {evidence_3}. You are also given a claim as {claim}. Answer SUPPORTS if the pieces of evidence support the given {claim}, REFUTES if the evidence refutes the given {claim}, or NOT ENOUGH INFO if there is not enough information to answer. Your answer should just be SUPPORTS, REFUTES, or NOT ENOUGH INFO and nothing else.",
%         VectorDB.similarity_search(f.claim) AS evidence_1, evidence_2, evidence_3,
%         f.claim
%     FROM fever f
% \end{minted}
% \end{mdframed}
%     \vspace{8pt}

%     \item \textit{Q6: Different SQL Operators (Join)} \shu{Not sure this is a good example}
%     \vspace{8pt}
% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
%  SELECT 
%     p.product_id, 
%     p.product_desc, 
%     r.review_content
% FROM Reviews r
% JOIN 
%     Products p ON p.product_id = (
%         SELECT product_id
%         FROM VectorDB.similarity_search(
%             LLM("Extract product mention from {review}", r.review_content),
%             p.product_desc
%         )
%         LIMIT 1
%     )
% \end{minted}
% \end{mdframed} 
    \vspace{8pt}
\end{itemize}

==> figures/z-notes.tex <==
There is a rich history of integrating machine learning models with the database for improved performance. In large part, past work has focused on how to optimize the \textit{training} process. For instance, many techniques have been developed to update models with the arrival of new data~\cite{}. In this setting, the database is a part of the training pipeline

There are decades of research on bringing machine learning into the database. For instance, ...
For the most part this work has focused on how to optimize the \textit{training} process using a database system.

Integrating LLMs into the database represents a paradigm shift from previous work. In this setting, we must consider how to optimize in-context learning and \textit{inference} with database systems. Rather than scanning and querying over large batches of data for training, inference applies specific functions over a defined set of data.


LLM background: why LLMs are expensive

We leverage the unique properties of LLMs to optimize these queries.

LLMs provide a convenient mechanism to process strings in a database.  

To enable complex data-intensive applications, the database community has expended considerable efforts in integrating machine learning models into data systems for improved performance. In large part, the focus of previous work has been on \textit{model training}. For instance, MauveDB~\cite{mauvedb} presents an early example of how to support models in the presence of frequent updates to data.
In recent years, research has expanded to also consider model deployment, serving, and management~\cite{velox}. The complex problems of providing low latency, serving at large scale, and managing integrated pipelines have been studied in detail~\cite{}.

Specifically, we assume that LLM requests are generated as a part of a SQL query over data stored in a relational database.

This process continues until the model outputs a termination token. As such, this sequential generation process requires that all tokens be stored in memory. 

A LLM stores all this state in the \textit{KV cache}, which represents the primary bottleneck for serving throughput. Since each request is processed sequentially,  However, there is a delicate tradeoff between processing larger batch sizes and overfilling the KV cache as tokens are generated during inference. 

and does not leverage query structure present in batch analytics to achieve higher throughput.

Invoking a model in such a way present many opportunities for inference optimization. 

At a high level, the task of language modeling is to model the probability of a list of tokens:  LLMs compute the joint probability over the whole sequence as the product of conditional probabilities (a.k.a. autoregressive decomposition~\cite{}). 

Until the model outputs a termination token, this generation continues sequentially, and 

Intuitively, the larger a batch that the LLM can process, the higher the serving throughput it observes. However, the LLM must ensure the batch size is not too large---all tokens for each request must fit in the available memory. Thus, balancing the tradeoff between memory and compute is the critical challenge for LLM inference today.

storing all the tokens to process [1] request requires, on average, 

% \accheng{talk about inference process and then cache}
% \accheng{talk about prefill as well}
% \accheng{just talk about prefix prompts}
% \accheng{separate section for background

% then have a section for opportunities in batch analytics: reordering, deduplication, and cost-optimization

% use a way to have list of them stand out more: here are the things that are new, make sure they don't miss it
% }

intelligent memory management is crucial for LLM inference today. Currently, state-of-the-art accelerators have [X]GB of RAM, of which 65\% of this memory must be allocated for the model weights~\cite{}. The remaining roughly 30\% is used to serve requests and how effectively this memory is utilized determines serving throughput.

recent work proposes \textit{memory sharing} to avoid storing the same \textit {system prompts} \accheng{just say prefix}, which are descriptions of the task including instructions and example inputs and outputs. A LLM user typically provide a system prompt along with task input (i.e., data) to form the prompt of a request. S 

\accheng{batch analytics key difference: reordering and other optimizations}


the database with knowledge of what data will be processed before inference.

batch analytics with LLMs presents many opportunities for optimizations since the database has access to the full set of queries before they are processed by the LLM.

\textbf{Opportunities with batch analytics.}

challenges for database systems: namely, how to 

% Advancements in LLMs have significantly expanded the capabilities of natural language processing, offering unique opportunities for integrating LLMs with database systems to enhance batch analytics. However, this integration introduces several challenges that must be addressed to fully leverage the potential of LLMs in this context. 
With the integration of LLMs into database systems, there are several key challenges for improving  We highlight the opportunities in batch analytics that are not exploited by online LLM inference systems or 

The rise of LLMs presents new challenges in optimizing for in-context learning and inference.  such optimizations and propose of range of new techniques for inference.

and typically adopt a simple eviction policy, such as [LRU]~\cite{}. \shu{LRU is probably fine, but they process the requests in sequence (no reordering, etc.)}


% tokens are produced based on the the product of conditional probabilities over the whole sequence.

% Since language has a natural sequential ordering, the task of language modeling is also serial: an LLM produces tokens based on the the product of conditional probabilities over the whole sequence. As a result, the LLM can only generate new tokens one by one for each request since the process depends on all the previous tokens in that sequence. 
% \accheng{add figure from vLLM talk}

\accheng{only sharing during prefill, not decoding?}

do not consider requests until they have arrived
\begin{itemize}
    \item Existing systems automatically admit every request into the KV cache and evict only when the cache runs out of space since they do not know what requests will be made a priori.
    \item In the offline setting, batch queries enumerate exactly when prefixes should be loaded into and removed from cache. \accheng{not admitting things saving writing to GPU memory, evicting proactively in a batch (more efficient)}
    \item Preemptively reducing the cache can free up memory for other LLM computations. \accheng{what is memory used for?}
\end{itemize}

In current systems, the default execution of batch queries with LLMs in FIFO order can result in significant underutilization of the KV cache. 
\begin{itemize}
    \item Online inference systems make no assumptions about future requests and process requests in arrival order. 
    \item In contrast, batch workloads provide full information about what requests need to be processed, and this can be used to maximize reuse of shared prefixes.
    \item Furthermore, batch queries operate over structured data, offering additional opportunities for memory management at the record and row level. For instance, [grouping together requests that all share the same field...] \accheng{shu: add example here}
    \item Existing inference engines~\cite{} do not leverage this knowledge to make better caching decisions, leading to premature eviction of useful data or unnecessary retention of unused prefixes.
\end{itemize}

an oracular scheduling algorithm that ensures we only cache prefixes that lead to future hits ... \accheng{update text}

has enabled the increased use of complex analytics tasks at unprecedented scale. 

LLMs are here to stay and will have a growing impact.
\begin{itemize}
    \item Advances in LLM are reshaping the current landscape of natural language processing 
    \item Diverse range of applications, including QA, chat applications, and mix of others 
\end{itemize}

, which represent a rapidly growing workload as developers apply these models to the enormous corpus of text data stored in relational systems today. 

the effectiveness of support services for customer service requests. Such queries will become increasingly common as LLMs are integrated into data-intensive applications.

Existing systems  %\shu{currently even they receive a large batch of requests, they do no special processing with it and process it sequentially}

% \accheng{Jump straight into problem
% LLM query example

% Explain tokens are many KB, scope for how much state is used

% Why do we need to batch stuff? because of autoregressivve nature, to utilize full capacity of hardware
% Balance between memory + compute is critical challenge
% Existing systems optimize in online setting but in SQL query, we have full knowledge of offline batch
% Prior work in DB-ML has looked at data flow workflows but none of this addressed strong order data-dependence; tradeoff between memory and CPU

% Highlight key differences of LLM

% Some figures would be nice (vLLM talk)

% A little more explanation about inference process
% }

% \shu{Following are my prefix background}
% \textbf{Introduction} 
% \begin{itemize}
%     \item The application of LLMs in processing batch workloads reveals patterns in data access and request structuring. 
%     \item A commonality across many query workloads is the shared prefixes within the inputs to the LLM.
%     \item These prefixes can take various forms, such as prompts (i.e. questions asked across many rows) or common database fields that recur across multiple records. 
%     \item This repetition present an opportunity for optimization, especially considering the computational cost and time associated with processing large volumes of data through LLMs. 
%     \item The identification and reuse of these shared prefixes enables faster and more efficient LLM processing model 
% \end{itemize} 
% \textbf{Prefix Cache Background}
% \begin{itemize}
%     \item Prefix caching is an approach to optimize the performance of LLMs by caching the KV values associated of previously computed prefixes in GPU memory. 
%     \item When new request arrives with a prefix that matches a cached entry, the LLM can bypass the initial computation steps, directly retrieved the stored result for the prefix. 
%     \item This reduces the computational overhead for frequent or repetitive inputs, leading to faster response times. 
% \end{itemize}

% \subsection{Queries and Goals}
% \todo{Maybe put the example here, and put the goals similar to the NoScope paper} \accheng{if we make this clear in intro, not sure we need this here}

% \accheng{Just talk about opportunities; existing engines are too basic---just say existing engines not designed to do offline inference

% optimizing batch analytics--we create new opportunities by knowing the workload info
% }
% \todo{when should we introduce the goals? of low latency?} \accheng{in the intro} \shu{Reference the Velox paper, maybe have an example application and the most naive solution}

% , which existing online inference systems are not designed to leverage.
% We highlight the challenges in improving end-to-end latency for SQL queries that invoke LLMs that are not addressed by online LLM serving systems.
%or existing techniques that optimize other machine learning models for databases. 

% a reordering algorithm that operates at the row and column level for input data to ensure that shared prefixes only need to be stored in cache once. Our strategy provides \textit{optimal} cache hit rate for a given workload.
% We also provide cache admission and eviction algorithms to ensure we only cache prefixes for as long as they benefit future requests.

% \accheng{is this true?}
% , including the structured nature of our data and access to all queries before execution,

% Limited Cache Reuse and Inefficient Request Formulation
%suboptimal cache usage. 
% A significant challenge is the inherent inefficiency in how batch requests are formulated, leading to minimal reuse of cached computations of prefixes. 
% \begin{itemize}
%     \item LLM is an order-sensitive UDF  
%     \item Structured data contain some information about characteristics of batch workloads (e.g. which fields are shared the most, etc.) 
% \end{itemize}

% \textit{Our Approach: Formulate Request with Reordering} We propose formulating the requests by strategically manipulating the order of input data.  
% \begin{itemize}
%     \item This can be done by ordering records and ordering fields within rows. 
%     \item This approach maximizes cache reuse by ensuring that requests with common prefixes are processed sequentially, thus enhancing the cache hit rate. 
% \end{itemize}

% \textbf{Suboptimal Cache Management}
% Existing cache management strategies of LLM inference engines (e.g. vLLM, SGLang) are not tailored to the unique demands of batch workloads. 
% \begin{itemize}
%     \item Fail to make informed decisions about prefix caching for offline workloads, leading to premature eviction of useful data or unnecessary retention of unused prefixes. 
%     \item This mismanagement results in inefficient memory usage and increased processing times. 
% \end{itemize}
  
% \textit{Our Approach: Batch-Aware Cache Scheduling} Leveraging the structured nature of our reshaped workload, we can make informed decisions on cache admission and eviction. 
% \begin{itemize}
%     \item This proactive strategy ensures optimal memory usage and minimizes the need for additional processing when there is not enough memory. 
% \end{itemize}

% \subsubsection{\todo{@Audrey} Explaination of Continuous Batching?}
% Continuous batching, also referred to as dynamic batching or iteration-level scheduling, is an method designed to enhance the efficiency of LLM inference. 
% \begin{itemize}
%     \item Traditional batching process requests in bulk, leading to delays as each requests waits for the entire batch to be processed. 
%     \item In contrast, continuous batching operates on a more granular level, handling tasks at the iteration stage. 
%     \item As soon as one iteration is completed, completed requests are removed, and new ones are added, allowing new requests to be processed after just a single iteration instead of waiting for a whole batch cycle. 
% \end{itemize}
% The presence of duplicate data elements and the lack of intelligent query optimization when invoking external UDFs like LLMs lead to redundant computations and inefficient execution strategies. 
% \begin{itemize}
%     \item Duplicate inputs are not processed before passing into these expensive UDFs. 
%     \item Traditional SQL optimizers are not equipped to handle the nuances of LLM inference, resulting in costly and time-consuming query processing.
% \end{itemize}

% \textit{Our Approach: Deduplication and SQL Optimizations}
% We address these challenges by implementing deduplication strategies with a set of hard rules and informing SQL optimizers of the expensive UDF calls. 
% \begin{itemize}
%     \item Hard rules: identify and eliminate redundant data before LLM invocation
%     \item SQL optimizers: recognize the cost of LLM calls, allowing for the prioritization of cheaper operations. 
%     This not only reduces the computational load but also ensures that the most expensive operations are invoked only when necessary, leading to more efficient query execution overall.
%     \item \shu{Shall we make a case for those hard rules}
% \end{itemize}

% \textbf{Lack of Workload Optimization}

% \begin{itemize}
% \item Batch workloads present unique opportunities for optimization that are not adequately exploited by current systems. 
% \item The potential for formulating requests to maximize cache reuse and enhance GPU utilization remains largely untapped.
% \item The absence of efficient workload shaping mechanisms, such as record-level and row-level reordering, hampers the ability to optimize prefix caching and reduce latency.
% \end{itemize}

% \textbf{High Computational and Monetary Costs} 
% \begin{itemize}
%     \item Naive execution of LLMs on large datasets can be prohibitively expensive, both in terms of computation and cost. 
%     \item Traditional SQL query optimizers are not designed to account for the cost characteristics of LLM invocations, leading to inefficient query execution plans. 
% \end{itemize}

% \textbf{Inefficient Cache Utilization}
% \begin{itemize}
% \item Current prefix cache management systems are primarily optimized for online, real-time processing. They lack the global scheduling awareness necessary for efficient batch workload processing, resulting in suboptimal cache hits and unnecessary recomputations.
% \item The existing cache management strategies do not effectively utilize the knowledge of batch workloads' structure, leading to premature eviction of useful prefixes or caching of unnecessary ones.
% \end{itemize}


% \textbf{Formulating Request}
% \textbf{Knowledge of Entire Batch for Scheduling}
% \textbf{Invoke Less: Cost-aware SQL Execution and Dedup}

% in a SQL query can lead to redundant computation: there are opportunities to reduce latency by minimizing the number of calls to the LLM.
% not processing duplicate queries and minimizing the number of LLM calls that need to be made.
\begin{itemize}
    \item 
   \item 
   \item 
    % LLM inference is usually the most expensive part of a SQL query, and this should be accounted for by traditional SQL optimizers.
\end{itemize}

\begin{itemize}
    \item We deduplicate prefixes before invoking the LLM.
    \item We adapt natural language processing techniques to identify redundant data before LLM invocation. 
\end{itemize}

\begin{itemize}
    \item 
    \item 
\end{itemize}

\accheng{in the same batch for our implementation}

\accheng{focus on the reordering}

These applications then leverage the LLM to perform data analysis, etc...

\begin{itemize}
    \item 
    \item 
    \item 
    % End-to-end latency \accheng{of the entire query} is the key metric for measuring LLM performance.
    % \item LLM is usually the bottleneck
    % \item LLM inference is typically bottlenecked on memory: requests are processed in batches and all requests (as well as their generated responses)  \accheng{introduce prefix and KV}
    % \item At a high level, LLM inference occurs sequentially for each request for which the model generates words as tokens one by one. For higher throughput, existing systems batch together requests. Crucially, all input prompts (i.e., \textit{prefixes}) and generated tokens must fit in memory within the key-value (KV) cache that stores tokens as key and value vectors.
    \item 
    \item 
    % \item Online systems admit all prefixes into the cache and evict once it is full.
\end{itemize}

We apply a variety of NLP preprocessing techniques to dedpulicate queries \textit{without} affecting accuracy of the end result. \accheng{just say we do exact, approximate for later}
    \item 
    \item     
% \end{itemize}

% There has been explosive interest in large language models (LLMs) across a range of different fields. LLMs provide general-purpose comprehension and generation of natural language, enabling a range of new applications and workloads that process textual data. To invoke LLMs, a growing class of applications query these models on structured data stored in relational systems. 

% \ion{that lead to redundant LLM invocations.}

\ion{and caching previous results}

==> mlsys/old_methodology.tex <==
\section{Recursive Request Reordering}
\label{sec:column-reordering}

This section introduces our request reordering algorithms which re-arranges the columns for each row to maximize prefix sharing in the KV cache. We leverage full workload information from analytical queries to ensure requests sharing the same prefixes are executed consecutively. Specifically, we first present an optimal recursive reordering algorithm to maximize prefix hit count (Sec~\ref{sec:optimal}). 
Because this algorithm has exponential complexity, we then introduce an efficient greedy simplification of the optimal algorithm  (Sec~\ref{sec:greedy}).
% with various optimizations that can be applied to real-world tasks .

% say worst case runtime, and say best case runtime too
% \accheng{update this sentence}
% in proximity of one another, thus optimizing the  

\subsection{Problem Setup}

% \textbf{LLM Request Structure.} 
We define the LLM function within the context of SQL queries. In addition to the text of the prompt, this function accepts \emph{set} expressions listing one or more columns $\{T.a, T.b, T.c\}$ or $\{T.*\}$ of table $T$.
This API design enables us to dynamically reorder fields within these expressions to optimize for cache efficiency. 

% \textbf{Objective} 
The goal of request scheduling is to \textbf{maximize} the \textit{prefix hit count} (PHC) by optimizing the order of columns and rows of an input table with $n$ rows and $m$ columns. 
Note that for each row, there may be a different column order.
We represent a request schedule as a list of tuples, $L$, where each tuple in $L$ corresponds to a row in the original table, and the tuple elements are the values within the row. The tuple order in the list can be rearranged to represent different row orders, and the order of the elements in each tuple can be rearranged to represent the chosen column order for the row. 
We pass the list $L$ of input requests along with the desired prefix prompt to the LLM for inference.
When providing each row as an input request to the LLM, we prepend column names in front of values to indicate the column each value belongs to using a standard JSON encoding.


% Each tuple in $L$ corresponds to a row, and the elements of the tuple correspond to the values within the columns. 

We define the PHC of $L$ as the number of consecutive column cell values shared with the previous row starting from the first cell, summing over all rows from $0$ to $n-1$. Each cell value must exactly match the corresponding cell of the previous row (cannot be a substring), and cell values past the first must match consecutively (must be a prefix). 
% We assume that the previously seen prefix must match the entire value of a previous cell, and cannot be a substring. 
Formally, a cell in the list of tuples is denoted as $L[r][c]$, indicating the value in tuple $r$ at position $c$. Then, the PHC for a list of tuples $L$ with $n$ rows and $m$ columns is given by: 
% $\text{PHC}(T) = \sum_{i=0}^{n-1} \max_{1 \leq j \leq m} \textit{hit}(T_{i,j})
% $. 

\begin{equation}
\text{PHC}(L) = \sum_{r=0}^{n-1} \textit{hit}(L, r)
\label{eq:phc}
\end{equation}

Here, the function $\textit{hit}(L, r)$ represents the prefix hit count for a single row $r$ in $L$. For simplicity, we assume that the input list is sorted. For each row $r$, the function checks if the value in each column $t$ matches any previously seen value in the same column of the previous row $r-1$. If all previous columns match, the hit count is the sum of the squares of the lengths of the values in those columns until a mismatch occurs. The squared lengths reflect the quadratic complexity of token processing in LLM inference, where each token computation depends on every preceding token and increases computational cost quadratically with input length. 
% \shu{make it clear about the Tuple index, tuple has order that represents column ordering; have to sort to make things work, previous rows (overlap), simplify by looking at, assuming at least one row fits into KV cache; n-1 (how much overlap, assume cache is large enough to reuse for previous few rows)}

% It is defined as the length of the concatenated string of cell values for row $i$ from column $1$ to $j$, if and only if all the concatenated cell values exactly match the previously seen concatenated cell values in the same columns.

% Defined over all previous rows 
% \begin{equation}
% \textit{hit}(L, r) = \max_{0 \leq c < m}
% \begin{cases} 
% \sum_{t=0}^{c-1} \text{len}(L[r][t])^2 & \text{if } \FORall t \leq c, L[r][t] = L[x][t] \\
% & \quad \exists x \text{ s.t., }  0 \leq x < r \\
% %& \quad \max\left(0, r -q \right) \leq x < r \\
% 0 & \text{otherwise}
% \end{cases}
% \label{eq:hit}
% \end{equation}

\begin{equation}
\textit{hit}(L, r) = \max_{0 \leq c < m}
\begin{cases} 
\sum_{t=0}^{c-1} \text{len}(L[r][t])^2 & \text{if } \forall t \leq c, L[r][t] = \\ & L[r-1][t] \\

%& \quad \max\left(0, r -q \right) \leq x < r \\
0 & \text{otherwise}
\end{cases}
\label{eq:hit}
\end{equation}


To simplify this challenging algorithm design task, we make a few assumptions. 
First, we assume that cell values do not have substring hits. 
A cell value must match the entire value of a previously seen cell to count as a hit. 
We also assume that the input list is sorted and at least one tuple (row) can fit into the KV cache to allow reuse. 
\accheng{@shu, what are the implications of these assumptions on performance?}
%\shu{is this enough for justifying just look at previous row and sort?}


\paragraph{Example Query}
% Since cache hits occur only for the request prefixes, determining the right order of columns in SQL queries can significantly impact performance. 
Consider the following query:
\vspace{1pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM("Summarize: ", pr.*) 
FROM (
    SELECT review, rating, description
    FROM reviews r JOIN product p ON r.asin = p.asin
) AS pr
\end{minted}
\end{mdframed} 
\vspace{1pt}

This query sends the columns \textit{review}, \textit{rating}, and \textit{description} from table \textit{pr} to the LLM for summarization. Starting with \textit{review} is inefficient due to its many distinct values, which reduces prefix sharing. Placing \textit{description} first increases shared prefixes, as more reviews link to the same product. Effective reordering must balance prefix frequency and length to optimize cache reuse.


% This query passes in the columns \textit{review}, \textit{rating}, \textit{description}, and \textit{title} for all the rows in table \textit{pr} to the LLM for summarization purposes. Using the default order in which \textit{review} comes first is inefficient because this column has more distinct values, leading to more unique prefixes. Instead, placing the \textit{description} column at the beginning can increase shared prefixes, as many more reviews are associated with the same product. The request reordering task in real datasets is complicated by the diversity in shared prefix values and their variable lengths. For instance, longer shared prefixes might lead to larger PHC, even if they arise less frequently than shorter prefixes. Thus, a reordering strategy must balance prefix frequency and size to maximize cache reuse. 

\paragraph{Our Proposal}
We propose an optimal request ordering algorithm, Optimal Prefix Hit Maximization (\optimal), to maximize PHC. 
Given the exponentially expensive computational cost of the \optimal algorithm,  we also introduce Greedy Group Recursion (\greedy), an approximation of \optimal that leverages functional dependencies and table statistics to reorder requests for large tables efficiently. 

%%%%%%%%%%%%% MLSYS ALGORITHM NEEDS RECONSTURCTION 
% \begin{algorithm}[t!]
% \caption{Optimal Prefix Hit Recursion (OPHR)}
% \begin{algorithmic}[1]
% \STATE \textbf{Input:} Table $T$
% \STATE \textbf{Output:} Prefix Hit Count $S$, Reordered List of Tuples $L$

% % \newcommand{\algorithmicfunction}{\textbf{function}}
% % \newcommand{\algorithmicendfunction}{\algorithmicend\ \algorithmicfunction}

% \FUNCTION{$\textsc{HitCount} (v, c, T)$ }
%     \STATE $R_v \gets \{i \mid T[i,c] = v\}$
%     \STATE {\bfseries Return} ${\text{len}(v)}^2 \times (|R_v| - 1)$
% \ENDFUNCTION

% \item[]
% \FUNCTION{$\textsc{Recurse}$ ($T$)}
%     \IF{$|T|_{rows} = 1$}
%         \STATE return 0, $[T[1]]$
%     \ENDIF 
%     \IF{$|T|_{cols} = 1$}
%         \STATE $S \gets \sum_{v \in \text{distinct}(T[,1])} \textsc{HitCount}(v, 1, T)$ % groupby or sort, choose best group, append 
%         \STATE {\bfseries Return} $S, sort([T[i] \mid i \in 1 \dots |T|_{rows}])$
%     \ENDIF
%     \STATE $max\_phc \gets -1$, $best\_L \gets T$

%     \COMMENT{For each distinct value $v$ in each column $c$}
%     \FOR{$c \in \text{columns}(T)$, $v \in \text{distinct}(T[,c])$} 
%         % \STATE $\text{distinct\_values} \gets \{T[i,c] \mid i \in 1 \dots |T|_{rows}\}$
%         % \FOR{$v \in \text{distinct\_values}$}
%         \STATE $R_v \gets \{i \mid T[i,c] = v\}$
%         \STATE $A\_HC, L_A \gets \textsc{Recurse}(T[\text{rows} \setminus R_v, \text{cols}])$
%         \STATE $B\_HC, L_B \gets \textsc{Recurse}(T[R_v, \text{cols} \setminus \{c\}])$
%         \STATE $C\_HC \gets \textsc{HitCount}(v, c, T)$
%         \STATE $phc \gets A\_HC + B\_HC + C\_HC$
%         \IF{$phc > max\_phc$}
%             \STATE $\max\_phc = phc$, 
%             \STATE $best\_L = [[v] + L_A[i] \mid i \in 1 \dots |R_v|] + L_B$
%         \ENDIF
%     \ENDFOR
%     \STATE $\textbf{return } \text{max\_phc}, \text{best\_L}$
% \ENDFUNCTION

% \STATE 
% \STATE \textbf{return } \textsc{Recurse}($T$)
% \end{algorithmic}
% \label{alg:optimal}
% \end{algorithm}


\begin{algorithm}[t!]
\caption{Greedy Group Recursion (GGR)}
\begin{algorithmic}[1]

\STATE \textbf{Input:} Table $T$, Functional Dependency $FD$
\STATE \textbf{Output:} Prefix Hit Count $S$, Reordered List of Tuples $L$


\item[]
\FUNCTION{$\textsc{HitCount} (v, c, T, FD)$}
    \STATE $R_v \gets \{i \mid T[i,c] = v\}$
    \STATE $\text{inferred\_cols} \gets \{c' \mid (c, c') \in FD\}$
    \STATE $\text{tot\_len} = \text{len}(v)^2 + \sum_{\substack{c' \in \text{inferred\_cols}}} \frac{\sum_{r \in R_v} \text{len}(T[r, c'])}{|R_v|}$
    \STATE \textbf{return } $\text{tot\_len} \times (|R_v| - 1)$, $[c] + \text{inferred\_cols}$
\ENDFUNCTION


\item[]
\FUNCTION{\textsc{MRecurse}($T$, $FD$)}
    \IF{$|T|_{rows} = 1$ or $|T|_{cols} = 1$}
        \STATE \textbf{return } \text{Base case processing as in \optimal}
    \ENDIF

    \STATE $max\_HC, best\_v, best\_c, best\_cols \gets -1, \text{None}, \text{None}, []$

    \FOR{$c \in \text{columns}(T)$, $v \in \text{distinct}(T[,c])$}
        \STATE $HC, cols \gets \textsc{HitCount}(v, c, T, FD)$
        \IF{$HC > max\_HC$}
            \STATE $max\_HC, best\_v, best\_c, best\_cols = HC, v, c, cols$
        \ENDIF
    \ENDFOR
    
    \STATE $R\_v \gets \{i \mid T[i, best\_c] = best\_v\}$
    \STATE $A\_HC, L\_A \gets \textsc{MRecurse}(T[\text{rows} \setminus R\_v, \text{cols}], FD)$
    \STATE $B\_HC, L\_B \gets \textsc{MRecurse}(T[R\_v, \text{cols} \setminus best\_cols], FD)$
    \STATE $C\_HC, \_ \gets \textsc{HitCount}(best\_v, best\_c, T, FD)$
    \STATE $S \gets A\_HC + B\_HC + C\_HC$
    \STATE $L \gets [[best\_v] + L_A[i] \mid i \in 1 \dots |R\_v|] + L\_B$
    \STATE \textbf{return } $S, L$
\ENDFUNCTION

\item[]
\STATE \textbf{return } \textsc{MRecurse}($T$, $FD$)
\end{algorithmic}
\label{alg:greedy}
\end{algorithm}

\subsection{Case Study: Fixed Column Ordering}
Most of the table has some default column orderings applied to all rows. How bad can this be in terms of PHC? 

Imagine a table with a column with all distinct values as the first column, for example, commonly seen ones including timestamp, ID, etc. Assuming each value in the table is of length of 1. In the worst case, assuming all other columns, each column has a single value. In this case, the hit rate difference of optimal ordering (i.e., putting distinct column last) compared with the naive fixed column ordering is 0 versus $(n-1)\times(m-1)$, where the only last column is missed, and the cold miss of the first row.  

Now imagine for example, there are some groups of values in the default ordering, first column, that does have some values. Assume that there are $i$ such groups from $G_1, ..., G_{i}$, each group has $x$ rows where $x < n$. We can always construct a case where if $i == 1$, and each column contains such group with non-overlapping rows compared to the previous or next column, then the PHC of such fixed column orderings is $x - 1$, where $-1$ account for the cold miss of such column. However, an obvious better ordering is to have different column orderings for different set of rows. For example, choosing $G1$ of column $1$ to be first, then for the next set of $x$ rows pick $G3$ of column $2$ to be first. In this case, the hit rate of such ordering will be $m \times (x-1)$. Thus, the ratio of PHCs comparing default orderings and a better orderings will be as high as $m$.  

\subsection{Optimal Prefix Hit Recursion (OPHR) } \label{sec:optimal}

%%%%%%%%%%%%%%%%%% Matei's feedback 
% \shu{need to explain: consider reordering rows but also columns, and doing it differently for each row. Why is it important to do it differently, if you don't add it you'll get $c$ times worse, show some base cases; might be losing accuracy. 

% Motivate: necessary to reorder both rows and columns somewhere (differently across different records), that's the new thing; why is that --> we prove that if you use a fixed column order, can be off by a factor of $c$ by hit rate. Imagine there's a group in each column. 

% Then: now that we know we need to choose different orders even within each row (optimal --> GGR) 

% Don't need to put the algorithm of optimal. Don't need. Example of how it can be off by a factor of c, show the picture. Motivate this. What's the claim (scientific question), obvious cases it does poorly 

% Don't add too many appendix, sglang it is ok to mention it is similar. Queries can be in there. }
%%%%%%%%%%%%%%%%%% Matei's feedback 
Our Optimal Prefix Hit Maximization (\optimal) algorithm is a recursive algorithm that finds the \textit{optimal} PHC for a given table $T$ by considering all possible ways to split the table into a group of cells with the same value and two sub-tables (Algorithm~\ref{alg:optimal}). % It finds the \textit{optimal} PHC for a given table $T$ by assigning column orders for each row (Algorithm~\ref{alg:\optimal}). 
% table layout algorithm, table ordering algorithm 
The algorithm takes as input a table $T$ and computes the optimal PHC $S$ along with a reordered list of tuples $L$. If $T$ only has one row or column, \optimal computes PHC and trivially returns the sorted $T$ (lines 8-14). In the recursive case, for each column $c$ in $T$, the algorithm identifies all distinct values $v$ in this column and the rows $R_v$ for which the column value is $v$. For each distinct value $v$, the table is split into two sub-tables: one of $T$ excluding rows $R_v$ (line 18), and one of $R_v$ excluding column $c$ (line 19). The PHC for the currently selected value $v$ is calculated as the sum of the PHC of the sub-tables and the PHC contribution of $v$ (line 20). The algorithm evaluates all possible groups of distinct values in each column and selects the value that yields the maximum PHC (Figure~\ref{fig:optimal}). 

Unsurprisingly, the \optimal algorithm has exponential complexity with respect to the number of rows and columns due to its recursive nature and the combinatorial explosion of possible distinct value groupings (we present a more efficient algorithm in Sec~\ref{sec:greedy}). 


\begin{figure}
    \vspace{-1em}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/SIGMODfigures/prefix_hit_maximization.pdf}
    \vspace{-1.5em}
    \caption{The \optimal algorithm evaluates each group of distinct values (e.g., v and a) and calculates PHC as the sum of PHC of the elected group values (yellow and red boxes), the sub-table $T$ excluding rows $R_v$, and the sub-table of rows $R_v$ excluding the column where the value is located in (blue and green boxes). \shu{change this graph to include OHPR and GGR illustration}}
    \label{fig:optimal}
\end{figure}


% is this even correct?
% $T(n,m) \leq m \cdot k \cdot T(n-1, m) + T(n, m-1)$  where $k$ is the number of distinct values per column. The worst-case time complexity of \optimal is $O((m \cdot k)^n))$. We now prove the optimality of \optimal. 

% Specifically, for each column, the algorithm considers all distinct values, leading to a time complexity of $O(m \cdot k \cdot T(n-1, m) + T(n, m-1))$ where $k$ is the number of distinct values per column. The worst-case time complexity of \optimal is O((m$\cdot$k)^n))

\paragraph{Optimality Proof}
In the base case, the \optimal algorithm trivially computes the best PHC: for the single row case, the PHC is 0; for the single column case, the PHC is the sum of the squared lengths of distinct values multiplied by their occurrences minus one, which accounts for the initial miss when a value is seen the first time. 
Next, we prove optimality by induction.
For the inductive case, assume that the \optimal algorithm is optimal for any table with $k \leq n$ rows and $l \leq m$ columns. 
For a table $T$ with $n+1$ rows and $m+1$ columns, the algorithm iterates through each column $c$. For each distinct value $v$ in column $c$, we split $T$ into two sub-tables: $T_A$ (rows not containing $v$), and $T_B$ (rows containing $v$ but excluding column $c$). Based on the inductive hypothesis, \optimal optimally computes PHC for both sub-tables because it is optimal for tables with fewer rows and columns. The PHC for $T$ is the sum of PHC for $T_A$ and $T_B$, plus the contribution of $v$. When the distinct value $v$ is used to partition the table, its full contribution to the PHC is captured. If the table were not split based on distinct values, this contribution could be fragmented or lost due to non-contiguous groupings, leading to suboptimal PHC.
Thus, the \optimal algorithm ensures optimal reordering by selecting the best from all possible configurations.


\subsection{Greedy Group Recursion (\greedy) Algorithm}
\label{sec:greedy}
\shu{Add architecture diagrams here? Design of this reordering algorithm similar to: https://arxiv.org/pdf/2311.04934}
Due to the computational complexity of the \optimal algorithm, we propose a Max Group Recursion (\greedy) algorithm (Algorithm~\ref{alg:greedy}) that approximates \optimal.  
The \greedy algorithm takes an input table $T$ and returns the PHC $S$ along with a reordered list of tuples $L$. It has the same base case as the \optimal algorithm if $T$ only has one row or one column. At a high level, the \greedy algorithm recursively selects the value with the maximum prefix hit count (lines 3-8) at each recursion step (lines 13-19) rather than iterating through all possible distinct values in the entire table. It then splits the table into groups of cells of the same values and recurses on two sub-tables (lines 21-23), similar to the \optimal algorithm. 

Since \greedy does not iterate through all possible distinct values but instead selects the one that gives the highest hit count at each step, the number of recursive calls is significantly reduced (i.e. the maximum depth of recursion is $O(min(n,m))$, where the algorithm reduces dimensions of the table at each recursive step). However, at each recursive step, the cost of scanning to determine distinct values can lead to quadratic complexity in terms of table size. 
% \shu{ends with this, is it weird? do we need some transition?} \joey{it might have helped to have table statistics next.}


% Count the total number of splits 
% Each time split: one row 
% Worst case
% Can also do that with stats, but scan 
% 1 column base case, how many total times (table with 2 columns, pick a value from one column, add a basecase); worst case: number of distinct values * how much the scan costs (more columns) 
% lots of distinct values - could be quadratic in the table -> individual step (do this in stats, linear in table size) 

% not have complexity analysis 

% \shu{Still exponential, just that the number of recursive calls reduces to O(m) not m * k?}

% branch and bound, prune the space 
% $T_{\greedy}(n,m) \leq O(m) \cdot T_{\greedy}(n-1, m) + T_{\greedy}(n, m-1)$ 
% Our \greedy algorithm improves the runtime complexity compared to the \optimal algorithm by avoiding the exhaustive search over all possible configurations. \greedy evaluates the hit count for distinct values in each column in each step and selects the best local configuration. Despite this simplification, the \greedy algorithm still faces exponential growth in complexity due to the recursion. \accheng{@shu, seems weird to end with this, is \greedy exponential in the worst case? we should find some way to bound it if so}
% \greedy also leverages functional dependencies and table statistics to improve performance further. We describe each of these techniques in detail below.

% \shu{not optimization, for corretness, avoid having to check each step as long as it captures most of the correlation between columns} 

\subsubsection{Functional Dependencies} We leverage functional dependencies to reduce the number of columns the \greedy algorithm needs to consider at each recursion step. This insight helps improve both the approximation and efficiency of the algorithm, bringing it closer to the optimal solution without the need for extensive backtracking as in the \optimal algorithm. 

A functional dependency (FD) is a constraint between two sets of attributes in a relation from a database. For example, let $R$ be a relation schema and let $X$ and $Y$ be nonempty sets of attributes in $R$. We define an instance $r$ of $R$ that satisfies the $FD$ $X \rightarrow Y$ if for every pair of tuples $t_1$ and $t_2$ in $r$: if $t1.X = t2.X$, then $t1.Y = t2.Y$. As an example, if $R(A,B,C)$ is a table with attributes (columns) $A,B,C$, and an $FD$ of $A \rightarrow C$ means that if two rows have the same value for $A$, then they must have the same value for $C$. In our \greedy algorithm, FDs help narrow down the columns that must be considered at each recursion step. Specifically, when a value $v$ in column $c$ is selected, all columns functionally dependent on 
that column only need to be processed once (lines 5-6). In the example where $A \rightarrow C$, we do not need to separately consider $C$ when $A$ is already included in the prefix, as $C$ will not provide a different PHC.
% are also considered as inferred columns (line 5-6). This means we only need to process these inferred columns once per recursion, which reduces redundant calculations and expedites the process. 
% \shu{Note: our algorithm here seems to ignore the case where you have $AB \rightarrow C$, where you have two rows have same value for $A$ and $B$? but under the assumption where we append columns it might not matter. Also shall we assume transitivity already in our psedocode? i.e. A -> C, C -> B, then FD includes A -> B too.}
% We also include functional dependency in the \greedy algorithm to enhance PHC by including related columns. In database literature, ...

\subsubsection{Table Statistics} To further reduce the algorithm runtime, we introduce an early stopping mechanism that halts recursion when the hit count (line 3) falls below a certain threshold. Additionally, we can further improve the quality of the solution by establishing a fixed column ordering for the subtables using table statistics once the recursion stops. Databases typically maintain statistics on stored data, such as the number of unique entries (i.e., cardinality) and the distribution of length of values for each column. Specifically, our \greedy algorithm estimate a \texttt{HITCOUNT} score for each column $c$ with $HITCOUNT(C) = avg(len(c))^2 \cdot (\frac{n}{cardinality} - 1)$. This score denotes the expected contribution of a column to the PHC, taking into account both the average length of the values and their frequency. Using these statistics, the algorithm can prioritize columns that are more likely to contribute to the PHC. Early termination and falling back to table statistics allows \greedy to avoid scanning the table and performing recursions on realistic workloads. 

% In practice, many datasets have columns with high cardinality (i.e., few shared prefixes), so their order has minimal impact on the cache hit rate.

% \subsubsection{Optimality Analysis}
% \shu{in what case does it match the \optimal? Can we match it} 

\subsubsection{Achieving Optimal PHC} While our \greedy algorithm is an approximation of the \optimal algorithm, there are specific scenarios when the \greedy algorithm can achieve optimal PHC.
% matches the prefix hit count of the \optimal algorithm exactly. 
In the simplest cases where the table has only one row or one column, the \greedy algorithm returns the same outputs as the \optimal algorithm by construction. When functional dependencies are accurate and cover all the columns of a table, the GGR algorithm can also identify the optimal solution. For instance, if there is a column $A$ that functionally determines all other columns, then \greedy algorithm will prioritize groups of values in this column due to the accumulated \texttt{HITCOUNT} score (line 3 in Algorithm~\ref{alg:greedy}), ensuring it can find the optimal reordering by capturing the most significant correlations early on. 
% As an example, if there is a column \textit{movie_year} that functionally determines the column \textit{movie_title}, the \greedy algorithm will prioritize groups of values in \textit{movie_year} ,
% \accheng{@shu, do we have an example of this in one of our benchmarks? would mention here if so}
However, in cases where there is a tie in the \texttt{HITCOUNT} score, the \greedy algorithm might be suboptimal because it lacks the mechanism to resolve ties as effectively as the \optimal algorithm, which explores all possible configurations that could potentially result in higher overall PHC.
% * For FDs which cover all the columns, the \greedy algorithm with functional dependencies will be able to identify the same output as optimal, without needing to even do the backtracking and iterating through all rows, if FDs are correct. 
% * Discuss when there is a tie on max group score, then the greedy algorithm is suboptimal, don't know what to do. 

% Think about some subset of cases where it is, can also think about with a table with just one column, it is okay, table of two columns, condition to be okay. (or independent), no FDs, independent; FD, method capture it (FDs, cover all things). Columns that are not covered by FDs, assumption if those are independently assign or distributed, then what we are doing is okay.

% Tie on the first step, don't find the right answer later, then this doesn't know what to do.

% \subsection{Row-level Reordering}
% Once we determine a column order, we need to group the rows of data such that we maximize the number of shared prefixes across requests. To achieve this, we concatenate all column values into a string and sort these strings lexicographically (over different rows) to determine the row order. 
% Conveniently, the structured nature of SQL queries enables us to efficiently sort requests---we can identify and easily group shared data based on the relational schema by using existing database operations (e.g., \texttt{GROUP BY and ORDER BY}). \shu{Add reasoning why row-ordering works, once we relax the assumption on not infintie cache size}

% \accheng{@shu, is there a reason we don't split this into a separate subsubsection?}
% Additionally, we introduce an early stopping mechanism based on the average values from the table statistics. Specifically, we manually add a early stopping parameter to not considering group with hit count is larger than a particular value \accheng{@shu, unclear what this means}. The algorithm stops the recursion and returns the current result if this parameter is satisfied, saving computational resources.
%while still providing a near-optimal solution.


% \begin{algorithm}[t!]
% \caption{Row-Level Sorting Based on Column Prioritization}

% \begin{algorithmic}[1]
% \STATE \textbf{Input:} Table $T$, Reordered Columns List $L$ from Algorithm 1
% \STATE \textbf{Output:} Reordered Table $T'$
% \item[] 
% \STATE $T' \gets T$ with columns reordered according to $L$ 

% \FOR{$i \gets 0$ to length($L$)$\text{ } - 1$}
%     \STATE $T' \gets stableSort(T', L[i])$ \Comment{Apply stable sort on $T'$ based on column $L[i]$, preserve previous sort orders}
% \ENDFOR


% \STATE \Return $T'$

% \end{algorithmic}
% \end{algorithm}

% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
% SELECT LLM("Summarize the content of this movie: {movie}", m.movieInfo) AS summary 
% FROM Movies m
% \end{minted}
% \end{mdframed} 
% \vspace{8pt}

% \shu{Remove this example, and connect to the previous section}
% In the context of querying LLM with SQL, a common pattern involves passing a specific column from database table as input to the LLM. 
% \begin{itemize}
%     \item For instance, consider a query that summarizes movie contents, where the \texttt{m.movieInfo} column from the \texttt{Movies} table is used to generate summaries. 
%     \item This approach generates content summaries based on detailed movie information stored in the database. 
% \end{itemize}

% \subsection{Row-level Reordering}
% Once we determine a column order, we need to group the rows of data such that we maximize the number of shared prefixes across requests. To achieve this, we concatenate all column values into a string and sort these strings lexicographically (over different rows) to determine the row order. 
% Conveniently, the structured nature of SQL queries enables us to efficiently sort requests---we can identify and easily group shared data based on the relational schema by using existing database operations (e.g., \texttt{GROUP BY and ORDER BY}). \shu{Add reasoning why row-ordering works, once we relax the assumption on not infintie cache size}

% Once we determine a column order, we concatenate all column values into a string and sort these strings lexicographically (over different rows) to determine the row order. 

% % To demonstrate how this technique improves cache usage, 
% Consider an example in which we have a batch size of three and six distinct prefixes that each appear three times. If the requests arrive in the following order (with batches shown in brackets): $[1,2,3],[4,5,6]$ $,[1,2,3],[4,5,6]$, the KV cache would evict and recompute all six prefixes under a caching algorithm, such as FIFO, leading to inefficient cache use. Instead, if we sort the rows of input to group common prefixes together (e.g., $[1,2,3],[1,2,3],[4,5,6],\newline[4,5,6]$), we ensure that each prefix is loaded into the cache only once and reused across any requests it is involved in. Upon eviction, we know that this prefix will never need to be loaded into the cache again. This approach can greatly reduce cache eviction and recomputation, leading to faster LLM processing times.


% with various optimizations that can be applied to real-world tasks .

% say worst case runtime, and say best case runtime too
% \accheng{update this sentence}
% in proximity of one another, thus optimizing the  

% \subsection{Problem Setup}

% % \textbf{LLM Request Structure.} 
% We define the LLM function within the context of SQL queries. In addition to the text of the prompt, this function accepts \emph{set} expressions listing one or more columns $\{T.a, T.b, T.c\}$ or $\{T.*\}$ of table $T$.
% This API design enables us to dynamically reorder fields within these expressions to optimize for cache efficiency. 

% % \textbf{Objective} 
% The goal of request scheduling is to \textbf{maximize} the \textit{prefix hit count} (PHC) by optimizing the order of columns and rows of an input table with $n$ rows and $m$ columns. 
% Note that for each row, there may be a different column order.
% We represent a request schedule as a list of tuples, $L$, where each tuple in $L$ corresponds to a row in the original table, and the tuple elements are the values within the row. The tuple order in the list can be rearranged to represent different row orders, and the order of the elements in each tuple can be rearranged to represent the chosen column order for the row. 
% We pass the list $L$ of input requests along with the desired prefix prompt to the LLM for inference.
% When providing each row as an input request to the LLM, we prepend column names in front of values to indicate the column each value belongs to using a standard JSON encoding.


% % Each tuple in $L$ corresponds to a row, and the elements of the tuple correspond to the values within the columns. 

% We define the PHC of $L$ as the number of consecutive column cell values shared with the previous row starting from the first cell, summing over all rows from $0$ to $n-1$. Each cell value must exactly match the corresponding cell of the previous row (cannot be a substring), and cell values past the first must match consecutively (must be a prefix). 
% % We assume that the previously seen prefix must match the entire value of a previous cell, and cannot be a substring. 
% Formally, a cell in the list of tuples is denoted as $L[r][c]$, indicating the value in tuple $r$ at position $c$. Then, the PHC for a list of tuples $L$ with $n$ rows and $m$ columns is given by: 
% % $\text{PHC}(T) = \sum_{i=0}^{n-1} \max_{1 \leq j \leq m} \textit{hit}(T_{i,j})
% % $. 

% \begin{equation}
% \text{PHC}(L) = \sum_{r=0}^{n-1} \textit{hit}(L, r)
% \label{eq:phc}
% \end{equation}

% Here, the function $\textit{hit}(L, r)$ represents the prefix hit count for a single row $r$ in $L$. For simplicity, we assume that the input list is sorted. For each row $r$, the function checks if the value in each column $t$ matches any previously seen value in the same column of the previous row $r-1$. If all previous columns match, the hit count is the sum of the squares of the lengths of the values in those columns until a mismatch occurs. The squared lengths reflect the quadratic complexity of token processing in LLM inference, where each token computation depends on every preceding token and increases computational cost quadratically with input length. 
% % \shu{make it clear about the Tuple index, tuple has order that represents column ordering; have to sort to make things work, previous rows (overlap), simplify by looking at, assuming at least one row fits into KV cache; n-1 (how much overlap, assume cache is large enough to reuse for previous few rows)}

% % It is defined as the length of the concatenated string of cell values for row $i$ from column $1$ to $j$, if and only if all the concatenated cell values exactly match the previously seen concatenated cell values in the same columns.

% % Defined over all previous rows 
% % \begin{equation}
% % \textit{hit}(L, r) = \max_{0 \leq c < m}
% % \begin{cases} 
% % \sum_{t=0}^{c-1} \text{len}(L[r][t])^2 & \text{if } \FORall t \leq c, L[r][t] = L[x][t] \\
% % & \quad \exists x \text{ s.t., }  0 \leq x < r \\
% % %& \quad \max\left(0, r -q \right) \leq x < r \\
% % 0 & \text{otherwise}
% % \end{cases}
% % \label{eq:hit}
% % \end{equation}

% \begin{equation}
% \textit{hit}(L, r) = \max_{0 \leq c < m}
% \begin{cases} 
% \sum_{t=0}^{c-1} \text{len}(L[r][t])^2 & \text{if } \forall t \leq c, L[r][t] = \\ & L[r-1][t] \\

% %& \quad \max\left(0, r -q \right) \leq x < r \\
% 0 & \text{otherwise}
% \end{cases}
% \label{eq:hit}
% \end{equation}


% To simplify this challenging algorithm design task, we make a few assumptions. 
% First, we assume that cell values do not have substring hits. 
% A cell value must match the entire value of a previously seen cell to count as a hit. 
% We also assume that the input list is sorted and at least one tuple (row) can fit into the KV cache to allow reuse. 
% \accheng{@shu, what are the implications of these assumptions on performance?}
% %\shu{is this enough for justifying just look at previous row and sort?}


% \paragraph{Example Query}
% % Since cache hits occur only for the request prefixes, determining the right order of columns in SQL queries can significantly impact performance. 
% Consider the following query:
% \vspace{1pt}
% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
% SELECT LLM("Summarize: ", pr.*) 
% FROM (
%     SELECT review, rating, description
%     FROM reviews r JOIN product p ON r.asin = p.asin
% ) AS pr
% \end{minted}
% \end{mdframed} 
% \vspace{1pt}

% This query sends the columns \textit{review}, \textit{rating}, and \textit{description} from table \textit{pr} to the LLM for summarization. Starting with \textit{review} is inefficient due to its many distinct values, which reduces prefix sharing. Placing \textit{description} first increases shared prefixes, as more reviews link to the same product. Effective reordering must balance prefix frequency and length to optimize cache reuse.


% % This query passes in the columns \textit{review}, \textit{rating}, \textit{description}, and \textit{title} for all the rows in table \textit{pr} to the LLM for summarization purposes. Using the default order in which \textit{review} comes first is inefficient because this column has more distinct values, leading to more unique prefixes. Instead, placing the \textit{description} column at the beginning can increase shared prefixes, as many more reviews are associated with the same product. The request reordering task in real datasets is complicated by the diversity in shared prefix values and their variable lengths. For instance, longer shared prefixes might lead to larger PHC, even if they arise less frequently than shorter prefixes. Thus, a reordering strategy must balance prefix frequency and size to maximize cache reuse. 

% \paragraph{Our Proposal}
% We propose an optimal request ordering algorithm, Optimal Prefix Hit Maximization (\optimal), to maximize PHC. 
% Given the exponentially expensive computational cost of the \optimal algorithm,  we also introduce Greedy Group Recursion (\greedy), an approximation of \optimal that leverages functional dependencies and table statistics to reorder requests for large tables efficiently. 


==> sections/0_abstract.tex <==
\begin{abstract}
% \accheng{needs to be updated}

% V3: ...
Analytical database providers (e.g., Redshift, Databricks, BigQuery) have rapidly added support for invoking Large Language Models (LLMs) through native user-defined functions (UDFs) to help users perform natural language tasks, such as classification, entity extraction, and translation, inside analytical workloads.
However, LLM inference is highly expensive in both computational and economic terms: for example, an NVIDIA L4 GPU running Llama3-8B can only process 6 KB of text per second.  
In this paper, we explore how to optimize LLM inference for analytical workloads that invoke these models within relational queries.  
We show that relational queries present novel opportunities for accelerating inference. These include reordering rows and columns to maximize key-value (KV) cache reuse and other standard techniques such as deduplication and SQL optimizations.  
We implement these optimizations in Apache Spark, with vLLM as the model-serving backend, and achieve up to 5.7$\times$ improvement in end-to-end latency on a benchmark of diverse LLM-based queries on real datasets. 
To the best of our knowledge, this is the first work to explicitly address the problem of optimizing LLM invocations within SQL queries. 

% L4 7B 2000 toks/s on prefill dominate workload.  800 toks/s on decode dominate workload. 1 tok is 4 bytes. Balancing this give us about 1500 toks/s -> 6000 bytes/s.

% \simon{maybe something like: To the best of our knowledge, this is the first work applying properties in LLM inference technologies in optimizing SQL queries.}


% V2: ...
% LLMs have seen increasing adoption in a wide range of fields. However, LLM inference is very computationally expensive: [stat and citation].
% In this paper, we focus on applying LLMs for batch analytical tasks in the context of SQL queries. For instance, an application might want to process millions of records from a products reviews database to deduce user sentiment. To optimize for LLM invocations via SQL, we leverage the workload information from queries to maximize memory usage of LLMs. Specifically, we introduce a reordering algorithm that groups requests with shared input prompts, or prefixes, together. 
% With these optimizations, we see up to 4.3$\times$ improvement in end-to-end latency. 

% V1:...
% There’s been a lot of work to build a real-time LLM application stack, including chains, vector DBs for retrieving items, etc. However, it’s also useful to apply LLMs in batch analytics tasks, such as processing millions of records in a database to figure out what a user’s sentiment is, which products reviews tend to mention, etc. How can LLMs and retrieval be used most efficiently in this context? For example, it might make sense to deduplicate records or group similar records before passing them to an LLM to minimize inference times, or to replace “point lookups” into a vector DB with some kind of efficient vector similarity join. Any work on this problem would also be useful to teams seeking to train or evaluate their LLM pipelines more efficiently on large datasets.
\end{abstract}

==> sections/1_1_outline.tex <==
\section{Outline}
\shu{Background and LLM inference (section 2), section 3 is problem setup and opportunities, this create 4-5 opportunities that we didn't have in classical stuff}
% \subsection*{Section 1: Introduction}
% \newline 
% \shu{Following my outline} \\
% \textbf{LLM is important}


% \subsection*{Section 2: Problem Setup}



% \shu{Backgrounds / problem setup: just background on LLM and inference, separately have a section on the optimization opportunities for batch anlaytics workloads, bring in the past LLM stuff, different from online setting where you just get the call from users, list format}

% \section{Introduction}
% Put one example into Introduction 
% \section{Background: LLM and stuff}
% Reference: 

% \subsection{Opportunities}
% Challenges and opportunities, also talk about goals and our approach 
% would require new offline optimizations to LLM inference (we could batch similar length prompts) and potentially run on cheaper hardware.  The query planner should also probably be aware of the monetary costs associated with LLM invocations.  

% One can imagine having a simple SQL UDF for LLM invocation as well as system optimizations to invoke the LLM and improve query planning for expensive UDFs. One can also frame the standard RAG paradigm as an SQL expression.

% Two key insights grounded the basis of the optimizations we looked into:

% \textbf{(1) Adapt the LLM to the queries we know it will process (Do work faster).}
% The advantage of batch analysis settings is that we have knowledge beforehand of the requests sent into the LLM for processing. We can make use of this while deciding our model-side optimizations. 

% \textbf{(2) Do less work.}
% First, LLM invocations are expensive, and it is critical to reduce these invocations as data is processed during batch analytic

% \shu{What is interesting about the problem, and what are the opportunities}

% \accheng{start from: decades of ML in DB (MADLib, MauveDB)

% long history of bringing ML into DB

% However, much of this work has focused on how to incorporate training into a DB system

% MADLib for training
% Query engine is used in the training pipeline, data clustering

% DB2 (MPI): how to distributed training in the DB
% SystemML (IBM): distributed training

% Velox (CIDR): all ML in DB is training, should be inference

% Rich history in training
% LLM setting changes to in-context learning and inference

% Specifically, we take advantage of unique properties of LLMs

% Expensive UDF BUT with structure

% Not scans over data from training but calling function over data

% 2. LLMs are expensive but there is structure

% Need to explain decoder architecture briefly

% Work: Paged Attention for problem structure

% What the SotA LLMs do (published)
% Attention kernel
% }

% \shu{Exploit LLM structure for query optimization: inference time (bigger blocks), tuning the page size for page attention, you know what's coming up (workload shaping for lLM), collapsing into single; knowing the workload, tune page size, replacement (eviction)}

% \shu{
% Workload shaping 
% 1. Record level / row level reordering 
% 2. Token dedup of some flavors (pick one) 

% Shape the workloads, schedule the inference 
% 1. Tuning the paging 
% 2. Eviction strategy (follow reorder is optimal, continuous batching w/ static prefix pool)
% }
% \accheng{
% Methodology:
% General optimization as a strength, can apply techniques on more than 1 system

% No system

% Fundamental story: cache reuse for token, record, row level --> main insight

% Transform workload for cache reuse
% 3.2: input-level cache reuse

% How to exploit LLM structure for query optimization
% }

% \shu{Unique properties in LLM (prefix sharing, and semantic / exact dedup, immediately saying that LLM has new kind of model that has structured at inference that where we can use for optimization; expensive UDF (but this is about the structure; system ML - transformer..; exploit the structure of these models for query optimizations; optimizations is okay}

% \textbf{Insights}
% \begin{enumerate}
%     \item Lots of sharing patterns: prefix cache sharing 
%     \item Lots of duplicate (variations) to the same entity 
%     \item Order of execution matters 
% \end{enumerate}
% \textbf{Example Query: RAG}
% Show example of a single RAG query to see how these three dimensions can apply. 

% \subsection*{Section 3: Our Solution}
% \textbf{3.1 Prefix Cache for Batch}
% This can include 
% \begin{enumerate}
%     \item Workload shaping for cache-awareness (row and record level) 
%     \item Workload-aware eviction strategies 
% \end{enumerate}
% \textbf{3.2 SQL Optimizations}
% \begin{enumerate}
%     \item Order of filtering
%     \item Orders of joins 
% \end{enumerate}
% \textbf{3.3 De-duplication}
% \begin{enumerate}
%     \item Exact de-duplication: do a duplicate studies on datasets 
%     \item Semantic de-duplication with hard rules: show some simple entity resolution examples 
% \end{enumerate}
% \subsection*{Section 4: System Architecture}
% \textbf{4.1 LLM engine}
% Implement as part of the vllm 
% \textbf{4.2 SQL engine: PySpark}
% Implement this as PySpark UDF 
% \subsection*{Section 5: Evaluation}
% \textbf{5.1 Types of Queries}
% \begin{enumerate}
%     \item Retriever: structured and unstructured data 
%     \item Pipeline: single-hop, multi-hop 
%     \item SQL types: selection, projection, join 
% \end{enumerate}
% \textbf{5.2 Ablation Study}
% \begin{enumerate}
%     \item SQL optimization effect 
%     \item Prefix cache effect 
%     \item Deduplication effect 
% \end{enumerate}
% \textbf{5.3 System Comparisons}
% \begin{enumerate}
%     \item Compare with vllm naive implementation 
%     \item Compare with SGLang online cache strategies
% \end{enumerate}
% \subsection*{Section 6: Related Work}
% \begin{enumerate}
%     \item SQL optimizations 
%     \item LLM inference: more of an online setup 
% \end{enumerate}


% \textbf{Background Setup}
% % \shu{maybe not RAG; but can work for LLM as well, don't make it; optimziing queries that include LLM, try to claim a bigger contributions; maybe not many backgrounds; but focus more on the contributions and evals (how to do this well)}
% % \shu{UDF? how to frame it with LLM / vector DB; DB papers on the UDF optimizations? }
% % \shu{SQL queries, new functions, can be built in functions in the query (easy-to-understand from the user standpoint); it is useful to use LLM in this context, describe a few potential use cases; challenge: LLM is expensive, retrieval is not cheap either, opportunities to optimize (semantic deduplication, prefix stuff), up to X amount of speedup; use LLM in the SQL context, but these things are very expensive, doing this naively is bad, this paper we explore them, and apply them in reallistic context}

% \shu{Having query at the beginning of the paper, query can demonstrate things; analytics queries are different; sentiment analysis: sentiment, concepts, QA, name extraction}
% \begin{enumerate}
%     \item RAG: LLM and retrieval are widely used \shu{LLM and offline analytics (better way to frame the work)}
%     \begin{enumerate}
%         \item In RAG, data is loaded and prepared for queries or "indexed"
%         \item User queries act on the index, which filters down the data to the most relvant context 
%         \item This context and the query then go to LLM along with the prompt, and LLM provides a response 
%     \end{enumerate}
%     \item RAG pipeline can be arbitrarily constructed 
%     \begin{enumerate}
%         \item Retriever: structured, semi-structured, and unstructured data 
%         \item LLM: can be of different types 
%         \item Orders of execution: single hop, multi-hop (chains of execution)
%         \item Example: Llamaindex \cite{https://docs.llamaindex.ai/en/latest/getting_started/concepts.html}, Langchain \cite{https://python.langchain.com/docs/use_cases/question_answering/} (e.g. RAG with agents)
%     \end{enumerate}
%     \item Use cases 
%     \begin{enumerate}
%         \item Chat applications 
%         \item Question Answering 
%     \end{enumerate}
% \end{enumerate}
% \shu{Talk about more about query optimizations, or optimizing queries that use LLM and retriever (otherwise sounds like building batch analytics)}
% \textbf{LLM and Retrieval in Batch Analaytics Context}
% \begin{enumerate}
%     \item Batch workloads: processing of data that is generated or collected in batches over a period
%     \item LLM and Retrieval is becoming more relevant for batch analytics workloads 
%     \begin{enumerate}
%         \item Retrieval: retrievers can connect to data of any types
%         \item LLMs: useful in interpreting large sets of textual data, extracting insights, or even automating certain decision-making processes based on the analyzed data
%     \end{enumerate}
% \end{enumerate}
% \textbf{New Challenge}
% \begin{enumerate}
%     \item Traditional: most systems today deals with online inference (e.g. vLLM) \shu{Not what we work on; not change the serving systems that much; FlexGen: limited devices, batch inference, but that's not what we are doing}\cite{https://mlinproduction.com/batch-inference-vs-online-inference/}
%     \begin{enumerate}
%         \item Retrieve and response in real time upon request 
%         \item Response are generated on a single observation on data at runtime 
%     \end{enumerate}
%     \item \shu{What are other systems we should compare ourselves against? From the perspective of the DB, naively running this is wasteful and expensive}
%     \item Our setup: batch inference 
%     \begin{enumerate}
%     \item Generate response on a batch of data
%     \begin{enumerate}
%         \item Data: not processed in real-time, but at scheduled intervals or after accumulating a certain amount of data 
%         \item Batch processing tasks: handle large volumes of data all at once
%         \item Optionally cache or store the results for easy retrieval later on when needed
%     \end{enumerate}
%     \item Challenge: naive execution on the pipeline leads to exploding execution time
%     \begin{enumerate}
%         \item Huge amount of data: e.g. tables of millions of rows 
%         \item LLM and Retriever execution is way too expensive, computationally and monetary, when handling data at scale 
%         \item One or two motivation figures showing the breakdown on diverse range of workloads \shu{Maybe not here, but later can put it there; obvious opportunities; degree of the cost estimation (it is not blackbox), cost tricks; showing that there is an opportunities; cardinality estimation; constraints in output (data types and domains), type returns (returned type is string or force)}
%     \end{enumerate}
%     \end{enumerate}
% \end{enumerate}
% \textbf{Insights}
%  Offline inference gives us better understanding on the data and compute
%  \shu{Cost estimate (support cost for UDF), fit it into the frameworks; 2 LLM (GPT 3.5 and GPT 4, and 3.5 is cheaper), shouldn't always do it last; a way to put it with other things; right thing todo, and we are not missing something}
% \begin{enumerate}
%     \item Compute insights
%     \begin{enumerate}
%         \item Given logical operators (e.g. selection, projection, and UDF)
%         \item Construct the best physical execution plan with ordering  
%         \item Goal: input as few as possible data into expensive UDF 
%     \end{enumerate}
%     \item Data insights 
%     \begin{enumerate}
%         \item Lots of duplicates 
%         \item Lots of shared data (e.g. prompt, shared prefix columns) 
%         \item Goal: input fewer data, and speed up processing speed of LLM UDF 
%     \end{enumerate}
% \end{enumerate}

% \textbf{New Solution}
%     \begin{enumerate}
%         \item Unified SQL abstraction 
%         \begin{enumerate}
%             \item Being able to describe standard RAG paradigm 
%         \end{enumerate}
%         \item Batch optimizations 
%     \begin{enumerate}
%         \item SQL optimizations: reordering and smarter constructions on the RAG physical execution plans 
%         \shu{pyspark: easier way to do this? write an optimizer generically look at UDF cost (Fit into some principal frameworks it should be good), don't spend too much time on this, too obvious; focus on things unique to the language model}
%         \item De-duplication: when to deduplicate, and how (e.g. semnatic, exact) \shu{Semantic one can add more depth: running this threshold on data put into the same cluster, identify datasets where this is actually happening (datasets, and algorithms); measure the accuracy, deduplication (formatting, captial letters, and some other ways to get certain guarantees, get some actual data; and see how much it helps), use embeddings to cluster sutff, have a rule (people's names, M jackson, Michael jackson, hard rules what actually counts as deduplicated), grouping and hard rules, idea is good but details can be its own paper, confirming and filtering; this is a performance optimizations, saving time, define this (up to capitalization, or something that the users understand and check mistakes)}
%         \item LLM internal batch optimizations: KV cache \shu{Reorder can be expensive, the cost of LLM (ideally known), maybe cheaper to run on unordered stuff; should we sort or not (experiments on sorting v.s model), to show the systems can decide do something and not to do something; reviewers might ask what if the models are cheap and sorting is expensive} \shu{Dictionary compression: tells you what the prefixes are; today database; maximize prefix for efficient LLM inference; physical operator (merge join and hash join, etc.); LLM is benefiting from sort order, so you know that ... if you don't use for LLM (interesting order, injected from merge and sort join), order sensitivity; interesting orders of LLM}
%     \end{enumerate}
% \end{enumerate}

% \shu{Cover settings that are within this optimizations, is there an opportunity for semnatic deduplications for the workloads, are there anything smart to do with the batching; characteristics }
% \subsection*{Milestones and Plans}
% \begin{enumerate}
%     \item Goal: Feb 1 (VLDB), approximate timeline is around 1.5 months (6 weeks)
%     \item Next week (Dec 20)
%     \begin{enumerate}
%         \item Creation on all workloads (benchmark and testing scripts) 
%         \begin{enumerate}
%             \item 2-3 Datasets 
%             \item 5-6 different query types for each, with tunable parameters as follows 
%             \begin{enumerate}
%                 \item Operators: selection, join, projection 
%                 \item Data retrieved: change the selectivity 
%                 \item Pipeline construct: orders of pipeline, multi-hop 
%             \end{enumerate}
%         \end{enumerate}
%     \end{enumerate}
% \end{enumerate}

% \shu{Database has a large fraction of raw text (e.g. Snowflake), LLM provides a new way to process these data. Here is how you might use LLM in SQL query to make sense on the text. What is the challenges of doing that (running the LLM call is expensive, talk about how LLM works, sequential decoding, each token depends on the previous one, so has to fit in memory the whole time), existing systems optimized for online setting, but in SQL we have full control on the workloads. How to shape the data to be as cost-effective as possible. And state the problem. These patterns look like something in prior works, etc. Prior works have look at dataflow workflows, ML for systems; LLMs are different, inherent sequential nature, trade-offs of memory and GPU utilization are different than prior works (auto-regressive nature, in order to use GPU needs lots of things to be done at once); smaller GPU: throughput lower, etc. For problem setup, picture might be good. vLLM talk (for figure references)}

==> sections/1_introduction.tex <==
\section{Introduction}
Large Language Models (LLMs) are changing the landscape of textual data analysis.
% making it dramatically easier to analyze textual data. 
In fact, a number of analytical database vendors, including AWS Redshift~\cite{aws-redshift-llm}, Databricks~\cite{databricks-ai-functions}, and Google BigQuery~\cite{google-bigquery-llm}, have already added LLM invocation functions to their SQL APIs. \shu{Matei: any user data to add here? Shall we remove this example}
As an example, consider the following SQL query: 

\vspace{4pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT user_id, request, support_response, 
  LLM('Did {support_response} address {request}?', support_response, request) AS success
FROM customer_tickets 
WHERE support_response <> NULL
\end{minted}
\end{mdframed}
\vspace{4pt}
where the LLM is invoked to analyze whether the customer service requests are effectively addressed.
Increasingly, analysts wish to leverage LLMs in such queries for tasks, including classification, entity extraction, summarization, and translation~\cite{databricks-ai-functions}. Going forward, we will refer to SQL queries that invoke LLMs as \textit{LLM queries}.

Unfortunately, applying LLMs this way to real-world datasets (which can contain millions of rows) has significant computational and economic costs. 
For example, question answering with 22K facts from Fact Extraction and VERification (FEVER) dataset~\cite{fever} takes 30 minutes on an NVIDIA L4 GPU instance with a Llama3-8B model~\cite{llama2}. Using OpenAI GPT-4o model, running a query over this single table along takes \$70. 
% For example, classifying the sentiment of 15K user reviews from Amazon Product Recommendation dataset~\cite{amazon-product-review-dataset} takes 30 minutes on an NVIDIA L4 GPU instance with a Llama3-8B model~\cite{llama2}. 

% Unfortunately, applying LLMs this way to real-world datasets (which can contain millions of rows) has significant computational and economic costs. 
% For example, classifying 15K rows of user reviews from Amazon Product Recommendation dataset~\cite{amazon-product-review-dataset} takes 30 minutes on an NVIDIA L4 GPU instance with a Llama3-8B model~\cite{llama2}. 
% On a similar sized instance, an analytical database, such as DuckDB~\cite{duckdb}, can process more than 100GB of data per second in the TPC-DS benchmark~\cite{duckdb-tpcds-benchmark}. 
% Processing the equivalent amount of data via the same LLM would take 96 days, more than 8 million times longer! Thus, minimizing the cost of LLM invocations is the critical objective for LLM queries. 
% Later in this paper, we demonstrate novel optimizations that can reduce LLM runtime by 5$\times$. 


There has been growing research on how to optimize this process. 
Notably, OpenAI, Anthropic, and the other model serving platform has deployed Prompt Caching~\cite{openai-pricing,vllm,cascade-inference,hydragen} \shu{cite anthropic and prompt cache paper}. This technique involves caching the attention states of commonly revisited prompt segments in key-value (KV) cache in memory~\cite{attention-is-all-you-need}, allowing for efficient reuse whenever similar segments of prompts reappear, which helps minimize latency. Reusing prefixes in the cache has also been shown to have an outsized impact on performance~\cite{sglang}. Accordingly, existing inference systems aim to maximize prefix hits in the KV cache to reduce LLM request time and monetary costs.

% At a high level, the output of each query is generated sequentially, as each output token depends on all previous tokens. To improve throughput, modern LLM serving engines batch multiple requests to process them in parallel.
% However, this requires storing all requests in a batch in memory while they are being processed. 
% As a result, efficient memory management is critical for LLM inference performance. LLM inference engines store intermediate states for past prompts and generations, or \textit{prefixes} of these requests, in a key-value (KV) cache~\cite{attention-is-all-you-need,vllm}. Reusing prefixes (e.g., between requests that share the same prompt) in the cache has been shown to have an outsized impact on performance~\cite{sglang,vllm,cascade-inference,hydragen}. Accordingly, existing inference systems aim to maximize prefix hits in the KV cache.

Existing LLM inference systems~\cite{vllm,sglang} are mostly optimized for online serving workloads---they process requests as soon as they arrive, typically in a first-in, first-out (FIFO) order, to minimize the latency. Thus, they miss out on opportunities to improve performance by potentially re-ordering requests to take advantage of the offline analytical workload information. 

In this work, we address the problem of optimizing inference for LLM queries. We introduce various techniques that reduce end-to-end query latency, dominated LLM request latency. To optimize for relational queries using LLMs, we propose dynamic \textbf{request reordering} at the row and column granularity to improve the KV cache hit rate. Our key insight is that, with oracular knowledge of all requests to be sent to the LLM, we can reorder both the requests and the fields inside each request to increase the number of cache hits. For instance, two requests that share the same prefix (which may be non-consecutive under FIFO ordering) should be passed to the LLM together so that the latter can experience a cache hit. 
Likewise, in requests that input multiple fields of data (e.g., a product name and review) into the LLM, the fields should be ordered to maximize the number of shared prefixes.
In real datasets, there can be many shared prefixes across both columns and rows of data, so changing the order and format of requests will markedly increase the prefix KV cache hit rate.


However, finding the optimal order and format of requests is challenging because there are an exponential number of ways to order the columns and rows of data in a query. For example, for a table with $n$ rows and $m$ columns, there are $n \times m!$ possible orderings. First, we introduce an optimal algorithm, \textbf{Optimal Prefix Hit Recursion (\optimal)}, which maximizes the prefix hit rate by recursively dividing the table in optimal subtables. However, \optimal is impractical for large datasets due to its exponential complexity. To approximate the optimal solution efficiently, we present the \textbf{Greedy Group Recursion (\greedy)} algorithm. Our key insight is to leverage functional dependencies and table statistics to approximate the optimal solution efficiently. In particular, we use functional dependencies to identify which fields will be correlated early in the recursive algorithm, thereby reducing the need for backtracking. %if we decide on the ordering early 
This way, \greedy narrows down the columns it needs to process at each step, reducing runtime while providing close-to-optimal performance. In addition, \greedy also leverages table statistics, such as the frequency and size of values, to approximate column order priority. 


% In addition to our request reordering techniques, we present two optimizations to further reduce the computational costs of LLMs in relational queries. First, we observe that many real-world workloads have duplicates in textual data that lead to redundant LLM invocations. With deduplication, we can minimize the number of LLM calls without affecting the accuracy of the overall query. 
% Second, we estimate LLM operator costs within query expressions. This optimization allows for the strategic reordering of operations by considering the significant expense associated with LLM operators. 


We implement our techniques in Apache Spark~\cite{spark-sql} with vLLM~\cite{vllm} and SGLang~\cite{sglang} as the model serving backend. 
Given the lack of standard workloads in this area, we build a diverse benchmark suite of LLM queries on multiple real-world datasets. We construct a wide range of query types, such as selection, projection, multi-LLM invocations, and retrieval-augmented generation (RAG)~\cite{retrieval-augmented-generation} queries, across a variety of recommendation and question-answering datasets, including Amazon Product Review \cite{amazon-product-review-dataset}, the Rotten Tomatoes Movie Dataset \cite{rotten-tomatoes-movies-dataset}, the Stanford Question Answering Dataset (SQuAD), and the FEVER Dataset \cite{squad-dataset}. We find that our techniques provide 2.1 -- 5.7$\times$ improvements in end-to-end query latency while preserving query semantics. In summary, our contributions are as follows: 
% \vspace{-1.6em}
\begin{itemize}
    \item We identify significant opportunities to speed up LLM queries through reordering rows and columns.
    \item We present an optimal algorithm (\optimal) that maximizes prefix sharing but with exponential complexity. We propose a greedy algorithm (\greedy) that approximates \optimal by leveraging functional dependencies and table statistics for efficiency.
    \item We present a set of LLM query benchmarks using real-world data to represent a range of retrieval and processing tasks. Our evaluation using vLLM and SGLang shows up to a 5.7$\times$ speedup in end-to-end query latency compared to naive baselines.
\end{itemize}


==> sections/2_background.tex <==
\section{Background and Motivation}

% \accheng{change to not say only offline, FIFO but there should be some info we use}
% \shu{to be fixed}
% LLMs are a powerful tool for programmatic analysis of text data and are being rapidly incorporated into major analytical DBMSes~\cite{google-bigquery-llm,aws-redshift-llm,databricks-ai-functions}.
% LLM inference has several unique characteristics that have significant implications for performance. 
This section provides a brief overview of the inference process and the key components of the LLM architecture.
%to provide context. 
% We then present opportunities to improve performance for relational analytics.
% While there is prior work on improving model serving with data systems~\cite{velox}, these do not focus on LLMs. In particular, this research does not address impact of data dependencies between requests and also does not optimize for the tradeoff between memory and compute present in LLMs.

\textbf{LLM inference.} 
% LLMs have seen growing usage in a range of application to comprehend and generate text. 
LLMs are made up of autoregressive Transformer models~\cite{attention-is-all-you-need}, which generate words as tokens, one at a time, until a termination token is generated or a token limit is reached. The inference process for LLMs occurs in two stages: (i) the prefill stage, in which the model processes all the input prompts at once, and (ii) the decoding stage, during which output generation occurs. 
Generation for each request proceeds sequentially since the process depends on (the product of the conditional probabilities of) all previous tokens. 
% Generation for each request proceeds sequentially (i.e., new tokens must be generated one by one) since the process depends on (the product of the conditional probabilities of) all previous tokens.
% This process continues until the model outputs a termination token. 
% LLMs are made up of autoregressive Transformer models~\cite{attention-is-all-you-need}, which generate words as tokens, one at a time, based on a given prompt and the existing sequence of tokens that have already been outputted. A \textit{token} is a concise representation, typically Byte-Paired Encoding \cite{byte-pair-encoding}, of a chunk of characters.

An LLM inference engine (e.g., vLLM \cite{vllm}, TGI \cite{tgi}, TensorRT-LLM \cite{trt-llm}) runs the transformer models and schedules the prefill and decode stages. The LLM inference engine batches multiple requests continuously \cite{orca-continous-batching} together to improve throughput. 
During the inference process, the intermediate computed state for all tokens involved is stored in memory.
This token state is cached as key and value vectors in the \textit{key-value (KV) cache}. Each token can take up to 800KB for a 13B Model \cite{vllm}, so an average request (involving 2,000 tokens) can take up to 1.6 GB of space. Furthermore, even with batching (for online workloads, batch sizes of up to 32 requests are used~\cite{orca-continous-batching}), LLM inference is computationally expensive and is currently limited to a processing speed of ~2,000 tokens/s on a single GPU. 
As such, LLM performance is currently the bottleneck in many analytical tasks.

% \joey{Don't forget to fill in [X]}

% \accheng{
% - what is a token? abstraction for string 
% - how to convert token to KV? tokens need to be computed b/c they in the attention step}


% \accheng{kv vecs are by-product

% since the new tokens are conditioned on the old tokens, you need to store the old ones in cache (an some computation is already done on them)
% }
\vspace{-0.5em}
\textbf{Prompt KV cache.}
A crucial factor for LLM serving throughput is memory management within the KV cache.
% Consequently, managing memory usage in the KV cache is crucial for LLM serving throughput. 
% This cache has several unique characteristics: it can dynamically grow and shrink over time as the model generates new tokens, and its lifetime and size are not known a priori. 
To enable maximum cache utilization (i.e., hit rate), recent work proposes sharing tokens across requests. Since many user prompts share the same \textit{prefix}, or input prompt, the KV cache can store one copy of the prefix in advance to reduce redundant computation during the prefill phase. For instance, if two requests share a prefix, the first request will have already performed some computation on the input tokens and loaded these results in the KV cache. The subsequent request can directly reuse these values for further inference without having to recompute the shared tokens. 

% An example of prefix sharing across requests to enhance KV cache efficiency is shown in Figure~\ref{fig:simple-sharing}. Reqs 2 and 3 share some prefix tokens with Req 1.
% \accheng{if not in cache, need to recompute KV for tokens}

% Existing research confirms that effective KV cache management is critical to end-to-end latency and throughput \cite{vllm, sglang}. 
% focuses only on online inference in which the LLM assumes no knowledge about future requests \cite{vllm}.
\vspace{-0.5em}
% \subsection{Optimization Opportunities in Analytics}
% \shu{this needs to be fixed - ignore now}
% In this paper, we optimize LLM inference in the context of relational analytics. We describe new opportunities to improve performance by utilizing the structure and semantics of SQL workloads. \shu{this sounds repetitive}

\textbf{Improving KV cache hit rate}.
% Existing LLM online inference engines make no assumptions about future requests and execute queries as they arrive, or first-in, first-out (FIFO) order. As a result, they miss out on opportunities to improve cache hit rate by leveraging the workload information present in relational analytics.
For data analytics, we observe particularly high opportunities for \textit{prefix KV cache} sharing. 
Given information about the structure and data of the full set of requests and, critically, the ability to rearrange the requests before execution, requests can be arranged to maximize prefix KV cache reuse during inference. 
% For instance, two requests that share a prefix may execute non-consecutively in the original data ordering, and both would lead to cache misses. Instead, if we ordered these requests together, we could ensure that the latter results in a cache hit. 
% Since all prefixes are known in batch queries, we can group shared prefixes together to increase the KV cache hit rate.
Overall, we want to maximize the \textit{prefix hit count}, or the sum of the length of prefixes that can be shared in the KV cache. 


\textit{Our Approach: Request Reordering.} We leverage workload information to enhance the KV cache hit rate. Specifically, we introduce algorithms that reorder requests and fields within each request to maximize prefix sharing across requests and enable efficient memory usage. Our algorithm leverages functional dependencies and table statistics to reduce runtime while finding near-optimal orderings that maximize prefix hit count.

%

==> sections/3_1_old_col_reordering.tex <==
\subsection{Column Reordering}
\label{sec:column-reordering}
Since cache hits occur only for the prefix of requests, determining the right order of columns in SQL queries can have a significant impact on performance. For example, consider the following query: 
% Many SQL queries access data over multiple columns, and In database applications, queries involving multiple columns as inputs to an LLM have become increasingly common (\cite{}).

\vspace{5pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
    SELECT 
        LLM("Give an overview based on this: ", pr.*) 
    FROM 
        (SELECT 
                r.reviewText,
                r.reviewerName, 
                p.description, 
                p.title, 
             FROM reviews r
             JOIN product p ON r.asin = p.asin
         ) AS pr
\end{minted}
\end{mdframed} 
\vspace{4pt}
This query passes in multiple columns, such as \textit{reviewText}, \textit{reviewerName}, and \textit{description}, for each row of data sent to the LLM for summarization. Using the default column order (e.g., \textit{reviewText} happens to be first in the schema) can be inefficient because there are more distinct values in this column, leading to more unique prefixes. Instead, we can place the \textit{description} column first to increase the number of shared prefixes: since many reviews are associated with the same product, these prefixes can be cached and reused. 


% \begin{enumerate}
%     \item This query involves passing in rows with multiple columns, including \textit{reviewText}, \textit{reviewerName},  \textit{description}, and \textit{title}, to an LLM for summarization.
%     \item Naively using the default column order (e.g., \textit{reviewText} is first) can be inefficient because values in this column are more likely to be distinct, leading to more unique prefixes.
%     \item Instead, we can place the \textit{description} column first to increase the number of shared prefixes: since many reviews are associated with the same product, these prefixes can be cached and reused. 
% \end{enumerate} increase the likelihood  of shared prefixes across requests to enhance cache reuse and reduce computational overhead. 
  
% \accheng{Do we use term "cache hit rate"? cache hit?}
% \accheng{need consistent naming for techniques} \accheng{size of shared prefixes right? token hit ratio}

\paragraph{Objective} The objective of column level input reordering is to order fields within requests such that we maximize the prefix token hit rate of the KV cache.
This task is complicated by the diversity in shared prefix values and their variable lengths. For instance, longer shared prefixes might lead to more token hits even if they arise less frequently than shorter prefixes. Thus, a reordering strategy needs balance between prefix frequency and size to maximize cache reuse.

% \accheng{we need to explain where the computation work comes from} 
% \begin{enumerate}
%     \item longer shared prefixes might save more computational work by putting them first even if they are less common, compared to shorter ones that are common.
%     \item Thus, our reordering strategy needs to balance the commonality of data and the potential length of shared prefixes, which directly impacts computational savings during the LLM inference process. 
% \end{enumerate} 

\subsubsection{Oracle Algorithm}
Finding the best order of columns is challenging because there is an exponential number of possible permutations for a given number of columns. For instance, a dataset with $N$ rows and $M$ columns would produce $N \times M!$ possible orders. Enumerating all of them would be prohibitively expensive in practice, so we need a heuristic that enables us to efficiently find an effective ordering.






\begin{algorithm}[t!]
\caption{Fixed Column Reordering}

\begin{algorithmic}[1]
\State \textbf{Input:} Table $T$
\State \textbf{Output:} Reordered Columns List $L$
\item[] 
\State Initialize $L \gets []$
\State Precompute $ASL \gets$ Map() \Comment{\parbox[t]{.5\linewidth}{Pre-computed average string length for each column}}
\item[]

\Function{CalculateScores}{$T$}
    \State Initialize $ColumnScores \gets$ Map()
    \For{each column $m$ in $T$}
        \State $C_m \gets$ Cardinality($T, m$)
        \State $ColumnScores[m] \gets ASL[m] \times \left( \frac{Table Length}{C_m} \right)$
    \EndFor
    \State \Return $ColumnScores$
\EndFunction
\item[]

\State $T_{current} \gets T$
\State $ColumnScores \gets$ CalculateScores($T_{current}$)

\While{Columns remain for selection in $T_{current}$}
    \State $c_{select} \gets \text{argmax}_{c} (ColumnScores)$ 
    \State $L.append(c_{select})$
    \State Remove $c_{select}$ from $T_{current}$
    \State $ColumnScores \gets$ CalculateScores($T_{current}$) \Comment{Calculate scores for remaining columns}
    % \State 
\EndWhile
\State \Return $L$
\end{algorithmic}
\end{algorithm}
% \vspace{-2em}

\subsubsection{Reordering Algorithm}
Our reordering algorithm employs column statistics---specifically, the cardinality of column values---to quickly search for an effective ordering. Databases typically maintain statistics, such as the number of unique entries (i.e., cardinality) and distribution of values for each column, on store data, which we leverage to infer the potential for prefix sharing. We simplify the problem by establishing a fixed column ordering for all rows. This allows us to avoid having to consider an exponential number of permutations. In practice, many datasets have columns with high cardinality (i.e., few shared prefixes), so their order does not affect the cache hit rate.
% ...\accheng{something we can say here?} \shu{many datasets have columns with high cardinality, so we can prune these columns to decrease the search space. Shu: what's the point here again?}

% Given the prohibitive cost of an exhaustive search, we employ a heuristic strategy based on column statistics - specifically, the uniqueness of column values. 
% \begin{enumerate}
%     \item  
%     \item 
%     % ing the combinatorial explosion and providing a manageable framework for prefix optimization.
% \end{enumerate}


% We can simplify the problem by assuming we have a fixed column ordering for all rows that are passed into LLM. (This might be natural because we can store it as a special index, and directly pass in the input as it is based on our ordering algorithm). 

Concretely, our algorithm begins by precomputing two pieces of metadata for each column: the average string length (ASL) and the cardinality (C) (or the number of unique values). These metrics enable us to estimate the likelihood of each column contributing to the token hit rate. We obtain the average length of the values in a given column by running a SQL query (e.g.,  \texttt{AVG(CHAR\_LENGTH(col)))} on the data.
% To compute the average length of column table, we obtain  like \texttt{AVG(CHAR\_LENGTH(col))}. 
% For efficiency, we sample a set of values from each column to precompute the average string length. 
% \accheng{how big is the sample size? does it matter?} \accheng{manually constructed query}
% \shu{We calculate the average length of column table column by using \texttt{AVG(CHAR\_LENGTH(col))}. For execution efficiency in larger table, we can sample... Shu: maybe no sample is okay, searched and realized that people just directly calculate it}
We retrieve the cardinality from existing database statistics present in most systems.

% The heuristics algorithm begin by precomputing two pieces of metadata for each column: the average token length (ATL) and the cardinality (C) (or the number of unique values). 
% \begin{enumerate}
%     \item These metrics serve as proxies for evaluating each column's likelihood to contribute to prefix cache utilization. 
%     \item We sample a set of values to pre-compute the average token length for each column. 
%     \item We can also retrieve cardinality of individual column easily, as it is often times stored in system table for optimizer use. 
% \end{enumerate}

Next, the algorithm calculates a score for each column.
We draw inspiration from standard caching algorithms, such as GDSF~\cite{gdsf}, which give equal weight to size and frequency factors. Our algorithm uses the following formula: $$\textit{Score(\text{col})} = \text{ASL}_\text{col} \times \frac{\text{Total Number of Rows}}{\text{C}_\text{col}}$$
Under this method, higher scores correspond to columns with longer and more frequent shared data values. Our algorithm then places columns in order of descending scores. 

% As an example, Table 1 shows...\accheng{example TBU}
% \joey{I think you need to say that this column ordering is then used in the subsequent steps to determine the row ordering as well as the ordering of the columns in the call to the LLM.}


% \accheng{early simulation results show...
% suggest lots of follow-on work
% }

\subsubsection{Limitations} While our column-level input reordering algorithm demonstrates the potential for enhancing cache efficiency, it has limitations. The primary assumption under our approach is the fixed ordering of columns across all data rows. This assumption simplifies the computational complexity but may not always hold in real-world scenarios. In practice, different rows could benefit from different orderings based on the specific data they contain. Future work could explore smarter reordering strategies, as we will talk about in Section \ref{sec:smarter_reordering}.

% The algorithm proceeds by calculating a score for each function, defined by $$\textit{Score} = \text{ATL} \times \frac{\text{Number of Rows}}{\text{C}}$$. 
% \begin{enumerate}
%     \item The scoring mechanism is designed to identify columns that are likely to contain long, reusable prefixes while being sufficiently common across different queries. 
%     \item Columns are then selected sequentially based on their scores, approximating an arrangement under practical computational constraints. 
%     \item \shu{Idk whether example as in table 1 is worth it?}
% \end{enumerate}

% \begin{table}[t!]
% \centering

% \begin{tabular}{ccc|ccc}
% \toprule
% \multicolumn{3}{c}{Original Order} & \multicolumn{3}{c}{Our Order} \\
% \midrule
% \textbf{Z} & \textbf{Y} & \textbf{X} & \textbf{X} & \textbf{Y} & \textbf{Z} \\
% \midrule
% 0 & 4 & 5 & 5 & 4 & 0 \\
% 10 & 6 & 8 & 5 & 7 & 3 \\
% 1 & 9 & 8 & 8 & 9 & 1 \\
% 2 & 6 & 8 & 8 & 6 & 10 \\
% 3 & 7 & 5 & 8 & 6 & 2 \\
% \bottomrule
% \end{tabular}
% \vspace{4pt}
% \caption{A small data table sorted in two different ways. Original order has 0 cache hits, our order has 4 hits.}

% \end{table}



% \begin{itemize}
%     \item Precompute Average Token Length (ATL): For each column, we sample a set of values to calculate the average token length. This step accounts for the computational work associated with processing each column's values. 
%     \item Calculate Number of Unique Groups (NG): For each column, use a \texttt{GROUP BY} operation to identify the number of unique groups formed by the column's values.
%     \item Estimate Column Scores:  For each column, calculate its score as $$\textit{Score} = \text{ATL} \times \frac{\text{Table Length}}{\text{NG}}$$ This score reflects the potential computational savings from reordering based on this column. 
%     \item Select Columns Sequentially: Starting with the column with the highest score, select columns for reordering, recalculating scores for the remaining columns after each selection to account for changes in the table structure. 
%     \item The algorithm is illustrated in Algorithm 1.
% \end{itemize}



% \subsubsection{Greedy Algorithm (Fixed Ordering for SubGroups)} 

% Now assume that we don't have the constraints on fixed column orderings for all rows. 
% \begin{enumerate}
%     \item In the case where we have two columns, we can reduce it to a graph problem. 
%     \item Assume that there is a fixed length for each column for now. 
% \end{enumerate}

% For example, let's consider two columns of requests as illustrated in Figure \ref{fig:table-and-figure}. We construct the graph representation of this table as follows 
% \begin{enumerate}
%     \item There is a list of nodes for each column.
%     \item Each node represents the unique value for each column.
%     \item Connect an edge between nodes across columns if this row exists.
%     \item The degree of nodes represents the sharing factor of this value (i.e. basically how many requests have this value). 
% \end{enumerate}

% Now, a single iterative algorithm can be 
% \begin{enumerate}
%     \item For each node, assign a score $$(\text{degree} - 1) - (\text{number of neighbors with degree} > 1)$$
%     \begin{enumerate}
%         \item degree - 1: amount of cache hits 
%         \item we subtract the number of neighbors with degree > 1 because the edge is symmetric. This means that prioritizing either side of the column does not matter. 
%     \end{enumerate}
%     \item Select the node with the max score and fix the column ordering for this unique value. 
%     \item Remove edges associated with this node after selection. Recompute scores for any node that gets affected. 
%     \item Do this iteratively until all edges are removed. 
% \end{enumerate}

% In our example, we will fix all rows for $C$ first, then choose $B$, and then $D$ and $J$. 

% \textbf{Note}
% \begin{enumerate}
%     \item This is hard to prove optimal at high-dimension.
%     \item At high-dimension, the problem where we don't have constraints on column orderings for all rows can potentially be solved using a DP program. 
%     \item We select the group with max shared first, then fix the rows associated with this group and solve it iteratively. 
%     \item Some optimizations: pruning the space (or groups that have few share) to reduce the computational complexity 
% \end{enumerate}



% \subsubsection{Comparison with Traditional Clustered Index} Traditional database indexing strategies prioritize short, unique, and static values to improve physical data retrieval efficiency, while LLM column ordering aims to maximize computational efficiency by prioritizing the reuse of common, longer shared strings to enhance cache performance. 

% \begin{enumerate}
%     \item Prioritize uniqueness: Traditional databases often prioritize columns with high uniqueness for the clustered index. This is because a unique or highly distinct column (like an ID or a primary key) helps in efficiently locating and retrieving data.
%     \item Prioritize short keys: Wide keys (i.e., keys with large data types or multiple columns) make the index bulky and reduce performance. 
% \end{enumerate}

% But find out some other works where low cardinality columns can be prioritized first. https://arxiv.org/pdf/0909.1346.pdf
% \begin{enumerate}
%     \item This contains proof for both row and column-level reordering 
% \end{enumerate}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROW


\subsection{Row Sorting}
% \begin{algorithm}[t!]
% \caption{Row-Level Sorting Based on Column Prioritization}

% \begin{algorithmic}[1]
% \State \textbf{Input:} Table $T$, Reordered Columns List $L$ from Algorithm 1
% \State \textbf{Output:} Reordered Table $T'$
% \item[] 
% \State $T' \gets T$ with columns reordered according to $L$ 

% \For{$i \gets 0$ to length($L$)$\text{ } - 1$}
%     \State $T' \gets stableSort(T', L[i])$ \Comment{Apply stable sort on $T'$ based on column $L[i]$, preserve previous sort orders}
% \EndFor


% \State \Return $T'$

% \end{algorithmic}
% \end{algorithm}

% \begin{mdframed}[linecolor=black, linewidth=.5pt]
% \begin{minted}[fontsize=\small]{sql}
% SELECT LLM("Summarize the content of this movie: {movie}", m.movieInfo) AS summary 
% FROM Movies m
% \end{minted}
% \end{mdframed} 
% \vspace{8pt}

% \shu{Remove this example, and connect to the previous section}
% In the context of querying LLM with SQL, a common pattern involves passing a specific column from database table as input to the LLM. 
% \begin{itemize}
%     \item For instance, consider a query that summarizes movie contents, where the \texttt{m.movieInfo} column from the \texttt{Movies} table is used to generate summaries. 
%     \item This approach generates content summaries based on detailed movie information stored in the database. 
% \end{itemize}

Once we determine a column order, we need to group the rows of data such that we maximize the number of shared prefixes across requests. To achieve this, we concatenate all column values into a string and sort these strings lexicographically (over different rows) to determine the row order. 

% treat each row in its column order and concatenate each column value into a string. Then, we sort the string lexicographically to determine the row order. 

% To achieve this, we employ a stable sorting algorithm to sort the rows. A stable sort is crucial here as it ensures that rows with equal values in the sorting column maintain their relative order post-sorting. This property is important for preserving the grouping of shared prefixes when the data is sorted on one of the selected columns. 

% To do so, we introduce a row sorting algorithm to increase cache utilization. Specifically, we stably sort the rows (using an existing sorting algorithm, such as \accheng{what sort do we actually use?}) to maintain the relative order of rows with equal values (i.e., shared prefixes), ensuring that their original order is preserved in the sorted output. This enables us to place rows with shared prefixes together...\accheng{shu, i'm still unclear here}

% \accheng{stable sorts, maintains sorted order}

% With a column order in hand, we turn to the problem or row level sorting to further increase cache utilization. 

% Assuming now we select some orderings of the column. Row-level reordering focuses on optimizing the order of requests to maximize cache utilization. Specifically, we group together inputs that share prefixes.

% \begin{itemize}
%     \item For instance, consider a query that summarizes movie contents, where the \texttt{m.movieInfo} column from the \texttt{Movies} table is used to generate summaries. 
%     \item This approach generates content summaries based on detailed movie information stored in the database. 
% \end{itemize}



% \begin{table}[!t]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \multicolumn{1}{c|}{T} & \multicolumn{2}{c|}{Without Reordering} & \multicolumn{2}{c}{With Reordering} \\ \hline
%         & Keys accessed & Cache state & Keys accessed & Cache state \\ \hline
%         1 & ${\color{red}1, 2, 3}$ & - & ${\color{red}1, 2, 3}$ & - \\ \hline
%         2 & - & $1, 2, 3$ & - & $1, 2, 3$ \\ \hline
%         3 & ${\color{red}4, 5, 6}$ & $1, 2, 3$ & $1, 2, 3$ & $1, 2, 3$ \\ \hline
%         4 & - & $4, 5, 6$ & - & $1, 2, 3$ \\ \hline
%         5 & ${\color{red}1, 2, 3}$ & ${4, 5, 6}$ & ${\color{red}4, 5, 6}$ & $1, 2, 3$ \\ \hline
%         6 & - & $1, 2, 3$ & - & $4, 5, 6$ \\ \hline
%         7 & ${\color{red}4, 5, 6}$ & $1, 2, 3$ & $4, 5, 6$ & $4, 5, 6$ \\ \hline
%     \end{tabular}
%     \vspace{0.5em}
%     \caption{Comparison of KV cache state with different prefix input orders. Red represents cache misses: without reordering, there are 12 cache misses; with reordering, there are only 6 cold misses. }
%     \vspace{-3em}
%     \label{tab:cache-state-comparison}
% \end{table}

% \accheng{do we want to use the term prefix cache?}
To demonstrate how this technique improves cache usage, consider an example in which we have a batch size of tee and six distinct prefixes that each appear tee times (as illustrated in Table \ref{tab:cache-state-comparison}). If the requests arrive in the following order (with batches shown in brackets): $[1,2,3],[4,5,6]$ $,[1,2,3],[4,5,6]$,     the KV cache would evict and recompute all six prefixes under a caching algorithm, such as FIFO, leading to inefficient cache use. Instead, if we sort the rows of input to group common prefixes together (e.g., $[1,2,3],[1,2,3],[4,5,6],[4,5,6]$), we ensure that each prefix is loaded into the cache only once and reused across any requests it is involved in. Upon eviction, we know that this prefix will never need to be loaded into the cache again. This approach can greatly reduce cache eviction and recomputation, leading to faster LLM processing times.

Conveniently, the structured nature of SQL queries enables us to efficiently sort requests---we can identify and easily group shared data based on the relational schema by using existing database operations (e.g., \texttt{GROUP BY and ORDER BY}).


% \begin{enumerate}
%     \item If the requests arrive in the following order with batches show in brackets: $[1,2,3],[4,5,6]$ $,[1,2,3],[4,5,6]$, 
%     the prefix cache would evict and recompute all six prefixes under an existing eviction method (e.g., FIFO), leading to inefficient cache use.  
%     \item Instead, if we reorder the inputs to group common prefixes together, such as $[1,2,3],[1,2,3],[4,5,6],[4,5,6]$
%     we ensure that each prefix is loaded into the cache only once and reused across any requests it is involved in. Upon eviction, we know that this prefix will never be loaded into the cache again.
%     \item This approach can greatly reduce cache eviction and recomputation, leading to faster LLM processing time (Section~\ref{}).
% \end{enumerate}



% Using the same query above as an example, to optimize for prefix caching, we can group data from $m.movieInfo$ using existing database operations (e.g., \texttt{GROUP BY}). 

% \subsection{Reordering Algorithm}
% \shu{Put the algorithms for each of the subsection, get rid of 3.3}
% In this section, we describe our algorithm for reordering rows and columns. 
% \begin{itemize}
%     \item The column reordering is designed to prioritize columns that, when used as prefixes, would result in the higher cache reuse rates. 
%     \item Once the columns are reordered, sort rows so that rows with common values in the highest-priority columns are grouped together. This step may involve sorting rows based on the values of one or more columns, starting with the first column.
% \end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Solutions: Workload Shaping and Oracle Cache Scheduling}
% % \begin{itemize}
% %     \item To address these challenges, we propose a strategy that leverages the unique characteristics of batch workloads 
% %     \item This involves 
% %     \begin{itemize}
% %         \item \textbf{Field Ordering    }
% %         \begin{itemize}
% %             \item Based on the workload characteristics  
% %             \item We have control in how to shape the workloads to maximize cache reuse
% %         \end{itemize}
% %         \item \textbf{Workload-aware cache scheduling}
% %         \begin{itemize}
% %             \item Optimize end-to-end cache hit rate and GPU utilization. 
% %             \item We know  
% %             \begin{itemize}
% %                 \item When exactly should the prefix be evicted so that it does not eat up GPU memory. 
% %                 \item When prefixes should not be stored in the first place. 
% %             \end{itemize}
% %         \end{itemize}
% %     \end{itemize}
% % \end{itemize}
% \textbf{Solution \#1: Reshape the Workload}
% \begin{itemize}
%     \item \textbf{Structured inputs} and \textbf{control over the workload} give us unique opportunities to reshape the inputs to maximize cache hits on prefix 
%     % \shu{Longest common prefix first; string A, B, C, A, B, C, D, currently in this order, strict subset comes after something else; slight twick on sorting, and say future works can explore; enough to put this into arxiv}
%     \item \textbf{Record-level reordering} 
%     \begin{itemize}
%         \item LLM is an order-sensitive UDF 
%         \item Sequential inputs: [1,2,3,4][5,1,2,3][4,5] are adversarial patterns to the LLM cache engine with LRU policy 
%         \item Solution: grouped inputs of ordered [1,1,1,1][1,1,1,1][2,2,...] allows prefix to be admitted only once, and repeatedly reused until eviction by LRU
%     \end{itemize}
%     \item \textbf{Row-level reordering} 
%     \begin{itemize}
%         \item One can imagine writing queries not just pass in one column from the database table, but the entire row 
%         \item For example, Fig. \ref{fig:row-reorder} illustrates that we can pass in all rows from \textit{movie} table entirely, which contains \textit{movieInfo}, \textit{movieTitle}, \textit{genres}, \textit{directors}, etc. and many other fields 
%         \item How to reorder these fields so that maximal prefixes can be shared is essential 
%         \item Example 
%         \begin{itemize}
%             \item Putting \textit{movieTitle} first does not make sense because the titles are most likely to be distinct 
%             \item If some \textit{directors} direct many movies, then it makes sense to put this field first 
%         \end{itemize}
%                           \item Solution: can use \textit{groupBy} to determine the sharing factor, select the most shared field, then use \textit{groupBy} to sort the rest of the field (without the first selected field), etc. Do this sequentially to select the next request in sequence. \shu{is this optimal? how to determine how many are shared, using something like RadixAttention?}
%     \end{itemize}
% \end{itemize}
% \textbf{Caveat: Warm up for Record-level Reordering}
% \begin{itemize}
%     \item Currently the requests within a batch cannot share the prefix (i.e. all of them are computed in parallel), which means that we need a separate warm-up phase to prefetch prefix in order to be reused 
%     \begin{itemize}
%         \item E.g. [A, A, A] has no reuse in cache, but [A] [A, A] has 
%         \item E.g. [A, A, B, B] [C, C, D, D] has 8 misses, while [A, B, C, D] [A, B, C, D] has 4 misses 
%     \end{itemize}
%     \item This might not be an issue when there is a lot of sharing (larger than batch size), but is an issue for smaller requests and for prefixes that are not shared that much 
%     \item @Shiyi: special kernel that allows sharing within batch 
%     \begin{itemize}
%         \item Assume the new kernel efficiency is on par with the current one 
%         \item Reordering with continuous batching yields the optimal cache hit rate, each unique prefix only has one cold miss 
%     \end{itemize}
%     \item \textbf{Assumption:} without that kernel for now 
%     \begin{itemize}
%         \item If we just consider \textbf{cache hit rate (or byte hit rate)} as an objective, then sequential processing and reordering is always the best (e.g. [A][A][B][B][B][C][C]) 
%         \item But we also want to \textbf{saturate the batch} and maximize parallelism 
%     \end{itemize}
% \end{itemize}
% \textbf{Solution \#1.1: Batching with Warmup}
% \begin{itemize}
%     \item For prefix that has only 1 request: put wherever there is space 
%     \item For prefix that has more than 2 requests 
%     \begin{itemize}
%         \item Sort the prefix according to their request frequency 
%         \item Fill in one by one until the batch is full 
%         \item Go tough distinct prefixes in this batch to drain all of their frequency counts 
%         \item If one frequency pool is drained, then the prefix is done, drain with another prefix request pool that can hit the current cache 
%     \end{itemize}
%     \item Example: D x 2, B x 3, C x 3, E x 4, A x 5, BS = 5 
%     \begin{itemize}
%         \item Naive reordering has 13 misses: [D, D, B, B, B] (All misses), [C, C, C, E, E] (All misses), [E, E, A, A, A] (E hits, A miss) [A, A] (A hits) 
%         \item This method has 5 misses: [D, B, C, E, A] (All misses), [D, B, C, E, A](All hits) , [DE, B, C, E, A](All hits) , [A, A] (All hits) 
%     \end{itemize}
% \end{itemize}

% We leverage table statistics, such as average token length (ATL) and unique value counts for each column, to estimate the optimal column order. This method allows us to circumvent the exponential complexity by fixing column orders based on their likelihood to contribute shared prefixes:



% \subsubsection{Formulation} 
% We formulate the problem of column-level input reordering as follows. Assuming the data value at a particular row and column, if cached, is cached entirely as a prefix (i.e. not considering sub-string of data as prefix now). We also assume that there are some auto-prefix detection mechanisms. 

% The primary objective is to find an optimal ordering of columns for each row in a database so that the number of shared prefix tokens is maximized across all requests. The efficiency is measured by \textit{amount of computation} saved by reusing prefixes in the cache. This requires an ordering of columns that maximizes the number of shared tokens across all rows. The number of shared tokens is the product of the number of shared data values times the length of these data values.

% \textbf{Definitions}
% \begin{enumerate}
%     \item Requests (rows): Let $R_i$ represents the $i^{th}$ request (or row) in the dataset, where $i \in 1, 2, ..., N$, and $N$ is the total number of rows 
%     \item Columns: Let $C_j$ denote the $j^{th}$ column in the table, where $j \in 1, 2, ..., M$, and $M$ is the total number of columns  
%     \item Data value: we denote string value in row $R_i$ and column $C_j$ as $D_{ij}$.  
% \end{enumerate} 


% \subsubsection{Optimal Algorithm}
% A naive optimal algorithm requires enumeration tough all the possible combinations of column orderings for each row, which is $O(N * M!)$ where $N$ is the number of rows, and $M$ is the number of columns from the table. 

% \begin{figure}[!t]
%     \centering
%     \begin{minipage}{0.51\linewidth}
%         \centering
%         \begin{tabular}{|c|c|}
%             \hline
%             \textbf{Column 1} & \textbf{Column 2} \\
%             \hline
%             D & L \\
%             \hline
%             D & A \\
%             \hline
%             B & G \\
%             \hline
%             B & F \\
%             \hline
%             C & Q \\
%             \hline
%             C & R \\
%             \hline
%             C & L \\
%             \hline
%             J & L \\
%             \hline
%             J & H \\
%             \hline
%         \end{tabular}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.43\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/two-column.pdf}
%     \end{minipage}
%     \caption{Rows and its graphical representation}
%     \label{fig:table-and-figure}
% \end{figure}


==> sections/3_2_sol_other_std_opt.tex <==
\section{Other Standard Optimizations}
~\label{sec:dedup}
\vspace{-1.0em}
% \accheng{shu, what is the category of a review? an int? maybe give an example} \shu{here there are only two types, one is 'Rotton', one is 'Fresh', and it is a string} 
% indicating a high level of duplication since most reviews fall into a small number of categories.

% \accheng{would be nice to have some statistics about our datasets + the \% of duplicates presents} \shu{In modern recommendation datasets, we often times see high degrees of duplication in the table columns. For example, for Rotton Tomato Movie datasets, \texttt{review\_type} is a column that categorizes the type of review. The selectivity ratio, a measure of uniqueness after deduplication compared to orginal dataset, was observed to be extremely low at 0.008. This indicates a high level of redundancy as majority of reviews fall into a small number of categories.} \accheng{clarify measure of uniqueness}


% A common challenge in large datasets is the presence of duplicates or similar data elements across rows. In our context, where LLMs or Vector DB process text data, it is typical to encounter similar or identical inputs and shared data elements. 
% there is a collection --> downplay it so that we don't get reviews (additional standard ones)
\paragraph{\textbf{Exact Deduplication}} We can further reduce runtime by minimizing the number of inference calls we need to make. Specifically, we can deduplicate across requests that have the same input prompts before passing them to the LLM or vector DB, in order to reduce the computational load.
% For instance, in the previous query shown in Section~\ref{sec:column-reordering}, many reviews might mention similar products. Processing every review through an LLM or vector DB would lead to redundant computations. Instead, we can identify these duplicates before passing them to the LLM or vector DB to reduce the computational load. 
In modern recommendation datasets, there are often high degrees of duplication in the table columns. For example, the Rotten Tomatoes Movie dataset~\cite{rotten-tomatoes-movies-dataset}, commonly used in recommendation models, has a \texttt{review\_type} column corresponding to the category of the review (e.g., ``Fresh'' or ``Rotten''). As a result, the selectivity ratio of distinct values compared to total values is only 0.008 since there are only two distinct categories.

% \accheng{how do we actually deduplicate? with filter operators?

% any challenges with doing this over many rows of data?} \shu{Updated}

%For instance, in SQL, the \texttt{DISTINCT} keyword can be used to eliminate duplicate rows from a result set, ensuring each unique item is processed only once. 

For this work, we choose to apply exact deduplication without affecting query results. In the RDMBS's, this is commonly achieved through the use of distinct filters (e.g., \texttt{DISTINCT} in SQL) on the query inputs. This approach is straightforward and effective for reducing the number of LLM invocations by filtering out duplicate requests before they reach the model. We present an ablation study on deduplication with columns of different selectivity ratios in Figure~\ref{fig:dedup} in Section~\ref{sec:evaluation}. Beyond exact matches, \emph{semantic} deduplication, which identifies semantically similar records, represents a promising area for future research. 
% We discuss it further in Section~\ref{sec:semantic_dedup}. 

\paragraph{\textbf{SQL Optimization}} Traditionally, relational databases employ cost-based query optimizers, which enhance the performance of requests by analyzing query structures and operators to minimize data accesses and computational overheads~\cite{catalyst}. We extend these optimizers to account for LLM operator costs so that they can find query plans that minimize LLM invocations. Specifically, we augment cost estimation for the external functions used to invoke LLMs. 
% Currently, LLMs are most commonly accessed via UDFs. For instance, Databricks offers an \texttt{ai\_query}() function that allows users to call a model endpoint~\cite{databricks-aiquery}. Similarly, Amazon Redshift enables uses to LLM calls via UDF functions~\cite{aws-redshift-llm}. 
We estimate LLM costs based on the input token length and the estimated decode length over requests. In most cases, LLM invocations are significantly more expensive than other query operators, so these calls are included in the query plan. 
% It is important to note that when deduplication is applied, the column statistics used by the MGR algorithm might not be directly usable. Therefore, we need to scan the input table to recalculate these statistics after deduplication. \shu{Argue that this is okay for the complexity of the algorithm already, overall?} In addition, applying deduplication across many rows of data presents challenges involving memory and processing time required to identify the duplicates efficiently. Furthermore, identifying duplicates is not helpful in scenarios with a vast amount of distinct data. We present an ablation study on deduplication with columns of different selectivity ratios in Figure~\ref{fig:dedup} in Section~\ref{sec:evaluation}. 

% A promising direction for future research is semantic deduplication (i.e., identify records that will give similar output results), and we discuss it further in Section~\ref{}.




% \accheng{what is our solution exactly? how do we actually account for the cost? are we gonna move this section to the implementation?}
% \shu{We should probably ask this. Traditional UDF cost estimation is hard, cardinality estimation is also hard; we only consider simple push-down predicates scenario. Are we going to make the claim that LLM UDF is definitely more expensive than the other operators?}

% \subsubsection{LLM Operator Costs}
% We let SQL optimizers to be aware of expensive invocations of these external functions. 



% \accheng{based on token length of the input and estimated decode length over requests? In most cases, LLM invocations are significantly more expensive than other query operators (Section~\ref{sec}), so these calls are pulled up in the query plan.}

% In the context of traditional SQL query optimization, the execution order of operations is crucial for efficient data retrieval and processing. SQL optimizers typically analyze query structures and reordering operations such as joins, selections, and projections to minimize data access and computational overhead. However, when integrating external UDF like LLM, the SQL optimizer needs to be aware of the external UDF cost. 




% Our solution involves pushing down cheaper operators and pushing up expensive LLM calls as much as possible, and let 

% \begin{figure}
%     \centering
%     \begin{mdframed}[linecolor=black, linewidth=.5pt]

%     \begin{minted}[fontsize=\small]{sql}
% -- Selection, Projection 
% SELECT u.UserID
% FROM Users u
% JOIN Comments c ON u.CommentID = c.CommentID
% WHERE
%     LLM("{Few_shot_examples}, sentiment on the {Text} is", c.Text) = 'Negative' 
%     AND c.Timestamp > '2023-10-01'
%     \end{minted}
%     \end{mdframed}
%     \caption{SQL Example with one LLM and one non-LLM filter. The order in which these filters are applied affects the end-to-end query execution time. \shu{Can remove this table if not enough space}}
%     \label{fig:filter}
% \end{figure}


==> sections/3_3_sol_sql.tex <==
\section{SQL Optimizations}
Traditionally, relational databases employ cost-based query optimizers to enhance the performance of requests. These optimizers analyze query structures and operators to minimize data accesses and computational overheads. We extend these optimizers to account for LLM operators costs so that they can find query plans that minimize LLM invocations.

% \accheng{what is our solution exactly? how do we actually account for the cost? are we gonna move this section to the implementation?}
% \shu{We should probably ask this. Traditional UDF cost estimation is hard, cardinality estimation is also hard; we only consider simple push-down predicates scenario. Are we going to make the claim that LLM UDF is definitely more expensive than the other operators?}

\subsection{LLM Operator Costs}
% We let SQL optimizers to be aware of expensive invocations of these external functions. 
We augment cost estimation for the external functions that are used to invoke LLMs.
Currently, LLMs are most commonly accessed via UDFs. For instance, Databricks offers an \texttt{ai\_query}() function that allows users to call a model endpoint~\cite{databricks-aiquery}. Similarly, Amazon Redshift enables uses to LLM calls via UDF functions~\cite{aws-redshift-llm}. We estimate LLM costs based on the token length of the input and estimated decode length over requests. In most cases, LLM invocations are significantly more expensive than other query operators, so these calls are pulled up in the query plan. 

% \accheng{based on token length of the input and estimated decode length over requests? In most cases, LLM invocations are significantly more expensive than other query operators (Section~\ref{sec}), so these calls are pulled up in the query plan.}

% In the context of traditional SQL query optimization, the execution order of operations is crucial for efficient data retrieval and processing. SQL optimizers typically analyze query structures and reordering operations such as joins, selections, and projections to minimize data access and computational overhead. However, when integrating external UDF like LLM, the SQL optimizer needs to be aware of the external UDF cost. 

As an example of how LLM operator costs affect query planning, consider the query provided earlier in Figure \ref{fig:filter} as an example. Without accounting for LLM inference costs, a naive execution might call the UDF on every row in the table before applying the filter \textit{c.Timestamp > '2023-10-01'}. This would lead to unnecessary LLM invocations and could significantly increase overall execution time. A better execution strategy would be to apply the filter before invoking the LLM UDF, thereby reducing the dataset size that the LLM processes. This optimization would also benefit other query operators, such as joins. In general, the optimizer will pull up LLM calls as much as possible since these tend to be the most expensive parts of the query.


% Our solution involves pushing down cheaper operators and pushing up expensive LLM calls as much as possible, and let 

\begin{figure}
    \centering
    \begin{mdframed}[linecolor=black, linewidth=.5pt]

    \begin{minted}[fontsize=\small]{sql}
-- Selection, Projection 
SELECT u.UserID
FROM Users u
JOIN Comments c ON u.CommentID = c.CommentID
WHERE
    LLM("{Few_shot_examples}, sentiment on the {Text} is", c.Text) = 'Negative' 
    AND c.Timestamp > '2023-10-01'
    \end{minted}
    \end{mdframed}
    \caption{SQL Example with one LLM and one non-LLM filter. The order in which these filters are applied affects the end-to-end query execution time.}
    \label{fig:filter}
\end{figure}


==> sections/4_architecture.tex <==
% \newpage
\section{System Architecture}

% Our work investigates a collection of optimizations enacted to enable LLM integration to SQL queries. Specifically, our optimizations enable both a cost-effective way to leverage LLM capabilities while reducing the latency bottleneck. In this section we discuss the specific design choices made in implementing our system to enable the queries discussed above.

% \subsection{Queries and Goal}
% \shu{I think for this query section put it more like as NoScope describes, talk about high level how does this query work (how would users write such SQL queries with UDF), I think detailed in types of queries can just be mentioned briefly but the overall structure of queries need to be explained first, and what does our \SYS/ do }
% \subsubsection{Single LLM Calls}
% Our most basic queries involved a single LLM UDF invocation from within the SQL query, either for projection or filtering. Specific query examples are shown in Figure \ref{fig:single-invoke}. Experiments were run varying the number of unique prefixes along with average prefix length.

% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- Rotten Tomatoes Movies --
%         --- Projection ---
%         SELECT LLM("Recommend movies for the user 
%             based on their review of the following movie. Below is a description of the movie followed by the user review.", r.review_content, m.movieInfo) AS recommendation
%         FROM reviews r
%         JOIN 
%             movies m ON r.rotten_tomatoes_link = m.rotten_tomatoes_link

%         --- Filtering ---
%         SELECT r.reviewer_name
%         FROM reviews r
%         WHERE
%             LLM("Analyze the sentiment of the following review. Answer with only 'Positive', 'Negative', or 'Neutral'.", r.reviewText) = 'Negative'
            
%         -- Amazon Digital Music --
%         --- Projection ---
%         SELECT 
%             LLM("Did the following review for the product match the quality indicated in the  following product description?", r.reviewText, m.description) AS matching_quality
%         FROM 
%             reviews r
%         JOIN 
%             metadata m ON r.asin = m.asin
%     \end{minted}
%     \caption{SQL Example: Single LLM invocation.}
%     \label{fig:single-invoke}
% \end{figure}


% \subsubsection{Multi-LLM Calls}
% In the multi-invocation queries, both a projection and a filter are done using two separate LLM invocations allowing analysis on only a specific subsection of the data. Here, one LLM call is used to leverage the model's filtering ability on unstructured columns (e.g. using sentiment analysis) and the other is used for the main query. Examples of this can be found in Figure \ref{fig:multi-invoke}

% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- Rotten Tomatoes Movies --
%         SELECT LLM("Recommend movies for the user 
%             based on their review of the following movie. Below is a description of the movie followed by the user review.", r.review_content, m.movieInfo) AS recommendation
%         FROM
%             Movies m
%         JOIN
%             Reviews r ON r.rotten_tomatoes_link = m.rotten_tomatoes_link
%         WHERE
%             LLM("Sentiment on the {Text}", r.review_content) = 'Positive'
%         -- Amazon Digital Music --
%         SELECT 
%             LLM("Did the following review for the product match the quality indicated in the following product description?", r.reviewText, m.description) AS matching_quality
%         FROM
%             reviews r
%         JOIN 
%             metadata m ON r.asin = m.asin
%         WHERE
%             LLM("Sentiment on the {Text}", r.reviewText) = 'Negative
%     \end{minted}
%     \caption{SQL Example: Multiple LLM invocations.}
%     \label{fig:multi-invoke}
% \end{figure}

% \subsubsection{Single RAG}
% RAG style queries are performed by embedding the contexts found within RAG datasets and performing similarity search on query questions before selecting relevant contexts to feed to the LLM invocation for analysis. Examples of these types of queries are shown in Figure \asim{TODO: insert figure} 



% \subsubsection{Multihop-RAG}
% In a similar flavor to traditional RAG queries, the multiple LLM invocation structure is leveraged to be able to run queries on multihop RAG datasets with multiple rounds of prompting the model with different contexts and/or questions. An example of this type of query can be found in Figure \ref{fig:rag}

% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- Single Invocation --
%         SELECT LLM("Answer the question given the   
%             following context", s.question, s.context)
%         FROM squad s
%         -- Multihop Invocation --
%         [insert query here]
%     \end{minted}
%     \caption{SQL Example: RAG LLM invocations.}
%     \label{fig:rag}
% \end{figure}

% \subsubsection{Different SQL Operators}
% Results of LLM invocations can also be used in aggreagating SQL expressions (such as AVG or SUM), and our benchmark includes these types of queries. Examples are shown in Figure \ref{fig:sql_operators}. 

% \subsection{Components}
% \shu{Implementation and technical details; Should have overview first; I think instead of subsubsection, using textbf will be better}
% \subsubsection{UDF} Our systems side optimizations are implemented in PySpark \asim{TODO: cite pyspark here} with a user defined function (UDF) implemented to handle invocations to the language model based on a batch of input queries. This UDF is responsible for input construction given a system prompt and column values along with output post-processing. Our datasets are read into PySpark dataframes and query scripts are also implemented using PySpark. Together, these scripts were implemented in 2.5k lines of Python code. 

% \subsubsection{SQL Optimizer} Within Pyspark, we perform smart SQL query optimizations to improve performance of our queries, including UDF pull-up (as this function cost is non-deterministic) along with push-down of non LLM filter operators. \asim{TODO: rewrite this section with proper details once this has been thoroughly implemented and fleshed out}

% \subsubsection{Model serving}
% Our experiments were run using vLLM to host a model locally. Modifications were made to enable prefix cache eviction and swapping during the course of inference for our queries which had many unique prefixes. 

==> sections/5_implementation.tex <==
\newpage
\section{Implementation}

In this section, we describe the implementation of our optimizations, which consists of 5K lines of Python code integrated with PySpark~\cite{spark-sql}. To invoke the LLM in SQL queries, we implement a PySpark~\cite{pyspark} \accheng{@asim,shu add brief clause about why we use PySpark/what PySpark is} UDF that makes external calls to an LLM endpoint and a vector database. The UDF takes in a prompt for the LLM as well as data values (per column) as arguments to pass to the model. We augment the query optimizer to account for LLM operators, and LLM output post-processing is handled in the UDF. 
% \amog{
% 1. Prompt construction can be very significantly shortened with more details and a concrete example in the Appendix.

% 2. Query optimization is not implemented. We should probably remove.

% 3. Constrained decoding is not novel. We can probably remove.


% The main takeaway currently is that the system is implemented in Spark, but it's also not clear how and when the reordering algorithms are actually executed.

% }

% \accheng{add high-level description of system like how calls go through pyspark to vllm}

% \subsection{LLM UDFs and Optimizations}
% We implement external calls to the LLM endpoint and vector database using a PySpark \asim{TODO: cite pyspark here} user defined function (UDF).
% \begin{enumerate}
%     \item This UDF is responsible for input construction given a system prompt and column values.
%     \item LLM output post-processing is also handled in the UDF. 
% \end{enumerate} 

\textbf{Prompt construction.} Our UDF converts column values to prompt strings that can be parsed by an LLM. The first part of every prompt is the \textit{system prompt} containing instructions for the LLM. In the \textit{user prompt}, the question is provided as well as a JSON encoding of the column values for a particular row.

% \textbf{Query optimization.} Traditionally, relational databases employ cost-based query optimizers, which enhance the performance of requests by analyzing query structures and operators to minimize data accesses and computational overheads~\cite{}. We extend these optimizers to account for LLM operators costs so that they can find query plans that minimize LLM invocations. Specifically, we augment cost estimation for the external functions that are used to invoke LLMs. 
% % Currently, LLMs are most commonly accessed via UDFs. For instance, Databricks offers an \texttt{ai\_query}() function that allows users to call a model endpoint~\cite{databricks-aiquery}. Similarly, Amazon Redshift enables uses to LLM calls via UDF functions~\cite{aws-redshift-llm}. 
% We estimate LLM costs based on the token length of the input and estimated decode length over requests. In most cases, LLM invocations are significantly more expensive than other query operators, so these calls are pulled up in the query plan. 

% \shu{I remove the SQL query example, describe in text instead to save space} 
% \accheng{@shu, removing this para since I don't think we need to go into detail}
% As an example of how LLM operator costs affect query planning, consider the query provided earlier in Figure \ref{fig:filter} as an example. Without accounting for LLM inference costs, a naive execution might call the UDF on every row in the table before applying the filter \textit{c.Timestamp > '2023-10-01'}. This would lead to unnecessary LLM invocations and could significantly increase overall execution time. A better execution strategy would be to apply the filter before invoking the LLM UDF, thereby reducing the dataset size that the LLM processes. This optimization would also benefit other query operators, such as joins. In general, the optimizer will pull up LLM calls as much as possible since these tend to be the most expensive parts of the query.

% We implement logic in our UDF for converting column inputs into LLM-readable prompt strings. 
% \begin{enumerate}
%     \item Takes a system prompt argument which contains the primary instruction repeated across all rows to be processed. 
%     \item If multiple columns are passed into the UDF, prompts are constructed using columns in the order they appear in the UDF column list argument.
%     \item If the constructed prompt for a given row is too long for our model context length (4096 tokens), we truncate the row to the system prompt and skip the row. \asim{do we need this?}
% \end{enumerate}

\textbf{Output post-processing.} LLM output can be inconsistent and contain rambling answers (even if the model is explicitly told to be concise in its instruction prompt).
We take advantage of the vLLM\cite{vllm} serving engine, which supports constrained decoding of outputs to match our output pattern(s). Accordingly, we implement our UDF to optionally take in output pattern(s) as arguments, which the UDF searches for in the LLM output. For example, in a sentiment analysis query, we may only want our outputs to be "Positive", "Negative", or "Neutral", so we specify these output targets to the UDF. \amog{Again, I would strongly consider removing this section. Guided decoding is a property of vLLM, not our work, and I believe we don't even use constrained decoding for any of our experiments.}

% LLM output is inconsistent and can often ramble to answer a user question in several words despite being told not to do so in its instruction prompt. 
% \begin{enumerate}
%     \item Therefore, in order to perform useful follow-up analysis on your table given the output of an LLM call, it is necessary to clean the LLM output and extract information we seek. 
%     \item Thus, we optionally allow for output pattern(s) as an argument to the UDF which will be searched for in the LLM output.
%     \item For example, in a sentiment analysis query, we likely only want our LLM outputs to be "Positive", "Negative", or "Neutral".
% \end{enumerate}

% \subsection{Prefix Caching}
% We implement a novel eviction strategy for the KV cache within vLLM to address a limitation of current system.
% The existing vLLM implementation assumes that all prefixes of a batch of requests can fit in the KV cache, but this does not hold when there is a high diversity in prefix size, which is typical for batch analytical workloads. We take a reactive approach: when a new request is scheduled and there is insufficient GPU memory to accommodate the new requests, the system automatically evicts prefixes based on first-in, first-out (FIFO) order. If a previously evicted prefix is needed for a future request, it is recomputed and readmitted into the cache. This strategy ensures that the system dynamically adapts to changing workload patterns while managing memory constraints effectively. 

% We address this limitation by implementing a novel eviction strategy for the KV cache within vLLM. 


% In our system, we address the limitations of the current vLLM implementation, which assumes that prefixes of all requests in a batch can fit within available memory. This assumption does not hold in scenarios with a vast and diverse range of possible prefixes, which are typical in our batch analytics setup. To manage this, we implement an eviction strategy for prefix caching within the vLLM framework. Our approach is reactive: when a new request is scheduled and there is insufficient GPU memory to accommodate the new requests, the system automatically evicts the the first-in, first-out (FIFO) prefixes from the KV cache. If a previously evicted prefix is needed for a future request, it is recomputed and readmitted into the cache. This strategy ensures that the system dynamically adapts to changing workload patterns while managing memory constraints effectively.

% \subsection{VectorDB Retrieval}


% \shu{Have separate sections; before evaluation, need implementation sections (Transactional caching paper), should be short; what systems, what do we change, and mention stuff in 3.5, do it straightforward way, separate it into the pyspark and vllm changes; first sentence: topic sentence, just read the first sentence, and know what they get from the topic sentence (get to the point as soon as possible), that sentence takes the longest to write, and be clear what is the structure; leave it for bullet point for now}

% \subsection{Optimized Cache Management}
% In this section, we address cache admission and eviction for batch queries.
% \begin{itemize}
%     \item Existing inference systems typically admit all prefixes into the cache and employ a simple eviction policy, such as FIFO, to serve online, dynamic requests.
%     \item Their lack of awareness of future requests can lead to severe cache underutilization.
%     \item For instance, any prefixes that occur only once should not be cached since they will not benefit future requests.
%     \item Furthermore, proactive eviction of prefixes that will no longer be used can free up memory for other purposes.
% \end{itemize}


% We implement admission and eviction algorithms based on workload knowledge.
% \begin{itemize}
%     \item From our reordering algorithm in Section~\ref{}, we are aware of which requests will access each prefixes.
%     \item \textbf{Admission}: We only admit prefixes to the cache if  they are accessed by more than one request, enabling us to reduce the write costs of loading prefixes into the KV cache.
%     \item \textbf{Eviction}: We proactively evict prefixes once they are no longer involved in future requests.
%     \item Consider as an example the following batches of requests: $[D,D,B][B,B,B][C,A,A]$.
%     \item We no longer need $D$ after the first batch, so we only cache $B$. After the second batch completes, we can evict $B$ immediately.
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{sec:queries}
% \begin{table}[t]
%     \centering
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular}{ m{7.5em}  m{16em}}
%           \toprule
%           {\bf Parameter} & {\bf Description}  \\
%         %   \hline
%             \midrule
%           Retriever & Structured and unstructured database \\%\hline
%       Analyzer & LLM, other ML models \\%\hline
%       Pipeline  & Single-hop, Multi-hop \\%\hline
%       SQL types & Selection, Projection, Join, Order By, Min, Max, Count, Sum, Avg \\%\hline
%       \bottomrule
%       \end{tabular}
%   }
%   \vspace{0.5em}
%     \caption{Benchmark Parameters.}
%     \label{tab:benchmark}
% \end{table}


% \subsection{Categories}
% \shu{Maybe shouldn't list these queries: maybe write it in this way: VBase paper, can't spend too much time on this, why making up the queries all by themselves, they take a page (very long), have to argue why these are the right queries and why they matter, those things should be in the evaluation, first section of Eval (Eval benchmark)}

% \label{sec:queries-categories}
% We systematically categorize various types of queries as our benchmark suite in the context of integrating LLMs and Vector DB with SQL, as shown in Table \ref{tab:benchmark}. This table classifies queries based on several key parameters. 

% \textbf{Retriever} This parameter distinguishes between structured and unstructured databases. Structured databases follow a fixed schema, like those stored in the traditional SQL database. Unstructured databases handle more flexible data formats like image and videos; these data are typically stored as embedding in vector database. The choice of retriever impacts the query formulation, especially in terms of data extraction and pre-processing.

% \textbf{Analyzer}: The role of the LLM as an analyzer is to interpret data. LLMs can process natural language, making them ideal for tasks like sentiment analysis, summarization, or extracting specific information from the data provided. While LLMs are central to our discussion, other machine learning models can also be used as analyzers, depending on the nature of the data or specific requirements of the query. Different models often have different trade-offs in terms of computational and monetary costs. 

% \textbf{Pipeline}: The pipeline parameter focuses on whether the query uses a single-hop or multi-hop approach. Single-hop queries directly retrieve and process data, whereas multi-hop queries involve multiple steps, often combining data retrieval and processing in multiple stages.

% \textbf{SQL Types}: This includes a range of SQL query types such as Selection, Projection, Join, Order By, Min, Max, Count, Sum, Avg. Each type can be used differently according to the workload context. 

% \subsection{Examples}
% \subsubsection{Retriever and Analyzer}
% The query in Figure \ref{fig:retriever} demonstrates the integration of different retrievers. It uses a structured database (albums and artists) to extract the reviews. The LLM acts as an analyzer to identify the artist's name mentioned from reviews. Then vector DB acts as a retriever, where it stores the correct artist name as embeddings, to correct misspellings in the artist name by doing similarity search. The results are then used in the structured database to extract the number of albums corresponding to this artist. 

% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- extract the number of albums for the artist mentioned in the review. 
%         SELECT SUM(albums) 
%         FROM albums 
%         WHERE album.aid IN (
%             SELECT aid 
%             FROM artists 	
%             WHERE artists.name IN s.correct_artist 
%                 (
%                     SELECT 
%                         review, 
%                         LLM("What is the artist mentioned in this review?", review) as artist, 
%                         Vector_DB("Correct this word spelling", artist) as correct_artist 
%                     FROM reviews
%               ) AS s
%         ) 
%     \end{minted}
%     \caption{SQL Example: retriever.}
%     \label{fig:retriever}
% \end{figure}

% \subsubsection{Complex Pipeline}
% The query in Figure \ref{fig:complex-pipeline} shows a scenario where LLM is invoked multiple times. Initially, it identifies negative sentiment reviews for products. Then, it performs a summarization task to condense the main issues from these reviews. 
 
% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- Multi-invocations to LLM in SQL 
%         SELECT 
%             p.ProductID, 
%             LLM("Summary of main issues in {Text}", 
%         	GROUP_CONCAT(r.ReviewText)) AS CommonIssues
%         FROM ProductReviews r
%         JOIN Products p ON r.ProductID = p.ProductID
%         WHERE 
%             LLM("Sentiment on the {Text}", r.ReviewText) = 'Negative'
%         GROUP BY p.ProductID
%         HAVING COUNT(*) > 100
%     \end{minted}
%     \caption{SQL Example: chain of execution.}
%     \label{fig:complex-pipeline}
% \end{figure}


% \subsubsection{SQL Operators}
% Figure \ref{fig:sql_operators} demonstrates queries with different operators. The first query within this figure exemplifies the use of the join operator, merging ticket request and response data. The second query demonstrates the selection and projection operators. By joining user and comment data, the LLM is used to assess the sentiment of each comment. The final query in this figure uses the aggregation operator to calculate the average sentiment of product reviews.

% \begin{figure}
%     \centering
%     \begin{minted}{sql}
%         -- Join (LLM output from both side) 
%         SELECT 
%             tr.ticket_id,
%             LLM(
%                 "Examples {few_shots}, Did {response_text} address {request_text}", 
%                 VectorDB(tr.response_text + tr.request_text) as few_shots, 
%                 tr.response_text,
%                 tr.request_text
%             )
%             AS resolution_success
%         FROM ticket_requests r
%         JOIN ticket_responses s ON r.ticket_id = s.ticket_id as tr 
%         WHERE s.response_text IS NOT NULL AND r.status = 'resolved'
        
%         -- Selection, Projection 
%         SELECT u.UserID
%         FROM Users u
%         JOIN Comments c ON u.CommentID = c.CommentID
%         WHERE
%             LLM("{Few_shot_examples}, sentiment on the {Text} is", c.Text) = 'Negative' 
%             AND c.Timestamp > '2023-10-01'

%         -- Average 
%         SELECT 
%             p.ProductID, 
%             AVG(LLM("Sentiment score on the {Text}", r.ReviewText)) as AverageSentiment
%         FROM Products p
%         JOIN Reviews r ON p.ProductID = r.ProductID
%         WHERE r.Timestamp BETWEEN '2023-01-01' AND '2023-12-31'
%         GROUP BY p.ProductID

%     \end{minted}
%     \caption{SQL Example: different SQL operators.}
%     \label{fig:sql_operators}
% \end{figure}





==> sections/6_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
% \shu{Matei: if we have time, I'd love an experiments that checks whether accuracy is significantly affected by column reordering in the queries we do that in.}

In this section, we evaluate the effectiveness of our optimizations within a constructed benchmark suite of queries. We aim to answer the following questions: 
% \shu{@Audrey: double check these questions?} %\shu{reframe this as question, not findings}
% \begin{enumerate}
%     \item \accheng{summarize main findings similar to NoScope S9s}
%     \item \accheng{do we have any non-negligible overheads for any of our optimizations? if we don't have any, we should state this somewhere}
% \end{enumerate}

% \begin{enumerate}
%     \item \accheng{summarize main findings similar to NoScope S9s}
%     \item \accheng{do we have any non-negligible overheads for any of our optimizations? if we don't have any, we should state this somewhere}
% \end{enumerate}
% \begin{enumerate}
%     \item Changing the order of inputs we provide to the LLM, both within a single prompt and within a batch of prompts, can noticeably reduce query latency.%, up to 3.0$\times$ over unreordered inputs in our experimental results. 
%     \item LLM output generation time dominates query latency, and optimizations that reduce the number of inputs the LLM receives significantly improve performance.% We see up to 1.7$\times$ over passing in the full input list to the LLM in our experimental results. 
% \end{enumerate}

\begin{enumerate}
    \item How does the request reordering optimization impact query latency across different LLM query types and datasets? 
    \item What effects do standard optimizations like deduplication and SQL optimizations have on query latency? 
    \item How does our request reordering algorithm influence LLM accuracy and solver time? 
\end{enumerate}
% \begin{enumerate}
%     \item What is the impact of reordering the inputs we provide to the LLM on the query latency, both within a single prompt and for a batch of prompts? 
%     %can noticeably reduce query latency.%, up to 3.0$\times$ over unreordered in∂∑puts in our experimental results. 
%     \item Does reducing the number of inputs the LLM significantly impact end-to-end latency? Does LLM output generation time dominate query latency?
%     % We see up to 1.7$\times$ over passing in the full input list to the LLM in our experimental results. 
% \end{enumerate}

% and compare it against baselines without these optimizations. 

\subsection{Evaluation Benchmark}
\label{sec:queries}

% \begin{table}[t]
%     \centering
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular}{ m{7.5em}  m{16em}}
%           \toprule
%           {\bf Parameter} & {\bf Description}  \\
%         %   \hline
%             \midrule
%           Retriever & Structured and unstructured database \\%\hline
%       Analyzer & LLM, other ML models \\%\hline
%       Pipeline  & Single-hop, Multi-hop \\%\hline
%       SQL types & Selection, Projection, Join, Avg \\%\hline
%       \bottomrule
%       \end{tabular}
%   }
%   \vspace{0.5em}
%     \caption{Benchmark Query Parameters. \asim{this table isn't referenced anywhere}}
%     \label{tab:benchmark-table}
% \end{table}

Given the lack of standard benchmarks for LLM queries, we construct a benchmark suite to represent real-world data retrieval and processing tasks. We create a range of query types over datasets from various sources to assess the impact of integrating LLMs into relational analytics.

% The integration of LLMs into batch analytics and SQL query processing introduces a novel paradigm, yet there exists no benchmark specifically designed to evaluate the performance of such systems. Thus, in our evaluation, we have developed a benchmark suite tailored to assess the efficiency of a variety of LLM queries. 


\subsubsection{Datasets}

% Skip the tables 
% \begin{table}[!t]
%     \centering
%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{tabular}{|c|c|c|c}
%             \hline
%             \textbf{Field} & \textbf{Type} & \textbf{Example} \\
%             \hline
%             asin & identifier & 0741304058 \\
%             \hline
%             reviewText & string & ``A favorite cd now...'' \\
%             \hline
%             verified & boolean & True \\
%             \hline
%             overall & double & 5.0 \\
%             \hline
%             summary & string & ``Five Stars'' \\
%             \hline
%             Format & string & "MP3 Music" \\
%             \hline
%             description & list of strings & [``Great CD for babies...'', ``'', ``''] \\
%             \hline
%         \end{tabular}
%     \end{minipage}
%     \caption{Amazon Products Schema}
%     \label{tab:products_schema}
% \end{table}

% \begin{table}[!t]
%     \centering
%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{tabular}{|c|c|c|c}
%             \hline
%             \textbf{Field} & \textbf{Type} & \textbf{Example} \\
%             \hline
%             rotten-tomatoes-link & identifier & m/10002114-dark-water\\
%             \hline
%             review-type & string & ``Fresh'' \\
%             \hline
%             review-content & string & ``Fun, brisk and imaginative'' \\
%             \hline
%             top-critic & boolean & True \\
%             \hline
%             movie-info & string & ``In this moody...'' \\
%             \hline
%         \end{tabular}
%     \end{minipage}
%     \caption{Rotten Tomatoes Movies Schema}
%     \label{tab:movies_schema}
% \end{table}

We build our benchmark suite on a variety of commonly used datasets for recommendation and natural language processing (NLP) models. \textbf{Amazon Product Reviews}\cite{amazon-product-review-dataset} is a recommendation dataset that contains product reviews and metadata from Amazon. We utilize the 2023 version of the dataset and select the "Handmade Products" category, which consists of 586.6K reviews. We use 15,060 rows of this dataset in our queries. % The schema of this dataset includes  the fields of interest for this dataset is shown in Table \ref{tab:products_schema}.
\textbf{Rotten Tomatoes Movie Reviews}\cite{rotten-tomatoes-movies-dataset} is a recommendation dataset that stores critic review data along with movie metadata from the popular movie review website Rotten Tomatoes. This dataset consists of 1,130,018 reviews. We use 15,018 rows of this dataset in our queries. %We show part of the schema with fields of interest in Table \ref{tab:movies_schema}. 
\textbf{Stanford Question Answering Dataset (SQuAD)} \cite{squad-dataset} is a reading comprehension dataset with more than 100,000 rows and consists of questions posed by crowdworkers on a set of Wikipedia articles. The context to every question is a segment of text, or span, from the corresponding reading passage. \textbf{Fact Extraction and Verification (FEVER)}\cite{fever} is a dataset consisting of claims that have been generated by altering sentences from a set of Wikipedia passages. The claims have been classified by human annotaters as either Supports, Refutes, or NotEnoughInfo if the claims is factually correct based off the Wikipedia passages. We use a deduplicated labeled dev set of Fever consisting of 22,862 claims. The Wikipedia dataset contains over 5 million passages.
% \begin{enumerate}
%     \item \textbf{Amazon Product Reviews}\cite{amazon-product-review-dataset} is a recommendation dataset that contains product reviews and metadata from Amazon. We utilize the 2023 version of the dataset and select the "Handmade Products" category, which consists of 586.6K reviews. We use 15,060 rows of this dataset in our queries. 
%     % The schema of this dataset includes  the fields of interest for this dataset is shown in Table \ref{tab:products_schema}.
%     \item \textbf{Rotten Tomatoes Movie Reviews}\cite{rotten-tomatoes-movies-dataset} is a recommendation dataset that stores critic review data along with movie metadata from the popular movie review website Rotten Tomatoes. This dataset consists of 1,130,018 reviews. We use 15,018 rows of this dataset in our queries. %We show part of the schema with fields of interest in Table \ref{tab:movies_schema}. 
%     \item \textbf{Stanford Question Answering Dataset (SQuAD)} \cite{squad-dataset} is a reading comprehension dataset with more than 100,000 rows and consists of questions posed by crowdworkers on a set of Wikipedia articles. The context to every question is a segment of text, or span, from the corresponding reading passage. 
%     % accheng{unclear here}
%     \item \textbf{Fact Extraction and VERification (Fever)}\cite{fever} is a dataset consisting of claims that have been generated by altering sentences from a set of Wikipedia passages. The claims have been classified by human annotaters as either Supports, Refutes, or NotEnoughInfo if the claims is factually correct based off the Wikipedia passages. We use a deduplicated labelled dev set of Fever consisting of 22,862 claims. The Wikipedia dataset contains over 5 million passages.
% \end{enumerate}
 


% \begin{itemize}
%     \item asin - “id” field, each product has a unique asin
%     \item reviewText - a plain-text user submitted review for a product.
%     \item verified - a boolean field that denotes whether a given product is "verified" on Amazon. 
%     \item description - from the metadata table, description contains a short description for the product.
% \end{itemize} 

% \begin{itemize}
%     \item rotten-tomatoes-link - like an “id” field, each movie has a unique rotten-tomatoes-link
%     \item review-type - “Fresh” or “Rotten” (used in filtering queries)
%     \item review-content - a plaintext user or critic review for a movie
%     \item top-critic - a boolean field that denotes whether the author for a review is a "top critic" on the website or not
%     \item movie-info - from the metadata table, this field contains a short description for the movie
% \end{itemize}
% \newline

\subsubsection{LLM Queries}\label{llmqueries}
Our benchmark suite incorporates a wide range of query types and use cases. We show examples of each query type below. 

% Our query benchmark suite is designed to explore the full spectrum of \sys's capabilities, incorporating a broad range of query types and use cases:
\vspace{8pt}

\textbf{\textit{Q1/Q5: LLM projection.}} This query type makes calls to an LLM within a \texttt{SELECT} statement to process information from specified database column(s). It reflects common tasks in data analytics in which the LLM is used for summarization and interpretation based on certain data attributes. Q1 passes in a subset of columns from the table, while Q5 passes in the entire table. 
\vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Recommend movies for the user based on {movie information} and {user review}', m.info, r.review)
FROM reviews r JOIN movies m ON r.link = m.link
\end{minted}
\end{mdframed} 
\vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Given the following fields, answer in ONE word, Yes or No, whether the movie would be suitable for kids.', 
    mr.*)
FROM ( SELECT r.*, m.* FROM reviews r JOIN movies m ON r.link = m.link ) AS mr
\end{minted}
\end{mdframed} 
\vspace{8pt}
\textbf{\textit{Q2: LLM filter.}} This query type leverages LLM for filtering data within a \texttt{WHERE} clause. The LLM processes and analyzes information to meet specific criteria, such as identifying positive reviews. This query type illustrates typical use cases in sentiment analysis and content filtering, which are important for application tasks such as customer feedback analysis and content moderation. 
\vspace{4pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
    \begin{minted}[fontsize=\small]{sql}
SELECT m.movie_title
FROM Movies m JOIN Reviews r ON r.link = m.link
WHERE LLM('Analyze whether this movie would be suitable for kids based on {movie information} and {user review}', m.info, r.review) = 'Yes'  
AND r.rtype == 'Fresh'
    \end{minted}
    \end{mdframed} 
\vspace{8pt}

\textbf{\textit{Q3: Multi-LLM invocation.}} This query type involves multiple LLM calls in different parts of the query and addresses scenarios in which several layers of data processing or analysis are required. It represents advanced analytical tasks, such as combining different data insights or performing sequential data transformations.
\vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Recommend movies for the user based on {movie information} and {user review}', m.info, r.review) AS recommendations
FROM Movies m JOIN Reviews r ON r.link = m.link
WHERE LLM('Analyze whether this movie would be suitable for kids based on {movie information} and {user review}', m.info, r.review) = 'Yes'  
AND r.rtype = 'Fresh'
\end{minted}
\end{mdframed} 
\vspace{8pt}

\textbf{\textit{Q4: LLM aggregation.}} This query type incorporates LLM outputs into further query processing. For example, one such query could use LLMs to assign sentiment scores to individual reviews and then aggregate these scores to calculate an average sentiment for overall customer feedback. This query type is essential for tasks that need to extract insights from complex textual data. %clear, actionable overview 
\vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT AVG(LLM('Rate a satisfaction score between 0 (bad) and 5 (good) based on {review} and {info}: ', r.review, m.info)) as AverageScore
FROM reviews r JOIN movies m ON r.link = m.link
GROUP BY m.movie_title
\end{minted}
\end{mdframed} 
\vspace{8pt}
    
\textbf{\textit{Q6: Retrieval-augmented generation (RAG)}.} This query type leverages external knowledge bases for enhanced LLM processing, enriching LLM queries with broader context. It simulates use cases where queries need to pull in relevant information from external sources, such as document databases or knowledge graphs, to provide comprehensive answers. 
\vspace{8pt}
\begin{mdframed}[linecolor=black, linewidth=.5pt]
\begin{minted}[fontsize=\small]{sql}
SELECT LLM('Given the following {context}, answer this {question}', VectorDB.similarity_search(s.question), s.question)
FROM squad s WHERE s.is_impossible = False
\end{minted}
\end{mdframed}
\vspace{8pt}
% \begin{enumerate}
%     \item \textbf{\textit{Q1: LLM projection.}} This query type makes calls to an LLM within a \texttt{SELECT} statement to process information from specified database column(s). It reflects common tasks in data analytics in which the LLM is used for summarization and interpretation based on certain data attributes.
    
%     \item \textbf{\textit{Q2: LLM filter.}} This query type leverages LLM for filtering data within a \texttt{WHERE} clause. The LLM processes and analyzes information to meet some specified criteria, such as identifying positive reviews. This query type illustrates typical use cases in sentiment analysis and content filtering, which are important for application tasks, such as customer feedback analysis and content moderation. 
    
%     \item \textbf{\textit{Q3: Multi-LLM invocation.}} This query type involves multiple LLM calls in different parts of the query and addresses scenarios in which several layers of data processing or analysis are required. It represents advanced analytical tasks, such as combining different data insights or performing sequential data transformations.

%     \item \textbf{\textit{Q4: LLM aggregation.}} This query type incorporates LLM outputs into further query processing. For example, one such query could use LLMs to assign sentiment scores to individual reviews and then aggregate these scores to calculate an average sentiment for overall customer feedback. This query type is essential for tasks that need to extract insights from complex textual data. %clear, actionable overview 

%     \item \textbf{\textit{Q5: LLM Projection (Entire Table)}.} This query type uses multiple columns for each of the Movies and Products dataset. Specifically, 7 columns are used for Movies and 8 are used for Products.  
    
%     \item \textbf{\textit{Q6: Retrieval-augmented generation (RAG)}.} This query type leverages external knowledge bases for enhanced LLM processing, enriching LLM queries with a broader context. It simulates use cases where queries need to pull in relevant information from external sources, such as document databases or knowledge graphs, to provide comprehensive answers. 
% \end{enumerate}

% \begin{enumerate}
%     \item \textbf{\textit{Q1: Single-Invocation of LLM}} These queries involve a one-time call to an LLM to retrieve or process information.
%     \item \textbf{\textit{Q2: Multiple Invocations of LLM}} Complex queries that necessitate multiple calls to LLMs, often involving different pieces of information or processing steps.
%     \item \textbf{\textit{Q3: RAG}} Leveraging retrieval-augmented generation to enhance query processing by incorporating external knowledge sources like vector databases. 
%     \item \textbf{\textit{Q4: Different SQL Operators}} Including LLMs in filters, joins, or aggregations.
% \end{enumerate} \accheng{since this query takes significantly longer to run?} \asim{yes -- it involves 2 invocations so it takes much longer}

We run Q1-Q5 on the Amazon Product Reviews and Rotten Tomatoes Movie Reviews datasets and Q6 on SQuAD and FEVER. We evaluate Q1-Q5 on around 15,000 rows of the Movies and Products datasets. For Q6, we evaluate roughly 20,000 questions/claims for both SQuAD and FEVER, where each question retrieves \textit{K=3} contexts to augment its answer. 



\subsubsection{Evaluation Metrics}
Our key evaluation metric is the end-to-end query execution time, the most relevant metric for running analytical queries. %\accheng{@shu, because this is what analytical queries care about...?}. 
Additionally, we analyze the prefix hit rate, which represents the ratio of prefix tokens served from the KV cache and the input token length. This metric corresponds directly to query latency speed-up from the LLM side.
% While our previous algorithms use PHC as an objective, assuming that the entire value hits on a cell without allowing substring hits, THR is a more precise measure that reflects the actual performance during LLM execution. Thus, we report THR in our evaluation.  

% We also collect statistics on LLM inference performance, including tokens per second (TPS) and requests per second (RPS) processed. 
% This is a metric to measure the overall effectiveness of our systems in utilizing cached KV to speed-up query processing. 
% \accheng{what's the diff between token hit rate and hit rate?}

\subsubsection{Experimental Setup} %Hardware and model configurations
% We collect results for the queries formulated on single L4 machines with 24GB GPU memory, with larger experiments run on A100 machines with 80GB memory. For experiments, we use the LLaMA model with 7B parameters. This model was both lightweight and inexpensive which we considered critical for workloads in this context.  collect results for the queries
We run experiments on a g2-standard-48 GCP instance (48vCPUs, 192GB RAM) with an NVIDIA L4 GPU accelerator hosted in the us-central1 region. For the LLM endpoint, we use the instruction tuned variant of Meta's LLaMA-3 model with 8B parameters~\cite{llama3}. This model is lightweight and inexpensive to host locally, making it well-suited to analytical tasks. We use vLLM~\cite{vllm} as our model serving engine. For RAG queries, we use a GTE embedding model  (Alibaba-NLP/gte-base-en-v1.5)\cite{li2023towards} to embed the context and use Facebook Similarity Search Library (FAISS) ~\cite{johnson2019billion} to store these context embeddings into an index.

% \accheng{need some more context here? what does FAISS stand for?} \asim{@shu can you elaborate on this above}
% \begin{enumerate}
%     \item All instances are hosted in the us-central1 region.
%     \item For LLM endpoint, we use Meta's LLaMA-2 model with 7B parameters \cite{}.
%     \item This model was both lightweight and inexpensive to host locally, which we considered critical for workloads in this context \asim{do we need this??}.
%     \item We use vLLM as our model serving engine with LRU as the prefix cache eviction policy.
%     \item For RAG queries, we use BGE embedding models (BAAI/bge-large-en-v1.5) to embed the context, and use FAISS to store these context embeddings into an index. 
% \end{enumerate}



\begin{figure*}[tbp]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
        \centering
        % \includegraphics[width=\textwidth]{figures/movies_runtimes_e2e.pdf}
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/movies.pdf}
        \caption{Rotten Tomatoes Movies Dataset}
        \label{fig:movies-runtimes}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        % \includegraphics[width=\textwidth]{figures/products_runtimes_e2e.pdf}
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/products.pdf}
        \caption{Amazon Products Dataset}
        \label{fig:products-runtimes}
    \end{subfigure}

    %\vspace{-2em}
    \caption{End-to-end Result: Our optimizations (Cache (\greedy + Dedup + SQL Opt)) achieve 2.1 - 3.0$\times$ on Movie Dataset and 2.2 - 2.8$\times$ speed-up on Product Dataset over Cache with FIFO ordering (Cache(FIFO)). }
    \label{fig:runtimes}
\end{figure*}

% \begin{figure*}[tbp]
%      \centering
%      \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/SIGMODfigures/squad.pdf}
%         \caption{SQuAD Dataset}
%         \label{fig:squad}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/SIGMODfigures/fever.pdf}
%         \caption{FEVER Dataset}
%         \label{fig:fever}
%     \end{subfigure}

%     %\vspace{-2em}
%     \caption{End-to-end Result: Our optimizations (Cache (\greedy + Dedup)) achieve 2.21 $\times$ on SQuAD Dataset and 2.13 $\times$ speed-up on FEVER Dataset over Cache with FIFO ordering (Cache(FIFO))}.
%     \label{fig:rag-runtimes}
% \end{figure*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/SIGMODfigures/rag.pdf}
    \caption{End-to-end Result: Our optimizations, Cache (\greedy + Dedup + SQL Opt), achieve 2.2$\times$ on SQuAD Dataset and   2.1$\times$ speed-up on FEVER Dataset over Cache with FIFO ordering (Cache (FIFO)).} %\shu{These bars are too wide, need to narrow it a bit; change Cache (GGR) caption to Cache (GGR + Dedup + SQL Opt)}}
    \label{fig:rag-runtimes}
\end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/SIGMODfigures/multicol.pdf}
%     \caption{End-to-end Result: On a query using multiple columns (7 columns for Movies and 8 columns for Products), our optimizations (Cache \greedy + Dedup) achieve 2.6 $\times$ on both the Movies and Products Datasets over Cache with FIFO ordering (Cache FIFO)}
%     \label{fig:rag-runtimes}
% \end{figure}


\subsection{End-to-End Benchmark Results}
%\shu{Needs to add a few words about: why do we not evaluate the \optimal algorithm}
\textbf{\textit{Overview}}. Figures~\ref{fig:runtimes} and~\ref{fig:rag-runtimes} show the end-to-end latency results on our optimization techniques for our full benchmark suite. 
As baselines, we show the results of not using the KV cache for prefixes (No Cache) and caching without any reordering (Cache (FIFO)). We also measure the impact of caching with our algorithm detailed in Algorithm \ref{alg:greedy}, denoted as Cache (\greedy), and measure it without and with additional optimizations, such as deduplication and SQL optimization (i.e., Cache (\greedy+Dedup+SQL Opt)).  Our evaluation shows that our approach can achieve up to 5.7$\times$ speedup compared to baselines. 
We do not evaluate the optimal prefix hit recursion algorithm in Section~\ref{sec:optimal} as its exponential complexity makes it infeasible to run over large tables. Even for a small table, the runtime of the algorithm far exceeds the LLM inference time. For example, solving for the optimal ordering with the \optimal algorithm takes several minutes for a 10-row table. 
% We thus ignore Algorithm~\ref{alg:optimal} and 
Next, we discuss the evaluation for each query type and the other baselines in detail as below.
% We constrain the output token length for each experiment run so that we limit the token length variation whether or not we apply 

% We compare our techniques against several baselines: no KV cache, KV cache with FIFO ordering, KV

% including no KV cache and KV cache with original request order. 

% \begin{enumerate}
%     % \item Cache (with ordering): involves both column reordering and row sorting.
%     \item \accheng{need to incorporate these details somewhere}
%     \item Column reordering might change the LLM output. 
%     \item We constrain the output token length for each experiment run so that we make sure with and without column reordering, the output token length variation is not too much.
% \end{enumerate}

% Overall, we find noticeable gains in performance using our algorithm for reordering and caching over the naive and non-reordered caching approaches for each of our queries.
% \begin{enumerate}
%     \item End-to-end experiments were run including all of our optimizations.
%     \item Each query was run without prefix caching, using prefix caching without request order optimization, and using prefix caching with request order optimization.
%     \item Results for Q1-Q4 are shown in Figure \ref{fig:runtimes}. 
%     \item Results for Q5 are visible in Figure.
%     \item Our results show that the LLM calls dominate the end-to-end runtime of the query
%     \item Up to over \textbf{3x} speedup from naive batched requests using our optimizations.
% \end{enumerate}
   
% The optimizations discussed in section 4 are implemented and ablation experiments were run investigating each of them. 

\noindent \textbf{\textit{Q1: LLM projection.}} This query type applies the LLM to selected data for a given task. For the Movie dataset, we use the LLM to recommend some movies to a user based on their review of a given movie. For the Product dataset, we use the LLM to analyze whether the product quality inferred from a user's review matches the quality advertised in the product description.

Compared to our No Cache baseline, we achieve up to 3.7$\times$ speed-up on projection queries in the Movie dataset and 3.6$\times$ speed-up in the Product dataset. 
% and KV cache with FIFO ordering. \asim{these speedups are over no KV cache, not KV cache with FIFO}%\accheng{update names} 
This significant speed-up results from the sharing of large prefixes. We observe significant savings by avoiding recomputation on these longer prefixes. The No Cache baseline constructs a prompt for each row in the table and thus sends as many prompts to the LLM as there are rows in the table. No computation is saved by the model itself, and as a result, this method incurs the highest query runtime for each of our queries. 
% We benchmark against this method with our optimizations. 

% This makes sense, as Q1 was run with the longest instruction prompt for the LLM, including few-shot examples for how to answer the question asked. The total length of this prompt was 172 tokens in the Movie dataset and 141 tokens in the Product dataset. As a result, due to prefix caching, a lot of LLM recomputation is saved, as visible in the speedup from Naive to Cache(Naive). From there, cache token hits are magnified by our reordering optimizations, which brings us the remaining speedup.

We analyze the impact of our optimizations in detail on the Movie dataset. Cache (FIFO) provides a 1.6$\times$ speedup over No Cache since we can now reuse computed tokens for the instruction prompt. Our Cache (\greedy) algorithm ensures that the \textit{movie\_info} column is ordered first and groups requests with similar prefixes together to achieve a further speed-up of 2.0$\times$. Standard techniques like deduplication and SQL optimizations have minimal impact on this query type over the datasets we use. This is because the \textit{review\_content} column contains few duplicates (only 99 rows can be deduplicated), and this query does not include a filter clause. Thus, our ultimate speedup using Cache \greedy and deduplication is 3.7$\times$ over Naive and 2.3$\times$ over Cache (FIFO).

% Analyzing the Movie dataset results in detail, we see speedup with each optimization introduction. 
% \begin{enumerate}
%     \item The naive method constructs a prompt for each row in our table using the columns inputted to the UDF, and thus inputs 15,000 prompts to the LLM. No computation is saved by the model itself, and as a result this method incurs the highest query runtime.
%     \item Adding FIFO prefix caching provides X$\times$ speedup, as computation is saved caching the instruction prompt.
%     \item To make the caching more effective, we reorder our columns to be able to cache \textit{movie\_info} as well, and sort our rows by this column to make use of caching locality. With this technique, we achieve a further Y$\times$ speedup.
%     \item Our final optimizations include deduplication of inputs to the LLM and SQL filter optimization. The latter does not apply to Q1 as no filter clause is present. Because \textit{review\_content} is included as part of the prompt in this query, there are only a few (~100 rows) that are  deduplicated, and speedup is marginal.   
% \end{enumerate}

Our optimizations achieve similar improvements on the Product dataset. Cache (FIFO) improves query latency by 1.6$\times$ over the No Cache baseline. Cache (\greedy) achieves much higher speed-ups by mostly ordering the \textit{description} column first. This column contains many longer prefixes shared across different user reviews. Consequently, we achieve a 3.4$\times$ speedup over the No Cache baseline and a 2.2$\times$ speedup over Cache (FIFO). Like the Movie dataset, deduplication and filter reordering have less impact on this query type, so Cache (\greedy+Dedup+SQL Opt) achieves a 2.3$\times$ speedup over Cache (FIFO) overall. 
% There is no filter clause, and the \textit{text} column of user reviews contains many unique values. 300 rows are deduplicated, leading to a 2.3$\times$ speedup over only our caching techniques.

% The Product dataset results show similar improvement with each optimization.
% \begin{enumerate}
%     \item Adding FIFO prefix caching improves query latency only 1.1x over naive. This is significantly less speedup than in the Movie dataset, and is because the suffix length dominates the prompt token length. Specifically, the Fig\ref{tab:example-alg-values} shows the average token length of the \textit{reviewText} and \textit{desccription} input columns to be 381.54 and 282.56 tokens respectively. The prompt token length itself is only 141 tokens, so even when caching it, the majority of the LLM input must be recomputed.
%     \item Reordering mitigates the previous issue by allows us to also cache the \textit{description} column with the system prompt. Rows are sorted by this column to make use of caching locality. With this technique, we achieve a 1.7$\times$ speedup over the naive method and 1.5$\times$ speedup over naive caching.
%     \item Similar to the Movie dataset, the deduplication and SQL filter optimizations have less profound impact in this scenario. No filter cluase is present and \textit{reviewText} is mostly unique. Nonetheless, roughly 2000 rows are deduplicated leading to a further 1.4$\times$ speedup over only caching with reordering. 
% \end{enumerate}

% \accheng{missing explanation of why we achieve these wins. need to mention cache hit rate results and if the other two optimizations make a difference}


\noindent \textbf{\textit{Q2: LLM filter.}} This query type applies LLM as a filtering tool. For the Movie dataset, we filter rows based on a standard SQL operator \textit{review\_type} (with condition ``Fresh'') and an LLM operator (with condition 'Yes'). For the Product dataset, we use rows where the \textit{rating} column is equal to ``5.0'' to filter and the same LLM operator to filter for ``Yes'' for whether a product is suitable for kids.

Our algorithm Cache (\greedy) can achieve 5.6$\times$ speed-up over No Cache in the Movie dataset and 5.2$\times$ in the Product dataset. In the Movie dataset, Cache (FIFO) provides up to 1.9$\times$ speed-up over No Cache since the former saves computation by caching the instruction prompt. Cache (\greedy) provides a further speed-up of 2.1$\times$ by increasing prefix sharing.
The \textit{review\_content} column has few duplicates, so deduplication has minimal impact. On the other hand, SQL optimizations demonstrate significant performance benefits (e.g., 1.4$\times$ improvement over Cache (\greedy)) because the execution order between the non-LLM and the LLM filter impacts query latency. Pushing the non-LLM filter down first results in only 10,461 rows being passed to the LLM after the first filter (\textit{review\_type} == ``Fresh'') out of the total 15,008 rows in the table.

% Each optimization introduction introduces overall speedup in query latency. 

% In the Movie dataset, ...
% \begin{enumerate}
%     \item Adding FIFO prefix caching provides 1.7$\times$ speedup over naive, as computation is saved caching the instruction prompt.
%     \item Column and row reordering of our inputs provides further 1.6$\times$ speedup. We cache \textit{movie\_info} alongside the instruction prompt and sort our rows by this column to make use of caching locality.
%     \item Our final optimizations include deduplication of inputs to the LLM and SQL filter optimization. Once again \textit{review\_content} is included as part of the prompt in this query so few prompts are  deduplicated to the LLM. However, Q2 contains both a non-LLM and an LLM filter, the order of execution of which impacts query latency. Pushing the non LLM filter down means that only 10000 rows are passed in to the LLM after the first filter (\textit{review\_type} == ``Fresh'') out of the entire 15000 row table. This results in 1.7$\times$ improvement over caching with reordering. 
% \end{enumerate}

For the Product dataset, Cache (FIFO) provides a 1.8$\times$ speedup over the No Cache baseline. For Cache (\greedy), we order \textit{description} as the first column and cache it alongside the instruction prompt to increase the cache hit rate. For deduplication, the \textit{text} column has few duplicates, so this optimization has limited impact. Our SQL optimization enables us to push down the non-LLM filter so that only 11,994 rows out of the 15,059 are passed to the LLM after the first filter (\textit{rating} == 5.0). As a result, we achieve 1.4$\times$ improvement over only caching.

% In the Product dataset ... 
% \begin{enumerate}
%     \item Adding FIFO prefix caching provides 1.3$\times$ speedup over naive, as computation is saved caching the instruction prompt.
%     \item Column and row reordering of our inputs provides further 1.6$\times$ speedup over FIFO caching. We cache \textit{movie\_info} alongside the instruction prompt and sort our rows by this column to make use of caching locality.
%     \item Our final optimizations include deduplication of inputs to the LLM and SQL filter optimization. Once again \textit{review\_content} is included as part of the prompt in this query so few prompts are  deduplicated to the LLM. This query contains both a non-LLM and an LLM filter so the order of execution of these filters greatly impacts query latency. Pushing the non LLM filter down means that only 8874 rows are passed in to the LLM after the first filter (\textit{verified} == True) out of the entire 15000 row table. This results in 2.2$\times$ improvement over caching with reordering. 
% \end{enumerate}

% With reordering, we bring down the latency v.s. no reordering by X \%. With our SQL optimization techniques, we make sure that we apply the other filter condition first to reduce amount of inputs passed into LLM, then apply the LLM filter on reduced number of rows. We show that by pushing down cheaper predicates, we achieve a further 1.8$\times$ speedup on the Movie dataset and 2.78$\times$ on the Product dataset over only caching and reordering inputs.  \accheng{explain any difference between the two datasets or if no differences, why}

% For evaluation, we perform a query with constrained output to filter on based on the review and description columns as context for both datasets. \accheng{why mention constrained output here if we already mention earlier?}

% \sys is able to achieve X.Y$\times$ speedup in the Movie dataset and X.Y$\times$ in the Product dataset on filter queries. 
% \begin{enumerate}
%     \item Q2 uses the LLM as a filter. 
%     \item Non-LLM condition for both dataset, and LLM condition for both \shu{@asim}
%     \item Specifically, for Movie dataset we filter {add}, and for Product dataset we filter {add}
% \end{enumerate}

\noindent \textbf{\textit{Q3: Multi-LLM invocation.}} In this query, we combine Q1 and Q2 for each dataset. We first apply an LLM filter before invoking the LLM again for recommending movies and analyzing products in the \texttt{SELECT} statement. We achieve 4.8$\times$ speed-up over the No Cache baseline on the Movie dataset and 4.2$\times$ on the Product dataset on multiple invocation queries over the No Cache baseline.

For the Movie dataset, Cache (FIFO) provides 2.0$\times$ improvement over the No Cache baseline. Cache (\greedy) provides 1.7$\times$ improvement over Cache (FIFO). Our SQL optimization significantly impacts latency (2.4$\times$ speed-up over FIFO caching and 4.8$\times$ over no caching) for this query type. Since the non-LLM filter selects roughly 5,000 rows, as detailed in the previous query analysis, we significantly reduce the number of LLM invocations. 

For the Product dataset, Cache (FIFO) provides a 1.9$\times$ speedup over No Cache. Our optimizations of Cache (\greedy + Dedup + SQL Opt) provide a further 2.2$\times$ speed-up, leading to a total speedup of 4.2$\times$ over the No Cache baseline. 

% The primary latency improvement in the Q3 experiments once again comes from the SQL filter optimization. 

% Movies
% \begin{enumerate}
%     \item FIFO caching provides 1.7$\times$ improvement over naive method.
%     \item This query is essentially a combination of Q1 and Q2, so speedup is similar along with the causes for speedup.
%     \item Reordered caching provides 1.4$\times$ improvement over FIFO caching.
%     \item Applying SQL filter optimization provides an additional 1.3$\times$ speedup over caching with reordering.
% \item Filter chosen was same as Q2: \textit{review\_type == ``Fresh''}
%     \item Non LLM filter has a selectivity ratio of 0.7.
% \end{enumerate}

% Products
% \begin{enumerate}
%     \item FIFO caching provides 1.5$\times$ improvement over naive method.
%     \item Reordered caching provides an additional 1.3 $\times$ improvement over FIFO caching.
%     \item Applying SQL filter optimization provides an additional 2.2$\times$ speedup over caching with reordering. The filter selected was the same as Q2: \textit{verified == True}.
%     \item Non LLM filter has a selectivity ratio of 0.7.
% \end{enumerate}

% \begin{enumerate}
%     \item We construct the multiple invocation queries by first 
%     \item Next, a projection invocation to LLM is performed similar to Q1.
% \end{enumerate} 

\noindent \textbf{\textit{Q4: LLM aggregation.}} In this query, we use the \texttt{AVG} operator to aggregate the average sentiment score on the reviews column with the description column provided as context. For the Movie dataset, we group by \textit{movie\_title} and average over the LLM sentiment score output. For the Product dataset, we group by \textit{parent\_asin} and average over the LLM sentiment score output. We achieve a 3.6$\times$ speed-up in both the Movie and Product datasets over the No Cache baseline on aggregation queries using our optimizations. The results of this query type are similar to that of Q1, as the same columns are passed into the LLM with an instruction prompt of similar length.
 
For the Movie dataset, Cache (FIFO) provides a 1.8$\times$ speed-up over the No Cache baseline. Cache (\greedy) generates an additional 2.2$\times$ speed-up over Cache (FIFO) since the \textit{movie\_info} columns contain many shared values. Like Q1, there is no LLM-filter clause and few duplicates in the \textit{review\_content} column, so not much extra benefit is achieved with these optimizations. As a result, the query latency improvement with all optimizations is 3.6$\times$ over no caching.

For the Product dataset, Cache (FIFO) leads to a 1.6$\times$ speed-up over the No Cache baseline, and Cache (\greedy) brings a 2.2$\times$ speed-up over Cache (FIFO). Like Q1, the \textit{description} column is cached with the instruction prompt. There are marginal deduplication benefits with roughly 300 rows being removed, and the ultimate speedup is 3.6$\times$ over no caching.

% \begin{enumerate}
%     \item We use the AVG operator to aggregate an average sentiment score on the reviews column with the description column provided as context.
%     \item For Movie dataset, we group by \textit{movie\_title} and average over the LLM sentiment score output.
%     \item For Product dataset, we group by \textit{asin} and average over the LLM sentiment score output. 
% \end{enumerate}
% The results of this query are similar to that of Q1, as the same columns are passed in to the LLM with an instruction prompt of similar length. Specifically, the length of the instruction prompt was 166 tokens in the Movie dataset and 112 tokens in the Product dataset.

% Movies
% \begin{enumerate}
%     \item FIFO caching provides us with 1.9$\times$ speedup over the naive method as we cache the instruction prompt.
%     \item Reordered prefix caching adds an additional 1.8$\times$ speedup over FIFO caching, since the \textit{movie\_info} columns can be sorted on and cached. 
%     \item Like Q1, there is no SQL optimization to be made here and few duplicates because of the \textit{review\_content} column. As a result, the query latency is nearly identical to reordered caching. 
% \end{enumerate}

% Products
% \begin{enumerate}
%     \item FIFO caching leads to 1.4$\times$ speedup over the naive method as we cache the instruction prompt.
%     \item Reordered prefix caching brings 1.5$\times$ speedup over FIFO caching. Similar to Q1, the \textit{description} column is cached with the instruction prompt. 
%     \item Marginal deduplication benefits can be seen with a 1.1$\times$ improvement over reordered prefix caching with deduplication, with roughly 2000 rows being deduplicated from the original input.
% \end{enumerate}
\noindent \textbf{\textit{Q5: LLM Projection (Entire Table).}} We run a projection query for all seven columns for the Movies dataset and all eight columns from the Products dataset as detailed in Section~\ref{llmqueries}. We achieve a 3.7$\times$ speedup over the No Cache baseline on the Movie dataset and a 3.9$\times$ speedup on the Product dataset.

For the Movie dataset, Cache (FIFO) gets 1.4$\times$ speedup over No Cache baseline. For this query, we provide hints of functional dependencies to our algorithm, such as the \textit{`rotten\_tomatoes\_link'}, \textit{`movie\_info'}, and \textit{`movie\_title'} columns. These columns are grouped as they have one-to-one dependencies, so this is an FD for our algorithm. Cache (\greedy) provides a further 2.5$\times$ speedup over Cache (FIFO). It is unlikely to have exact duplicate values across seven columns, so speedup from adding deduplication is minimal. Thus, our final speedup is 3.7$\times$ over No Cache and 2.6$\times$ over Cache (FIFO). For the Product dataset, the columns of \textit{`product\_title'} and \textit{`asin'} have one-to-one dependencies, which serve as the input of the FD to our algorithm. Results on this dataset show that Cache (FIFO) is 1.5$\times$ faster than the No Cache baseline. From here, Cache (\greedy) achieves an extra 2.5$\times$ speedup over Cache (FIFO). The final speedup of our algorithm is 3.9$\times$ over No Cache and 2.6$\times$ over Cache (FIFO). 
% \begin{itemize}
%     \item We run a projection query using 7 columns from the Movies dataset and 8 columns from the Products dataset as detailed in \ref{llmqueries}.
%     \item Movies
%     \begin{itemize}
%         \item Cache (FIFO) gets 1.4$\times$ speedup over No Cache baseline.
%         \item Cache (\greedy) gets further 2.5$\times$ speedup over Cache (FIFO).
%         \item The functional dependencies here are the 'rotten\_tomatoes\_link', 'movie\_info', and 'movie\_title' columns. These are grouped together.
%         \item Not likely to deduplicate exact values across 7 columns, so speedup from adding deduplication is minimal.
%         \item Final speedup is 3.7$\times$ over No Cache and 2.6$\times$ over Cache (FIFO). 
%     \end{itemize}
%     \item Products
%     \begin{itemize}
%         \item Cache (FIFO) gets 1.5$\times$ speedup over No Cache baseline.
%         \item Cache (\greedy) gets further 2.5$\times$ speedup over Cache (FIFO).
%         \item Few duplicate values across columns.
%         \item Final speedup is 3.9$\times$ over No Cache and 2.6$\times$ over Cache (FIFO). 
%     \end{itemize}
% \end{itemize}


\noindent \textbf{\textit{Q6: RAG}}. This query is performed on a table of questions and the top three supporting evidence extracted from the SQuAD and FEVER datasets. We achieve a 3.5$\times$ speed-up on the SQuAD and 2.7$\times$ on FEVER over the No Cache baseline. In this experiment, we embed all supporting contexts for a question/claim into a FAISS index. We perform a K-nearest neighbor search on the vector index for each question to fetch the top K relevant contexts, where we choose $K = 3$. The embeddings and retrieval are computed before query time. At runtime, we apply our \greedy algorithm to the table of questions and contexts to maximize cache hits.

For the SQuAD dataset, Cache (FIFO) results in a 1.6$\times$ improvement over No Cache. Cache (\greedy) improves this further with 1.3$\times$ over Cache (FIFO). In this dataset, deduplication yields significant benefits because of the duplicated evidence lists, with only 9,561 prompts passed into the LLM after deduplication. Thus, the final speedup is 2.2$\times$ over Cache (FIFO) and 3.5$\times$ over No Cache.

For the FEVER dataset, Cache (FIFO) provides a 1.3$\times$ speedup over No Cache. Cache (\greedy) presents a further 1.9$\times$ speedup over Cache (FIFO). Roughly 3,000 out of 20,000 prompts are deduplicated. Thus, the final speedup is 2.1$\times$ over Cache (FIFO) and 2.7$\times$ over No Cache.

\noindent \textbf{Prefix Hit Rate.} We also measure the prefix hit rate (\%) for Cache (FIFO) and Cache (\greedy) for the query types in Figure~\ref{fig:runtimes}. This metric represents the ratio of tokens that can be served from the KV cache over all tokens in the input prompt. It indicates the effectiveness of the KV cache and is directly correlated with latency performance. On the Movie dataset, Cache (\greedy) achieves an average hit rate of 83.8\% while Cache (FIFO)'s average hit rate is 47.4\%. Across queries, Cache (\greedy) provides between a 22.9--45.7\% token hit rate improvement over Cache (FIFO). On the Product dataset, Cache (\greedy) achieves an average hit rate of 83.9\% while Cache (FIFO) has an average hit rate of 48.3\%. Cache (\greedy) overall can achieve 25.1--46.2\% hit rate improvement over Cache (FIFO) across different query types. %\accheng{maybe also add the raw values for context? what's a typical good cache hit rate for KV caches?}

% \subsection{Row-Reordering Ablations}
% We fix the column ordering for dataset and perform ablation experiments varying the row ordering across different queries. In this experiment, we run the same query as described in the previous section but without constraining the output token length. The end-to-end result shows that our approach achieves up to 2$\times$ on Movie, and 1.5$\times$ speedup on Product.

% \begin{table}[!t]
%     \begin{tabular}{l|r|r|l}
%     \toprule
%     Column Name   & \multicolumn{1}{l|}{ASL} & \multicolumn{1}{l|}{Cardinality} & Score \\ \midrule
%     ``description'' & 282.56                  & 144                     & 29460.80  \\ \hline
%     ``reviewText''  & 381.54                  & 12932                  & 442.97  \\ \hline
%     ``Format''       &  8.93                 & 16                     & 8379.69 \\ \bottomrule
%     \end{tabular}
%     \caption{Column statistics for Product table.}
%     \label{tab:products-alg-values}
%     \vspace{-2em}
% \end{table}
% % 

% \begin{table}[!t]
%     \begin{tabular}{l|r|r|l}
%     \toprule
%     Column Name   & \multicolumn{1}{l|}{ASL} & \multicolumn{1}{l|}{Cardinality} & Score \\ \midrule
%     ``movie\_info'' & 407.27                  & 68                     &  89946.78 \\ \hline
%     ``review\_content''  & 131.50                  & 14977                   & 131.86  \\ \hline
%     ``review\_type''       & 5.3                   & 2                     & 39797.7 \\ \bottomrule
%     \end{tabular}
%     \caption{Column statistics for Movie table.}
%     \label{tab:movies-alg-values}
%     \vspace{-2em}
% \end{table}


\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/movies_hr.pdf}
        \caption{Movie Dataset}
        \label{fig:cdf_size}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/products_hr.pdf}
        \caption{Product Dataset} 
        \label{fig:cdf_freqs}
    \end{subfigure}
    \label{fig:cachehitrate}
    \caption{Cache Hit Rate Ablation. We illustrate the cache hit rate improvements achieved by Cache (\greedy) compared to Cache (FIFO), showing up to a 46\% increase on both the Product dataset and Movie datasets.}
\end{figure}

\begin{figure}[t!]
     \centering
    \includegraphics[width=.65\linewidth]{figures/SIGMODfigures/order_ablation.pdf}
    \caption{Request Ordering Ablation. The default request order is the order of the original table. Execution with our algorithm (\greedy Request Order) achieves 2.5$\times$ speedup and 2.9$\times$ speedup on end-to-end query latency on Movie and Product Dataset, respectively.}
    \label{fig:col_ordering}
\end{figure}

\subsection{Impact of Request Reordering} 
% \accheng{Movie and Product naming?}
To measure the effect of request reordering, we evaluate how overall query latency changes under varying request orders on an LLM projection query similar to Q1. For this set of experiments, three columns provide input data into the LLM invocations from both the Movie and Product datasets. Figure \ref{fig:col_ordering} shows the query latency results for the default request order as well as the best request order outputted by our algorithm. 

For the Movie dataset, we use the \circled{1} \textit{movie\_info}, \circled{2} \textit{review\_type}, and \circled{3} \textit{review\_content} columns in the query. The default column order in execution is \circled{3}:\circled{2}:\circled{1}, whereas the \greedy puts \circled{1} first most often, followed by \circled{2} and then \circled{3}. Unsurprisingly, caching the \textit{movie\_info} column, which is repeated across different reviews of the same movie, produces a large speed-up of 2.5$\times$ over the default ordering (\textit{review\_content} first). While the \textit{review\_type} column has many shared values (there are only two unique values across the entire dataset), the length of each field is one token in length since the value is either ``Fresh'' or ``Rotten''. Due to the quadratic cost of LLM inference in regards to input length, it makes more sense to cache the \textit{movie\_info} column first as it has the longest average token length, resulting in large prefixes that improve performance significantly when they are shared across requests.
% \accheng{how long is it? why is it short?} 

    % Movies
    % \begin{enumerate}
    %     \item For the movies dataset, we choose the \textit{movie\_info}, \textit{review\_type}, and \textit{review\_content} columns. 
    %     \item Column metadata is shown in Fig \asim{insert column metadata table}.  
    %     \item Unsurprisingly, caching the \textit{movie\_info} column, which is repeated for multiple reviews on the same movie, produces the fastest query runtime at 2.0x improvement over the worst ordering of \textit{review\_content} first. 
    %     \item While the \textit{review\_type} column has many shared values across the dataset with only 2 unique values, its length is too short to see prefix caching benefits. 
    %     \item The \textit{movie\_info} column also has the longest average length, and as a result the prompt prefix to suffix ratio is high. This further improves the speedup in caching this column. 
    % \end{enumerate}

     % \accheng{why is the formatting of the col names different?}\asim{I use the default column names from the dataset?} 

For the Product dataset, we choose the \circled{1} \textit{description}, \circled{2} \textit{rating}, and \circled{3} \textit{text} columns. The default column order in execution is \circled{3}:\circled{2}:\circled{1}, whereas \greedy puts \circled{1} first most often, followed by \circled{2} and then \circled{3}. Caching the \textit{description} column, which is repeated across reviews of the same product, produces a speed-up of 2.9$\times$ improvement over the default ordering (\textit{text} first). While the \textit{rating} column has many shared values across the dataset (with only five unique values total), its length is too short, containing integer values between one and five, that are one token in length.


% \accheng{how long is it? why is it short?}  \accheng{in general or under our query?}
% thus the ratio of prefix to suffix length for the prompts in the products dataset is lower. \accheng{do you mean reviewText avg len is shorter than movie\_info avg len?} \asim{no, it's longer. that's why there's not as much improvement as in Movie dataset, because here even though the description is cached, the suffixes are longer}

    % Products
    % \begin{enumerate}
    %     \item For the products dataset, we choose the \textit{description}, \textit{format}, and \textit{reviewText} columns. 
    %     \item Column metadata is shown in Fig \asim{insert column metadata table}.  
    %     \item As expected, caching the \textit{description} column, which is repeated for multiple reviews on the same product, produces the fastest query runtime at 1.5x improvement over the worst ordering of \textit{reviewText} first. 
    %     \item While the \textit{format} column has many shared values across the dataset with only 17 unique values, its length is too short to see prefix caching benefits. 
    %     \item The improvement here is less than the movies dataset for two primary reasons: (1) The description column in the products dataset isn't replicated as often for our query. (2) The \textit{reviewText} column has the longest average length, and thus the ratio of prefix to suffix length for the prompts in the products dataset is lower.
    % \end{enumerate}

\subsection{Impact of Standard Optimizations}

\subsubsection{Deduplication}
We investigate the effects of basic deduplication in detail for our setting. We construct queries based on Q1 while changing the specific LLM column inputs. Specifically, we vary the selection of columns passed into the LLM for analysis based on their cardinality. 
% \accheng{vary the column order?} \asim{better?} \accheng{still confused, do you mean: vary which columns are passed in based on their cardinality?} 
Before LLM invocation, we deduplicate exact input prompt matches and pass only the first occurrence of each distinct prompt into the LLM. Figure~\ref{fig:dedup} shows the results on the Movie and Product datasets.

% \accheng{is this correct (pass in only 2 cols at a time)?} \asim{yes this is how this experiment was run}
For the Movie dataset, we pass in the \textit{movie\_info} column alongside either the \textit{review\_type}, \textit{review\_score}, or \textit{review\_content} columns. For these columns, the deduplication speedup is 18.4$\times$, 4$\times$, and 1.1$\times$, respectively. This is expected, as the \textit{review\_type} column has only two distinct values while the \textit{review\_score} column has only five distinct values, so the query with these columns is often deduplicated. In contrast, the \textit{review\_content} column contains mostly unique values, with only 99 rows deduplicated out of 15,018.

\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/movies_dedup.pdf}
        \caption{Movie Dataset}
        \label{fig:dedup_movie}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/products_dedup.pdf}
        \caption{Product Dataset} 
        \label{fig:dedup_products}
    \end{subfigure}
    \caption{Deduplication Ablation. Exact prompt matches are deduplicated before going into the LLM. For the lowest cardinality column on each of the Movie (review\_type: 2) and Product tables (rating: 5), deduplicating inputs leads to 18.4$\times$ and 9.3$\times$ faster query execution, respectively.}
    \label{fig:dedup}
\end{figure}

\begin{figure}[t!]
% \centering
% \includegraphics[width=0.48\textwidth]{figures/selectivity.pdf}
% \caption{Selectivity Ablation. Different columns are filtered on with resulting rows passed into LLM invocation. The lowest selectivity of the non LLM-filter for each the Movie table (0.13) yields a 6.7$\times$ faster query runtime than filtering with the LLM first.}
    \centering
     \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/movies_selectivity.pdf}
        \caption{Movie Dataset}
        \label{fig:movie_selectivity}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SIGMODfigures/products_selectivity.pdf}
        \caption{Product Dataset} 
        \label{fig:product_selectivity}
    \end{subfigure}
    \caption{Selectivity Ablation. Different columns are filtered on with resulting rows passed into LLM invocation. The lowest selectivity of the non-LLM filter for each of the Movie and Product tables (0.3 and 0.2, respectively) yields 4.2$\times$ and 3.4$\times$ faster query runtimes than filtering with the LLM first.}
    \label{fig:selectivity}
\end{figure}

For the Product dataset, we pass in the \textit{description} column alongside either the \textit{rating}, \textit{review\_title}, or \textit{text} column.
% pass in the \textit{description} column with either the \textit{summary} or \textit{reviewText} column as LLM inputs. We also pair the \textit{title} column with the \textit{overall} column as input to the LLM. 
% \accheng{unclear what this means}
The \textit{rating} column, which captures the review score, has only five distinct values, so the query with this column has 9.3$\times$ faster runtime than the no deduplication baseline. On the other hand, the \textit{review\_title} and \textit{text} columns do not contain many duplicate values as they are mostly unique to each user. As a result, deduplication achieves only 1.1$\times$ speedup for each. 

% We investigate the effect of deduplicating requests to the LLM in query execution and observe the query runtime. 
% \begin{enumerate}
%     \item We construct queries similar to Q1, varying the columns passed in to the LLM for analysis based on the cardinality of the column.
%     \item Prior to LLM invocation, we deduplicate exact prompt matches and pass only the first occurence of the prompt into the LLM.
%     \item Movies
%     \begin{enumerate}
%         \item We pass in the \textit{movie\_info} column along with the \textit{review\_type}, \textit{review\_score}, and \textit{review\_content} columns.
%         \item \textit{review\_type} has only 2 distinct values, so the query with this column had a runtime 8.2x faster than no deduplication.
%         \item \textit{review\_score} similarly has only 5 distinct values, so the query with this column had a runtime 3.3x faster than no deduplication.
%         \item \textit{review\_content} is mostly unique, with only 99 rows being deduplicated out of 15000. As a result, the differences in runtime for this query with deduplication is negligble.
%     \end{enumerate}
%     \item Products
%     \begin{enumerate}
%         \item We pass in the \textit{description} column with the \textit{summary} and \textit{reviewText} columns and the \textit{title} column with the \textit{overall} column. 
%         \item The \textit{overall} column has just 5 values representing a review score, so the query with this column had a runtime 1.9x faster than no deduplication. 
%         \item Both the \textit{summary} and \textit{reviewText} do not share many duplicate values as they are properties of a user review, and as a result deduplication achieves only 1.1x speedup for each. 
%     \end{enumerate}
% \end{enumerate}
% Figure \ref{fig:multiple-invocations-runtimes} displays end to end time runtime 
% results for the queries listed in Figure \ref{fig:multi-invoke}. A 2.3x speedup is observed from naive execution to our optimized execution of the query for the movies dataset. A 1.9x speedup is observed with the Amazon products dataset. 

\input{evaluation/table}

\subsubsection{SQL Optimizations}
Finally, we investigate the effects of our SQL optimizations. Specifically, we evaluate the latency impact of varying the order in which filter clauses for LLM queries are applied. We construct queries identical in structure to Q2 and vary the column(s) to filter on, alongside the LLM predicate of whether the movie/product is suitable for kids. %\accheng{what is the LLM predicate?}). 
We measure the overall query runtime for two scenarios: (1) the LLM filter and (2) the non-LLM filters are executed first. 
We choose columns to filter on alongside the LLM based on their \textit{selectivity ratio}, measured as the ratio of LLM input size to the table size. Figure~\ref{fig:selectivity} shows query latency as a factor of selectivity ratio. 
% \accheng{what does choose columns mean? we just vary the selectivity ratio right?} \asim{different columns are being used to do filtering to get different number of inputs into LLM}

For the Movie dataset, we choose the columns \textit{review\_type} and \textit{top\_critic} to filter on. We construct queries filtering with each possible value in \textit{review\_type} (``Fresh'', ``Rotten'') and as well as a combination of values (\textit{review\_type} == ``Fresh'' \& top\_critic = False). We find that, as expected, query latency decreases as selectivity decreases since fewer inputs are being passed into the LLM. At the lowest selectivity level in this experiment (0.3), applying this filter order optimization yields a 4.2$\times$ faster overall runtime than executing the LLM filter first. For the Product dataset, we choose the columns \textit{rating} and \textit{price}. We construct query filtering with each possible value in \textit{verified} (True, False) along with a filter on \textit{price} > 15. Like the Movie dataset, query latency decreases with fewer inputs being passed in at a lower selectivity. At the lowest selectivity level in this experiment of 0.3, applying this filter order optimization yields a 3.4$\times$ faster runtime overall over executing the LLM filter first. 
% We investigate the effect of pulling up non-LLM filter clauses prior to the LLM filter clause in an ablation experiment and observe the query runtime.
% \begin{enumerate}
    % \item We construct queries identical in structure to Q2, and vary the column(s) to filter on alongside the LLM filter.
    % \item Written naively, these queries will execute the LLM filter first on the entire table before applying the non-LLM filters. 
    % \item We collect the runtime in two scenarios: (1) the LLM filter is executed first; (2) the non LLM filters are executed first. 
    % \item We choose columns to filter on alongside the LLM based on their \textit{selectivity ratio}, measured as the ratio of inputs to the LLM to the table size. \asim{does selectivity ratio need to be explained in a DB paper??}
    % \item Movies
    % \begin{enumerate}
    %     \item We choose the columns \textit{review\_type} and \textit{top\_critic}. We ran queries filtering with each possible value of \textit{review\_type} ("Fresh", "Rotten") and "top\_critic" (True, False), and additionally ran a query filtering with a combination of those values (\textit{review\_type} = Fresh \& top\_critic = True).
    %     \item We intuitively see that query runtime decreases as selectivity decreases. We were surprised to find that the improvement was linear with the number of requests, indicating similar request token length for different queries constructed in this dataset. 
    % \end{enumerate}
%     \item Products \accheng{products results not in yet}
%     \begin{enumerate}
%         \item We choose the columns "summary", "verified", and "overall" columns. 
%         \item We ran queries filtering the 
%     \end{enumerate}
% \end{enumerate}

% \todo{Use the stage breakdown plot, plot it in matplotlib, no gray grid, use large font (i.e. 20)}

% \subsubsection{SQL Optimization}
% We evaluate the speedup in optimizing execution within the SQL engine of complex queries with multiple filter steps at various selectivities for the non LLM filter. Results are shown in Figure \ref{fig:selectivity}. We can see an obvious and intuitive speedup in end-to-end runtime for execution when evaluating the non-LLM filter first, with the speedup increasing as selectivity decreases. 



\subsection{Algorithm Analysis} %\asim{this title is a bit confusing/vague}
\subsubsection{Impact of Reordering on Accuracy} %\shu{write in paragraph, no bullet points. for any paragraphs like this with one or two sentences more than a line just rephrase and make it shorter}
In this section, we evaluate the effect of our reordering algorithm \greedy on the accuracy of LLM queries. Since our algorithm changes the order in which data fields are placed in the prompt inputted into the model, we want to ensure that doing so does not affect the quality of the LLM outputs. We select the Movie and FEVER datasets for our experiment. For the Movie dataset, we run the filter expression from Q2 as described in Section~\ref{llmqueries}. The LLM outputs either "Yes" or "No" on whether a movie is suitable for kids given movie\_info and review\_description fields. We randomly sample 100 rows and manually label them as the ground truth for the query. We run the experiment with two columns (Movies) and seven columns (Movies-Full). For the Product dataset, we run Q5 from Section~\ref{llmqueries} on the Fever Dataset. Given a claim and three pieces of evidence, the LLM is asked to determine if the claim is factually correct, outputting SUPPORTS, REFUTES, or NOT ENOUGH INFO. The FEVER dataset already contains ground truth labels for all 22,682 rows.

We run all three experiments against the Llama-3-8B-Instruct model and GPT-4o. We measure accuracy as the percentage of exact matches between the LLM output and the ground truth labels. As Movies and Movies-Full only have 100 labeled rows, we employ statistical bootstrapping \cite{bootstrapping}. We perform 10,000 bootstrap runs, where on each bootstrap, we sample a new dataset from the original dataset with replacement and calculate the accuracy of this sampled dataset. This gives us a distribution of accuracy measurements across all 10,000 runs.

In Table~\ref{tab:accuracyresults}, we show the mean over all of the bootstrap runs and a 90\% confidence interval for accuracy. Across the board, we see that the accuracy distribution of \greedy ordering is within 5\% accuracy of the original ordering. The only exception is Fever with Llama3-8B, in which the ordering with \greedy performs significantly better than the original. This is due to the \greedy algorithm preferring to place the "claim" column at the end of the prompt instead of at the beginning. However, the same behavior does not hold for GPT-4o, showing that higher-quality models are more robust to column reordering.

\subsubsection{Algorithm Overheads}

Table~\ref{tab:solvertimes} shows the \greedy algorithm overheads on each of our experiment datasets. The solver is run on the Movies, Products, and SQuAD datasets with an early stopping threshold of group size 2. In the recursive process, if the max group found is size two or lower, we fall back to the column orderings for the sub-tables using table statistics.  We use an early stopping threshold of 1,000 on the FEVER dataset. The FEVER dataset requires the longest solving time using \greedy, with a mean solver time of 90 seconds. This dataset has the highest number of unique groups, so the recursive depth is also the highest. The Movies, Products, and SQuAD datasets require a solver time between 20 and 30 seconds, which is small compared to the LLM inference time, which is generally in the range of tens of minutes. Adding deduplication following our algorithm adds only linear time overhead, so its impact on end-to-end latency is minimal. The deduplication step can even be skipped if it is inferred from table statistics that there are many unique values.
% \shu{Add a few sentences on the algorithm overhead of dedup (over many distinct tables, say if the table statistics indicate that many distinct value, it does not worth doing dedup )} 

%\asim{shu: review this analysis}

\input{evaluation/e2e_runtimes}
\input{evaluation/rag_e2e_runtimes}

==> sections/7_discussion.tex <==
\section{Discussion} 
% \accheng{discussion or limitations?}
% \shu{@Audrey: removing subsections, and just have short sections on paragraph}
% \shu{Some additional discussions we want to have: different prompt length, different GPU types, different models (reference the VLDB reviewer comments)}
% Our techniques for optimizing LLM queries have been pragmatically motivated: we consider straightforward optimizations that apply broadly to most LLM inference systems and relational databases. 
We consider straightforward optimizations that apply broadly to most LLM inference systems and relational databases. In this section, we outline future research directions to enhance LLM inference in relational analytics further.
% that can extend the current capabilities of optimizing SQL queries involving LLM invocations. 
% Our discussion is organized into three subsections: distributed cache and request routing, cost estimation for LLM invocations, and semantic de-duplication. These directions are critical to improving the scalability of database systems with LLM invocations. 

% \accheng{not sure about this term} \simon{maybe the reverse: ... scalability of database systems with LLM invocations}, ensuring that the benefits of LLM integration can be realized more widely.
% achieved across multiple computational environments. 

% \joey{We don't leverage this decode length knowledge but it could be a big opportunity for a future version of this paper. I wonder if we want to mention that in the future work. }

% \subsection{Column Reordering and Row Sorting} 
% \label{sec:reordering-future}
% Our column reordering and row sorting algorithms leverage straightforward, practical heuristics to efficiently identify shared prefixes. We can further extend these algorithms in future work by adopting a finer-grained approach. For instance, instead of maintaining a fixed order of columns for all rows in a table, we can consider different column orderings for subsets of rows to potentially enable higher token hit rates.

% To do so, one potential strategy would be to iteratively determine column orders for each group of rows that share a value in a designated ``pivot'' column. Once an order is established for a group, we can exclude these rows from subsequent iterations, thereby reducing the complexity and focusing on determining the orders of the remaining rows. This recursive approach would allow us to progressively refine the column order to enhance the cache hit rate without giving up computational efficiency. Moreover, we plan to introduce a pruning mechanism for columns that consistently show negligible impact for prefix sharing. By excluding these columns from the reordering process, we can further reduce the computational overhead of this technique. %and potentially further optimize the overall performance of the system. 

% before show potential for optimizing cache efficiency through intelligent data arrangement. 
% However, the current approach, which maintains a fixed order of columns for all data rows, may not work well for all datasets. In our future work, we aim to refine the algorithm by adopting a more fine-grained approach that considers unique value-based column ordering for each data segment.  

% One potential strategy involves an iterative process where, for each group of rows sharing a unique value in a designated "pivot" column, we determine an optimal column ordering. Once an order is established for a group, we exclude these rows from subsequent iterations, thereby reducing the complexity and focusing on remaining data subsets. This recursive approach allows for progressively refining the data structure to maximize cache hit rates and computational efficiency. Moreover, we plan to introduce a pruning mechanism for columns that consistently show negligible impact on cache efficiency. By excluding these columns from the reordering process, we can reduce computational overhead and potentially further optimize the overall performance of the system. 

% \subsection{Prefix Caching: Opportunities}
% \subsubsection{Decode Length Knowledge} 
% While our work focuses on memory management for input prompts, output decoding also has a significant impact on performance. In particular, there are potential performance benefits with guided decoding in the analytics setting. Guided decoding, also known as structured generation or controlled generation, is a popular method to deterministically enforce a schema on the output of LLM \cite{guidance, sglang, outlines, lmql, aici}. Since guided decoding involves computing a large intermediate state, it does not typically employ batching, hurting GPU utilization. In the relational analytics scenario, we can utilize our knowledge of the output schema and decoding length to construct the output constraint ahead of time. In many cases, we can skip tokens that are known a priori and perform batching to improve utilization.
% \simon{Shu I think this paragraph is broken}
% \shu{We can skip this}


% on the optimizing the input process of the data in LLM, decoding the output is equally important factor to consider. There are many opportunities in applying guided decoding in relational analytics settings. Guided decoding, also termed structured generation or controlled generation, is a popular method to deterministically enforce a schema on the output of LLM \cite{guidance, sglang, outlines, lmql, aici}. The typical method of guided decoding involves computing a large finite state machine over the token space to constrain the tokens to be allowed for sampling. This process typically does not batch, hurting GPU utilization.



% \shu{@simon add the constrained decoding and some opportunities with batching here}
% \asim{can maybe add a small section here to discuss "very large" tables leading to long prompts, and say it is unclear how this impacts our algorithm performance and overall runtime. however, we can also clarify that for such a table it would be standard practice to only pass in a few columns to the LLM}
\paragraph{Batch-Aware Reordering.} \label{sec:smarter_reordering}
While column reordering and row sorting can improve cache hit rates, they don't account for how requests in a batch are processed in parallel during LLM inference. Some systems \cite{tgi} do not support prefix sharing within the same batch. For example, processing requests in the sequence $[1,1,1][2,2,2][3,3,3]$ leads to six cache misses, as each prefix ($1,2,3$) is recomputed in the same batch. However, reordering to $[1,2,3][1,2,3][1,2,3]$ reduces cache misses to three. To address this, we propose a batch-aware reordering strategy. This strategy should include a warm-up phase to pre-load the cache with diverse prefixes expected to be reused in subsequent batches and should be aware of inference batch size.% The algorithm sorts prefixes by frequency and arranges them across batches to ensure each batch contains distinct prefixes, thereby reducing cache misses significantly.
% ensure maximum cache utilization due to how 
% \begin{itemize}
%     \item Since inference occurs simultaneously for all requests in a batch, prefixes cannot be shared within the same batch.
%     \item Consider a sequence of requests $[1,1,1][2,2,2][3,3,3]$. None of these prefixes benefit from being cached because each distinct prefix ($1,2,3$) is computed multiple times with the same batch. As a result, there are six cache misses on this workload.
%     \item However, if we instead reorder these requests according to the sequence $[1,2,3][1,2,3][1,2,3]$, we observe benefits from using the prefix cache---$1, 2, 3$ are computed and cached after the first batch, allowing them to be reused in subsequent batches. Thus, there are only three cache misses on this series of requests.
% \end{itemize}

% The constraints of parallel batch computation necessitate a \textit{warm-up phase} that loads the cache with prefixes that will reused in subsequent batches. To further increase cache hit rate, we ...\accheng{shu, can you summarize the high-level idea of the alg in 1-2 sentences?}
% % e develop an algorithm to further increase cache hit rate while also ensuring we can run the largest batch size possible to fully utilize the GPU compute and memory capacity.

% \begin{itemize}
%     \item First, we sort all prefixes based on descending frequency. 
%     \item Then, we fill batches with distinct prefixes based on the sorted order.
%     \item Once all requests involving a given prefix have completed, we replace this prefix as we serve further requests (with different prefixes) following our sorted order.

%     \item For the example above with request prefixes $\{1,1,1,2,2,2,3,3,3\}$, our algorithm would construct batches $[1,2,3][1,2,3][1,2,3]$, which maximizes cache hit rate.
%     \item More complex example: reference Table \ref{tab:cache-state-comparison-warmup}.
    
% \end{itemize}

% \begin{table}[!t]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \multicolumn{1}{c|}{T} & \multicolumn{2}{c|}{Naive Reordering} & \multicolumn{2}{c}{Better Reordering} \\ \hline
%         & Keys accessed & Cache state & Keys accessed & Cache state \\ \hline
%         1 & ${\color{red}1, 1, 1}$ & - & ${\color{red}1, 2, 3}$ & - \\ \hline
%         2 & - & $1$ & - & $1, 2, 3$ \\ \hline
%         3 & ${\color{red}2, 2, 3}$ & $1, 2, 3$ & $1, 2, 3$ & $1, 2, 3$ \\ \hline
%         4 & - & $1, 2, 3$ & - & $1, 2, 3$ \\ \hline
%         5 & $3, 3, 3$ & $1, 2, 3$ & $1, 3, 3$ & $1, 2, 3$ \\ \hline
%     \end{tabular}
%     \vspace{0.5em}
%     \caption{Comparison of cache state of different input orderings for Section 3.4: three requests of 1, two requests of 2, four requests of 3. Better ordering can reduce the cache misses by half.} 
%     \label{tab:cache-state-comparison-warmup}
% \end{table}

% \shu{Future work; put it before related work; bsection about each of the possible future extension: http://www.bailis.org/papers/bolton-sigmod2013.pdf}
% \accheng{have we discussed these with a prof yet?}
% \simon{I think it is a very natural to claim this}
% \accheng{as in, is there something specific about batch analytics + the distributed setting we want to mention? the text currently seems to apply to LLM inference systems in general}
% \accheng{go back to calculations for 100GB so want to distribute but this is hard
% reiterate that we're opening a new area}
\paragraph{Distributed Cache and Request Routing.}
On large-scale datasets, we need to distribute the inference workload over many machines to enable queries to be completed in a reasonable amount of time. However, distributed KV caching is challenging; we need to ensure that requests with similar or identical prefixes are directed to the same machine. As such, balancing load over different machines with varying cache contents will be a critical objective. 

%RAG queries bring additional complexities since the KV cache must store not only LLM prefixes but also embeddings and associated retrieved contents, which may be distributed across nodes.

% Our current system has demonstrated potential for improving performance through request formulation and prefix caching for LLM on a single machine, tailored specifically for relational analytics tasks. However, deploying such systems in real-world scenarios often involves distributed computing environments where queries are processed across multiple nodes \cite{spotserve}. 

% In a distributed environment, maintaining cache locality is important. We want to ensure that requests with similar or identical prefixes are directed to the node where those prefix KVs are cached. The challenge compounds when dealing with RAG queries. Here, the cache not only contains the LLM prefixes but also can be the embeddings and associated retrieved contents, where may be distributed across nodes. Optimizing cache locality in this context both means LLM internal KV cache locality and also the data locality associated with query processing. 

% In addition, we want to ensure that no single node becomes a bottleneck. Our request routing should distribute both the computational load and data storage in a manner that prevents any single node from being overwhelmed. This requires real-time monitoring and adaptive request distribution strategies that can react to the cache access patterns and specific query demands. 


% Future work should focus on the development of distributed LLM cache management strategies that optimize these factors. This could involve techniques for intelligent request routing based on cache content locality, thereby leveraging local cache hits to minimize LLM computation. For RAG queries, where embeddings can potentially be stored across different nodes, it is also essential to consider the locality of retrieved contents to reduce data transfer times. 

% \subsection{Cost Estimation}
% \accheng{what makes LLM workloads interesting is that we can have decode constraints so we can predict what the responses will be like} \accheng{could drop this if nothing unique}
% Our system utilizes predicate push-down techniques to reduce the number of LLM invocations within SQL queries, focusing primarily on local execution scenarios. However, in many real-world scenarios, LLMs are not run locally but are accessed via remote endpoints \cite{openai-pricing}, and there can be different types of LLM models invoked in the query.

% Future research should aim at developing cost estimation models that account for the types of models that are used, and the complexities of remote LLM executions. This involves assessing factors such as network latency and data transfer costs, which are particularly relevant when LLMs are deployed across different geographical locations. Moreover, understanding the computational load of different LLMs and how they interact with SQL queries is essential for precise cost modeling.

% Building on this, there is a compelling need for development on a more intelligent SQL optimizer.  

\paragraph{Semantic Deduplication.}\label{sec:semantic_dedup}
We can extend our exact deduplication technique to filter out more data by implementing rule-based methods. Specifically, we can leverage NLP pre-processing techniques that remove case sensitivity (e.g. ‘Apple’ and ‘apple’) and noise (e.g. ‘<Apple>’ and ‘Apple’) as well as apply stemming and lemmatization (e.g. ‘running’, ‘ran’, ‘runs’ ), spelling correction (e.g. ‘mitake’ vs. ‘mistake’), and stop word removal (e.g. remove ‘a’, ‘the’, etc.). These could be implemented as hard constraints (optionally specified by the user) to reduce the number of LLM invocations without impacting query accuracy since the equivalence of text is specified via the given rules. We can deduplicate even more aggressively by identifying semantically similar rows. For example, "I like this restaurant" and "I love this place" have the same semantic meaning and will likely produce identical output under an LLM sentiment analysis task, so we can send only one of these inputs.
%As such, sending only one of these inputs to LLM for processing should be sufficient for most purposes. 
% While there has been previous work on statistically bounding the accuracy of inference for neural networks~\cite{} \accheng{and other settings?}, this is an open problem for LLMs.  \simon{I don't need we need to open to this direction? Added SemDeDup}
% One possible direction is to evaluate token similarity within the LLM to identify semantically equivalent requests. We are also looking forward to bringing in methods in training dataset de-duplication such as SemDeDup \cite{semdedup} for production workload processing.
% We could provide different thresholds for the user to specify desired query accuracy, similar to techniques used in neural network queries over video~\cite{noscope}. \accheng{others have explored bounding statistical settings but it's an open problem for LLM}
% \accheng{token level similarity }


% \simon{
% A natural extension to this work is to de-duplicate semantically similar rows to reduce computation. For example, de-duplicating "I like this restaurant" and "I love this place" for a sentiment analysis task because they have the same semantic meaning and the output will be identical.

% Importantly, we believe the de-duplication should not affect accuracy of LLM generation. This means the final output should be exactly the same as if it is processed with original batch of rows. Therefore, we see the future work to leverage rule based methods instead of embedding based similarity search. 

% For example, the rules can include using \textit{DISTINCT} for exact de-duplication, removing case sensitivity (e.g. ‘Apple’ and ‘apple’), removing noise (e.g. ‘<Apple>’ and ‘Apple’), stemming and lemmatization (e.g. ‘running’, ‘ran’, ‘runs’ ), noun normalization (e.g. ‘USA’ and ‘United States’ ), spelling correction (e.g. ‘mitake’ vs. ‘mistake’), and stop word removal (e.g. remove ‘a’, ‘the’, etc.). 

% Furthermore, being aware of the tokenizer's behavior can helo further de-duplication. For example, while \textit{\_hi} (with white-space) and \textit{hi} (without white-space) are two different tokens, they are semantically equivalent.
% }


% We choose to avoid affecting the accuracy of query results.

% Hard Rules: 
% \textbf{Solution} 
% \begin{itemize}
%     \item Exact deduplicate with \textit{DISTINCT} before input to external UDF 
%     \item Deduplicate with hard rules for entity resolution datasets 
%     \begin{itemize}
%         \item Case sensitivity: E.g. ‘Apple’ and ‘apple’ 
%         \item Noise removal: E.g., ‘<Apple>’ and ‘Apple’
%         \item Stemming and lemmatization: E.g., ‘running’, ‘ran’, ‘runs’ 
%         \item Normalization: E.g., ‘USA’ and ‘United States’ 
%         \item Word correction: E.g., ‘mitake’ vs. ‘mistake’
%         \item Stop word removal: E.g., remove ‘a’, ‘the’, etc.
%     \end{itemize}
%     \item TODO: token-level deduplication and workload shaping 
% \end{itemize}

% And semantic duplicates
% \textbf{Prefix Cache}
% \begin{enumerate}
%     \item Multi-tenant queries (even larger batch)
%     \item Distributed setup: caching and routing to different cores based on locality 
%     \item Optimize sub-hits 
%     \item Advanced cost estimation on different models as input to LLM 
% \end{enumerate}
% \textbf{Deduplication}
% \begin{enumerate}
%     \item Can say that provide an interface for users to specify those hard rules according to their heuristics 
%     \item Left semantic deduplication for future work 
% \end{enumerate}

% \textbf{More TODOs (relevant directions)}
% \begin{itemize}
%     \item When SQL queries involve joins with each side using different LLMs, understanding the computational costs of these models is crucial for optimizing query execution
%     \begin{itemize}
%         \item E.g. if we have two LLMs, LLM-A (less expensive) and LLM-B (more expensive), the join type (left-join, right-join, inner-join) impacts the efficiency and cost
%         \item Ideally, the more expensive model (LLM-B) should process fewer rows to minimize costs
%         \item The order of join and choice of model should be decided based on some factors like size of datasets, and complexity of tasks they perform 
%     \end{itemize}
%     \item Different model choices affect the cost model 
% \end{itemize}

==> sections/8_related-work.tex <==
\section{Related Work}

Our optimizations build on recent work in LLM inference as well as prior work integrating machine learning and data management. We describe several major related areas below.

% \textbf{Outline}
% \begin{enumerate}
%     \item Existing pipeline tools
%     \begin{enumerate}
%         \item Langchain
%         \item Llamaindex
%     \end{enumerate}
%     \item Throughput optimized LLM inference
%     \begin{enumerate}
%         \item FlexGen
%         \item vLLM
%     \end{enumerate}
%     \item Vector DB papers
% \end{enumerate} 

% \noindent \textbf{Text2SQL.} LLM usage in Text2SQL tasks, where an LLM generates SQL queries given a natural language prompt, has been increasingly explored in recent work ~\cite{gao2023texttosqlempoweredlargelanguage}\cite{zhang2024benchmarkingtexttosqlcapabilitylarge}. While this task involves LLM inference on tabular data, it is distinct from our setting of optimizing LLM operators that are called within SQL queries.  Future work may explore Text2SQL where an LLM generates a SQL query that itself contains LLM operators. %\asim{shu/amog: review this}

% \noindent \textbf{Model pipeline tools.} LLM toolkits, which have grown rapidly in popularity, provide users with the ability to stitch model pipelines together from basic abstractions. Among these, LangChain \cite{langchain} and LlamaIndex \cite{llamaindex} have seen the most usage. LangChain's framework allows for convenient abstractions for different parts of the LLM serving stack and also enables users to ``batch'' multiple requests into a model. However, this is accomplished through basic thread parallelism and without any model optimizations applied to handle the series of queries found in a typical analytics workload.  \amog{Replace this with Text2SQL? Model pipeline tools should be combined with Inference-optimized system section. And I wouldn't realy consider LlamaIndex and LangChain to be model pipeline tools.} \asim{agreed this can be removed now I think}
% \accheng{so this is more basic than vLLM? what's the relation to our work?} \simon{This can be taken out, but I think these actually are more high level LLM workflow tool that can benefit from this work. Think an ORM to a DB.}
\vspace{-0.5em}
\noindent \textbf{Inference-optimized systems.} There has been a recent rise of dedicated systems for LLM inference, including FasterTransformer \cite{faster-transformers}, Orca \cite{orca-continous-batching}, vLLM \cite{vllm}, and FlexGen \cite{flexgen}. Our work builds upon prior work investigating high-throughput LLM inference and continuous batching for model serving. However, past systems focus on the online setting and make no assumptions about the requests sent to the LLM. In contrast, we leverage full workload information from batch queries to improve performance significantly.

% vLLM \cite{} introduces a system for efficient memory management during serving, which is relevant to our problem scenario with potentially large batches of queries. Specifically, our system relies on vLLM's scheduler and utilizes parallel decoding in a continuous batching strategy. Furthermore, the system processes requests in the order they arrive to the model engine. This was something we believe can be improved in an analytics setting, where the order of outputted responses is less critical, and smarter execution planning can be done within the model to reuse computation with common prefixes. 

% FlexGen \cite{} applies both offloading and quantization to efficiently serve large models on limited gpu space with high throughput. However, trade-offs are made for the system assuming a set of latency-insensitive tasks. Our goal was to create a unified abstraction to augment analytics with LLM capabilities while still preserving the ability to make fast, one-off queries on both tabular and unstructured data. 
\vspace{-0.5em}
\noindent \textbf{Prefix Sharing.} Recent work explores developing memory-efficient GPU kernels that perform inference while leveraging shared prefixes. %to compute LLM attention leveraging shared prefix. 
SGLang's RadixAttention \cite{sglang}, Hydragen \cite{hydragen}, and Cascade Inference \cite{cascade-inference} all implement optimized kernels. Our work heavily leverages these kernels to enable prefix sharing while delivering higher throughput as compared to traditional attention kernels \cite{flash-attention}. % \shu{try reducing this}
% \accheng{unclear how these kernels are different from other kernels. what are the other kernels? how does our work leverage these kernels?} \simon{I cited the baseline kernels. This section is to claim we are not on the same track as these work by building on top of the.} achieve memory saving

% \shu{DBML}
\vspace{-0.5em}
\noindent \textbf{LLMs in Relational Data Analytics} 
% \accheng{Ralf and Velox citation} \simon{done}
% There is extensive work on integrating machine learning models with analytics~\cite{noscope,blazeit,prob-pred}. MADLib~\cite{madlib} is one example of many works that have focused on designing systems to train complex models on large datasets. Recent works such as Velox explore online serving using data management systems~\cite{velox}, and Ralf optimizes machine learning feature maintenance in data pipeline ~\cite{ralf-feature-store}. \amog{The works above don't seem very related to our work at all. Systems for training models, or feature stores are unrelated.} 
% There has been prior work on frameworks to run ML models or LLMs as operators on relational data. Systems like Spark MLlib\cite{sparkmllib}, and SystemML\cite{systemml} However, these past works did not specifically address large language models with extremely high computational costs and unique architectural properties, such as the KV cache. As such, LLMs offer many new optimization opportunities in the context of analytics.
There are many systems that support calling LLMs as operators on relational data, spanning from production database vendors like Databricks \cite{databricks-ai-functions}, Google BigQuery \cite{google-bigquery-llm} and AWS Redshift \cite{aws-redshift-llm} to programming frameworks like LOTUS \cite{lotus}. While these works provide APIs for running LLMs over relational data, they do not specifically explore data reordering optimizations to maximize KV cache hits. NoScope~\cite{noscope}, BlazeIt~\cite{blazeit}, and Probabilistic Predicates~\cite{prob-pred} propose approximating expensive ML model calls with less expensive models for approximate query processing, but this can reduce query accuracy, and does not take advantage of the unique opportunities for KV cache reuse in LLM inference.

% 
% Blending advancement of machine learning with database technologies is not new. For example, both MADLib \cite{madlib} and Velox \cite{velox} adds model training and inference as part of analytic workflow. However, the past literature focus on classical machine learning algorithms such as linear regression and K-means clustering. Large language models are a lot more expensive to compute and have interesting properties related to prefix sharing. Therefore, LLMs open up new opportunities to for relational operator optimization such as sorting and better cost estimation. \simon{this paragraph is poorly written, someone plz rewrite it}

% \accheng{Joey/Matei, is there other related work we should be citing?} \matei{approximate queries with ML in SQL: NoScope, BlazeIt, Probabilistic Predicates}
